DAG-aware Synthesis Orchestration

The key methodologies of modern logic synthesis techniques are conducted on multi-level technology-independent representations such as And-Inverter-Graphs (AIGs) of the digital logic via directed-acyclic-graph (DAGs) traversal based structural rewriting, resubstitution, and refactoring. Existing state-of-the-art DAG-aware logic synthesis algorithms are all designed to perform stand-alone optimizations during a single DAG traversal. However, we empirically identify and demonstrate that these algorithms are limited in quality-of-results and runtime complexity due to this design concept. This work proposes Synthesis Orchestration, which orchestrates stand-alone operations within the single traversal of AIG. Thus, orchestration method explores more optimization opportunities and results in better performance. Our experimental results are comprehensively conducted on all 104 designs collected from ISCAS'85/89/99, VTR, and EPFL benchmark suites, with consistent logic minimization improvements over rewriting, resubstitution, refactoring, leading to an average of 4% more node reduction with improved runtime efficiency for the single optimization. Moreover, we evaluate orchestration as a plug-in algorithm in resyn and resyn3 flows in ABC, which demonstrates consistent logic minimization improvements (3.8% and 10.9% more node reduction on average). The runtime analysis demonstrates the orchestration outperforms stand-alone algorithms in both AIG minimization and runtime efficiency. Finally, we integrate the orchestration into OpenROAD for end-to-end performance evaluation. Our results demonstrate the advantages of the orchestration optimization technique, even after technology mapping and post-routing in the design flow have been conducted.

==> TCAD24-Orch/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Logic optimization plays a critical role in design automation flows for digital systems, significantly impacting area, timing closure, and power optimizations~\cite{bjesse2004dag, haaswijk2018deep, brayton1990multilevel, amaru2015majority, mishchenko2007abc, yu2020flowtune, yu2018developing}, as well as influencing new trends in neural network optimizations~\cite{rai2021logic, huang2022quantized}. The goal of logic optimization is to achieve higher performance, reduced area, and lower power consumption, all while maintaining the original functionality of the circuit.

Modern digital designs are complex and feature with millions of logic gates, coupled with an extensive exploration space. This complexity underscores the importance of efficient, technology-independent optimizations for design area and delay at the logic level. Key methodologies in modern logic optimization techniques are conducted on multi-level, technology-independent representations, such as And-Inverter-Graphs (AIGs)~\cite{mishchenko2006dag, mishchenko2005fraigs, yu2016dag} and Majority-Inverter-Graphs (MIGs)~\cite{amaru2015majority, soeken2017exact}, for digital logic. Additionally, XOR-rich representations are crucial for emerging technologies, as seen in XOR-And-Graphs~\cite{ccalik2019multiplicative} and XOR-Majority-Graphs~\cite{haaswijk2017novel}.


A framework for logic synthesis, {ABC}~\cite{mishchenko2007abc}, introduces multiple state-of-the-art (SOTA) Directed-Acyclic-Graphs (DAGs) aware Boolean optimization algorithms. These include structural rewriting (command \textit{rewrite} in ABC)~\cite{mishchenko2006dag, riener2022boolean, haaswijk2018sat}, resubstitution (command \textit{resub} in ABC)~\cite{brayton2006scalable}, and refactoring (command \textit{refactor} in ABC)~\cite{mishchenko2006dag}, all of which are based on the AIG data structure. {During the existing logic optimization process, the algorithm considers a single specific optimization method and applies the optimization based on a single criterion~\cite{mishchenko2006dag}. }%For instance, during the single AIG traversal in the \textit{rewrite} algorithm, each node is evaluated against the optimization criterion of structural rewriting, and optimization is applied accordingly. Even though some logic cuts might be optimized using other methods, such as \textit{refactor} and \textit{resub}, these optimization opportunities are overlooked during the singular \textit{rewrite} optimization process.} %Therefore, existing optimization methods that consider only one specific optimization within a single traversal of the AIG are referred to as "stand-alone" optimizations in this context.}
Our empirical studies further reveal critical limitations inherent in the mainstream stand-alone concept of logic optimization, particularly in missing significant optimization opportunities. These opportunities are often overlooked due to a consistent tendency of becoming stuck in "bad" local minima. In other words, the optimization of a node, when various applicable optimization opportunities are present, is constrained by the limitations inherent in the current stand-alone optimization concept. For instance, as depicted in Figure \ref{fig:aig_alone}, although node $g$ is suitable for both \textit{refactoring} and \textit{resubstitution}, it misses potential optimization opportunities when subjected solely to \textit{rewriting}. 

{In this work, we propose a novel logic synthesis development concept, \textbf{DAG-aware Synthesis \textit{Orchestration}}, that maximizes optimizations through Boolean transformations by orchestrating multiple optimization operations in the single traversal of the logic graph.} Specifically, we implement the synthesis orchestration approach based on AIGs by orchestrating \textit{rewrite}, \textit{refactor}, and \textit{resub} implemented in ABC~\cite{mishchenko2007abc} in the single optimization command \textit{orchestration}. The orchestration algorithm is orthogonal to other DAG-aware synthesis algorithms, which can be applied to Boolean networks independently and/or iteratively. Our results demonstrate that applying orchestration in DAG-aware synthesis can significantly improve logic optimization compared to the existing optimization methods. We anticipate that the concept of logic synthesis orchestration can be effectively extended to other data structures, such as Majority-Inverter Graphs (MIGs)~\cite{amaru2015majority}.
%For each AIG node, \textit{orchestration} provides all valid operations to select from and apply the operation to update the graph, as illustrated in Figure \ref{fig:aig} and Figure \ref{fig:orch_flow}. With our method, the optimization space within the single traversal of the AIG is expanded and more optimization opportunities are explored at the same runtime scale. 

The main contributions of the work are summarized as follows:
\begin{itemize} 
    \item Our comprehensive analysis and examples (Figures \ref{fig:aig_alone} and \ref{fig:ana}) highlight significant optimization losses in current logic optimization implementations. %Comprehensive node optimization opportunity analysis (Figures \ref{fig:aig_alone} and \ref{fig:ana}) and motivating examples are provided, which demonstrate significant optimization opportunity loss in existing SOTA implementations.
    
    \item We propose two DAG-aware synthesis orchestration algorithms, \textit{Priority-ordered orchestration} and \textit{Local-greedy orchestration} to define the criteria for orchestrating \textit{rewrite}, \textit{refactor}, and \textit{resub} in AIG optimizations (Section \ref{sec:approach}).
    
    \item We provide the performance evaluations and runtime analysis on 104 designs from five benchmark suites (ISCAS'85/89 \cite{brglez1989combinational}, ITC/ISCAS'99 \cite{davidson1999itc}, VTR \cite{murray2020vtr}, and EPFL benchmarks \cite{soeken2018epfl}), which shows our {orchestration} technique achieves an average of 4.2\% more AIG reductions compared to existing logic optimization algorithms in ABC (Section \ref{sec:single_result} and \ref{sec:runtime_result}). %We provide comprehensive evaluation and explorations of proposed \texttt{orchestration} on 104 designs collected from five benchmark suites, including ISCAS'85/89 \cite{brglez1989combinational}, ITC/ISCAS'99 \cite{davidson1999itc}, VTR \cite{murray2020vtr}, and EPFL benchmarks \cite{soeken2018epfl}, with an average of 4.2\% more AIG reductions compared to SOTA stand-alone optimizations. %, and provides $11.7\%$ optimization in graph size compared to \textit{resyn}, and $2.24\times$ compared to \textit{resyn3} .
    \item We provide the evaluations of sequential optimizations with {orchestration} algorithms, where the {orchestration} techniques show its performance advantage of 4.7\% for \texttt{resyn} and 11.5\% for \texttt{resyn3} (Section \ref{sec:iterative_result}). 
    \item We further integrate orchestrated logic optimizations into OpenROAD \cite{ajayi2019openroad} for end-to-end design evaluations, demonstrating consistent AIG minimization and area improvements for post-technology mapping and routing (Section \ref{sec:eval_openroad}). %We further integrate the orchestrated logic optimization into OpenROAD \cite{ajayi2019openroad} to evaluate the \texttt{orchestration} performance w.r.t the end-to-end chip design flow, demonstrating consistent AIG minimization and area improvements for post technology mapping and post routing.
    \item Our approach is available in ABC \cite{mishchenko2007abc} through a new command, \textit{orchestration}.
\end{itemize}


 

==> TCAD24-Orch/2_preliminary.tex <==
\section{Preliminary}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{figs/aig_ori-crop.pdf}
        \caption{original AIG}
        \label{fig:aig_ori}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{figs/aig_rw-crop.pdf}
        \caption{AIG with \texttt{rw}}
        \label{fig:aig_rw}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
\includegraphics[width=1\textwidth]{figs/aig_rf-crop.pdf}
        \caption{AIG with \texttt{rf}}
        \label{fig:aig_rf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
\includegraphics[width=1\textwidth]{figs/aig_rs-crop.pdf}
        \caption{AIG with \texttt{rs}}
        \label{fig:aig_rs}
    \end{subfigure}
    
    \caption{{The optimized graph produced by stand-alone optimization operations: (a) original AIG, graph size is 25; (b) optimized AIG with stand-alone \texttt{rw}, graph size is 23; (c) optimized AIG with stand-alone \texttt{rf}, graph size is 23; (d) optimized AIG with stand-alone \texttt{rs}, graph size is 22.}
    }
    \label{fig:aig_alone}
\end{figure*}

\subsection{Boolean Networks and AIGs}
\label{sec:background_BN}
A Boolean network is a directed acyclic graph (DAG) denoted as $G=(V, E)$ with nodes $V$ representing logic gates (Boolean functions) and edges $E$ representing the wire connection between gates. The input of a node is called its \textit{fanin}, and the output of the node is called its \textit{fanout}. The node $v \in V$ without incoming edges, i.e., no \textit{fanins}, is the \textit{primary input} (PI) to the graph, and the nodes without outgoing edges, i.e., no \textit{fanouts}, are \textit{primary outputs} (POs) to the graph. The nodes with incoming edges implement Boolean functions. The level of a node $v$ is defined by the number of nodes on the longest structural path from any PI to the node inclusively, and the level of a node $v$ is noted as $level(v)$.

%\subsection{And-Inverter Graph (AIG)}
%\label{sec:background_AIG}
\textit{And-Inverter Graph} (AIG) is one of the typical types of DAGs used for logic manipulations, where the nodes in AIGs are all two-inputs AND gates, and the edges represent whether the inverters are implemented. An arbitrary Boolean network can be transformed into an AIG by factoring the SOPs of the nodes, and the AND gates and OR gates in SOPs are converted to two-inputs AND gates and inverters with DeMorgan's rule. There are two primary metrics for evaluation of an AIG, i.e., \textit{size}, which is the number of nodes (AND gates) in the graph, and \textit{depth}, which is the number of nodes on the longest path from PI to PO (the largest level) in the graph. 
{A \textit{cut} $C$ of node $v$ includes a set of nodes of the network. The leaf nodes included in the \textit{cut} of node $v$ are called \textit{leaves}, such that each path from a PI to node $v$ passes through at least one leaf. The node $v$ is called the \textit{root} node of the \textit{cut} C. The cut size is the number of its leaves. A cut is $K$-feasible if the number of leaves in the cut does not exceed $K$.}
%called leaves, such that each path from a PI to n passes through at least one leaf. Node n is called root of cut C. The cut size is the number of its leaves. A trivial cut of the node is the cut composed of the node itself. A cut is K-feasible if the number of nodes in the cut does not exceed K. A cut is said to be dominated if there is another cut of the same node, which is contained, set-theoretically, in the given cut. The volume of a cut is the total number of nodes encountered on all paths between node n and the cut leaves.
The logic optimization of Boolean networks can be conducted with the AIGs efficiently~\cite{hosny2020drills, yu2018developing} based on the Boolean algebra enabled logic transformations. 



%The AIG-based optimization process in the single traversal of the graph usually involves two steps: \textbf{(1)} \textit{transformability check} -- check the transformability w.r.t the optimization operation for the current node; \textbf{(2)} \textit{graph updates} {(\texttt{Dec\_GraphUpdateNetwork} in ABC)} -- apply the applicable optimization operation at the node to realize the transformation and update the graph for the next unseen node. %\cy{I think we could link these two steps with pseduo code syntax that is used in our Algs 1 and 2, e.g., \texttt{Dec\_GraphUpdateNetwork}}



\subsection{DAG-Aware Logic Synthesis}
\label{sec:background_DAG_syn}


To minimize logic complexity and size, subsequently leading to enhanced performance, DAG-aware logic optimization approaches leverage Boolean algebra at direct-acyclic-graph (DAG) logic representations, aiming to minimize area, power, delay, etc., while preserving the original functionality of the circuit. 


This is achieved through the application of various technology-independent optimization techniques and algorithms, such as node rewriting, structural hashing, and refactoring. In this work, we focus specifically on exploring DAG-aware logic synthesis using And-Inverter Graphs (AIGs) representations. 
{The AIG-based optimization process, during a single traversal of the logic graph, typically involves two steps: \textbf{(1)} \textit{transformability check} -- checking the transformability of the optimization operation for the logic cut in relation to the current node; \textbf{(2)} \textit{graph updates} -- if the optimization is applicable, the optimization operation is applied at the node to realize the transformation of the logic cut and subsequently update the graph.}

\noindent
\textbf{Rewriting~\cite{mishchenko2006dag}}, denoted as \texttt{rw}, {is a fast greedy algorithm for logic optimization.} {It iteratively selects an AIG logic cut with the current node as the root node and replaces the selected subgraph with the same functional pre-computed subgraph (NPN-equivalent) of a smaller size to realize the graph size optimization. In the default settings in ABC, the target logic cuts for each node are 4-feasible cuts. For AIG rewriting, all 4-feasible cuts of the nodes are pre-computed using the fast cut enumeration procedure. In each iteration, the Boolean function for the current logic cut is computed and its NPN-class is determined by hash-table lookup.
After trying all available subgraphs, the one that leads to the largest improvement at a node is used.}
For instance, Figure \ref{fig:aig_rw} illustrates the optimization of the original graph shown in Figure \ref{fig:aig_ori} using \texttt{rw}. The algorithm traverses each node in topological order, checking the transformability of its cut with \textit{rewriting}. In Figure \ref{fig:aig_rw}, node $k=efr$ is optimized using \texttt{rw}, resulting in a reduction of 2 nodes for the logic optimization.

\noindent
\textbf{Refactoring~\cite{mishchenko2006dag}}, denoted as \texttt{rf}, is a variation of the AIG \textit{rewriting} using a heuristic algorithm to produce a larger cut for each AIG node. Refactoring optimizes AIGs by replacing the current AIG structure with a factored form of the cut function.
For example, Figure \ref{fig:aig_rf} illustrates the optimization of the original AIG with \texttt{rf}. {Node $g$ is optimized to the factored form of $g=ac(\overline{n} + a)$ and the node $w$ is optimized to $w=qo({u} + {h})$}. As a result, the optimized graph with \texttt{rf} has a graph size of $23$ with $2$ nodes reduction.



\noindent
\textbf{Resubstitution~\cite{brayton2006scalable}}, denoted as \texttt{rs}, optimizes the AIG by replacing the function of a node with functions of other existing nodes, referred as {divisors}, within the graph. This approach aims to eliminate redundant nodes unnecessary for expressing the function of the current node. {In \textit{resubstitution}, cuts containing no more than 12-16 leaves are considered, and the optimization is performed using explicitly computed truth tables and exhaustive simulation. During \textit{resubstitution}, the introduction of new nodes may occur to complete the functionality in the AIG, which is a process known as $k$-resubstitution (where $k$ represents the number of newly introduced nodes) and $k$ should not exceed the number of nodes saved by the optimization. In the default settings of ABC, $k$-resubstitution is checked for $k=\{0, 1, 2, 3\}$, and the number of divisors in each cut is limited to $150$.}
For example, in Figure \ref{fig:aig_ori}, the node $g=a\overline{p}$, with $p=\overline{m}\overline{d}$, ${d}=\overline{a}{c}$, and $m=abc$, implies $g=abc$. This condition allows for resubstitution with node $m$, leading to the removal of nodes $g, p,$ and $d$ from the graph, as depicted in Figure \ref{fig:aig_rs}. Consequently, \texttt{rs} optimizes the original AIG by reducing the graph size through the removal of $3$ nodes.


\noindent
{\textbf{Definition 1: \textit{Stand-alone} Logic Optimization}: Stand-alone logic optimization refers to the process of optimizing the logic graph using a single pre-set optimization criterion during the single traversal of the entire graph.}
{\textbf{Example 1:} The existing optimizations, such as structural \textit{rewriting}, \textit{refactoring}, and \textit{resubstitution}, are stand-alone optimizations as they only assess the transformability with respect to a single pre-set operation and update the graph based on the corresponding optimization criterion.
}




==> TCAD24-Orch/3_approach.tex <==
\section{Approach}
\label{sec:approach}

\input{figs/analysis_figure}
\input{TCAD24-Orch/figs/venn}

{In existing logic optimization algorithms that follow a stand-alone optimization approach as shown in Figure \ref{fig:aig_alone}, certain nodes may miss optimization opportunities. For instance, node $g$, which is suitable for both \textit{refactoring} and \textit{resubstitution}, may be overlooked for optimizations in \textit{rewriting}.}
{To further enhance the logic optimization process in DAG-aware logic synthesis, we introduce "\textit{Orchestration}" for logic optimization in this work. This approach is in contrast to \textit{Stand-alone Logic Optimization} defined in Definition 1. We provide the details of \textit{Orchestrated Logic Optimization} in Definition 2.}


\noindent
{
\textbf{Definition 2: \textit{Orchestrated} Logic Optimization:} Orchestrated logic optimization involves multiple optimization operations being considered during a single traversal of the logic graph. {In each optimization iteration, multiple operations can be evaluated and applied based on the predefined orchestration criteria.}}

{In the orchestration optimization, multiple optimizations are made available for each node, thereby maximizing its optimization opportunities. Specifically, we orchestrate optimization operations including \textit{rewriting} (\texttt{rw}), \textit{resubstitution} (\texttt{rs}), and \textit{refactoring} (\texttt{rf}), in a single traversal of the AIG for the logic optimization. }The orchestration technique can be iteratively applied to the AIG multiple times, in combination with other optimization operations such as \textit{balance}, \textit{redundancy removal} to achieve iterative DAG optimization. Moreover, the optimized AIG resulting from our orchestration method can be verified for equivalence to the original AIG using Combinatorial Equivalence Checking (CEC). 

In this section, we first explore optimization opportunities in the single traversal of AIG for both stand-alone optimizations and orchestrated optimization. We then introduce two orchestration policies: \textit{Local-greedy orchestration}, which selects the operation yielding the highest local gain (i.e., the number of nodes saved by applying the optimization operation) at each node for AIG optimization, and \textit{Priority-ordered orchestration}, which prioritizes operations in a predefined order for AIG optimization at each node. %\yingjie{Finally, we provide an analysis of the runtime costs associated with the orchestration algorithms for logic optimization and compare them with existing stand-alone algorithms.}

\subsection{Optimization Opportunities Studies}
\label{sec:space}

First, we analyze the optimization opportunities in a single traversal of the AIG for various optimization methods. {We record the number of iterations where optimization leads to graph updates, termed as "valid iterations," in this analysis. The results for logic optimizations using \texttt{rw}, \texttt{rs}, \texttt{rf}, and the orchestration method are illustrated in Figure \ref{fig:ana}. The orange bar represents the number of valid iterations with \texttt{rw}, purple for \texttt{rs}, and blue for \texttt{rf}. The bar labeled "Ours" shows the number of valid iterations with the orchestration optimization, incorporating valid iterations from different optimizations (\texttt{rw}, \texttt{rs}, \texttt{rf}), indicated by the corresponding colors within the bar.} For instance, for the design \textit{voter}, stand-alone optimization methods (\texttt{rw}/\texttt{rs}/\texttt{rf}) result in $1917$/$2106$/$738$ valid iterations respectively (Figure \ref{fig:ana_voter}). In contrast, the orchestration method yields $3696$ valid iterations, presenting 93\%, 75\%, and 400\% more valid iterations than the \texttt{rw}, \texttt{rs}, and \texttt{rf} methods, respectively, in a single traversal of the AIG.

{For a better illustration, we present a Venn diagram using design \textit{bfly} in Figure \ref{fig:venn} as a detailed analysis of Figure \ref{fig:bfly_bd}. Here, the orchestration algorithm employed is the \textit{priority-ordered} algorithm with $\widehat{\texttt{O1}}$, which prioritizes \texttt{rw} most, then \texttt{rs} and \texttt{rf} least, and follows the definition in Section \ref{sec: Orchrules}. The diagram in Figure \ref{fig:venn_rw_rs_rf} demonstrates that while there are overlaps between different stand-alone optimizations, most root nodes found are distinct for each method. Additionally, the diagrams in Figure \ref{fig:venn_o1_rw} to \ref{fig:venn_o1_rf} for orchestration optimization and its corresponding stand-alone optimizations highlight unique root nodes in both approaches. It is noteworthy that the ratio of overlap to uniqueness varies with different orchestration algorithms and across designs.}

Our observations from this study highlight two key points: \textbf{(1)} Stand-alone optimization algorithms can miss significant optimization opportunities; \textbf{(2)} Orchestrating multiple optimizations in a single DAG traversal can introduce more optimization opportunities and more efficient logic optimization. %\yingjie{\textbf{(3)} For most designs, a large part of valid iterations with the orchestration optimization is contributed by \texttt{rw} (e.g., for designs \textit{bfly} and \textit{fir}).} 


{Given the context of orchestration, we can define the theoretical solution space and its optimal solution as follows: Consider a combinational And-Inverter Graph (AIG), denoted as \( G(V,E) \). It is postulated that within the entire solution space, which encompasses \( 3^{|V|} \) possibilities, there exists at least one orchestration decision ensuring that \( G(V,E) \) can be minimized to its smallest possible form utilizing a single traversal algorithm. Consequently, the theoretical upper limit for the complexity associated with pinpointing the optimal orchestration solution scales exponentially with the size of the graph, represented by \( |V| \). Nevertheless, within the scope of Boolean minimization, it has been empirically observed that the expansive solution space of \( 3^{|V|} \) may actually equate to a considerably reduced space of quality-of-results, specifically concerning the dimensions of the optimized AIGs. Note the solution space will increase if orchestration elaborates more than three synthesis techniques (i.e., increasing the base of the exponential complexity). This space of results tends to be notably constricted for smaller Boolean networks.}


Thus, to orchestrate multiple optimizations in a single AIG traversal, an effective orchestration policy (heuristic) is essential. In this work, we propose two policies: \textbf{(1) The \textit{Local-greedy orchestration}}, which selects the optimization operation resulting in the highest local gain (node reductions from the logic transformation of the operation) at the node for AIG optimization; and \textbf{(2) The \textit{Priority-ordered orchestration}}, which follows a pre-defined priority order for orchestrating multiple operations, i.e., applying optimizations according to the order. These policies are detailed in Algorithms \ref{alg:local} and \ref{alg:orch}, respectively.




\begin{figure}
\label{fig:aig_orch}
\centering
 \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{TCAD24-Orch/figs/aig_local-crop.pdf}
        \caption{AIG with \texttt{Local-greedy} orchestration}
        \label{fig:aig_local}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{TCAD24-Orch/figs/aig_prio-crop.pdf}
        \caption{AIG with \texttt{Priority-ordered} orchestration}
        \label{fig:aig_pri}
    \end{subfigure}
    \caption{{The optimized graph produced by orchestration optimization operations: (a) optimized AIG with \textit{Local-greedy orchestration}, graph size is 19; (b) optimized AIG with \textit{Priority-ordered orchestration}, graph size is 21.}}
\end{figure}




\subsection{{Algorithm 1: Local-greedy Orchestration}}
The \textit{Local-greedy orchestration} algorithm takes a graph $G(V, E)$ as input, where $V$ represents the set of nodes in the AIG, and $E$ denotes the edges between nodes. Following the topological order, we initially check the transformability of each node with respect to all orchestrated optimization operations, namely \texttt{rw}, \texttt{rs}, and \texttt{rf}. This process yields the corresponding local optimization gains, $G_{rw}$, $G_{rs}$, and $G_{rf}$ (line 2). When none of the operations are applicable to a node, the local gain $G$ is set to $-1$.
{Once the local gains $G_{rw}$, $G_{rs}$, and $G_{rf}$ at the node are determined, the algorithm identifies the optimization operation with the highest non-negative local gain (lines 3, 6, and 9). The operation with the highest gain is then applied, and the graph is updated accordingly (lines 4, 7, and 10). If no operation is applicable (all gains are negative), the node is bypassed for optimization (line 12), and the algorithm proceeds to the next node in the iteration (line 13).}


{Compared to \textit{stand-alone optimizations}, the \textit{Local-greedy} orchestration algorithm incurs additional runtime overhead due to the necessity of pre-computing transformability checks and local gains for all available optimization operations (line 2).}%However, this overhead is offset by the reduced number of required iterations resulting from the effective orchestration of optimizations. This trade-off between overhead and efficiency is further discussed in Section \ref{sec:runtime_result}.}

\input{alg_local}

\noindent
\textbf{Example:} An illustrative example is shown in Figure \ref{fig:aig_local}, based on the original AIG from Figure \ref{fig:aig_ori}. Following the topological order of the AIG, the Primary Inputs (PIs) are bypassed for optimization. Nodes $n$, $m$, $d$, and $p$ are also skipped as none of the optimizations are applicable to them. {The algorithm then evaluates node $g$, checking its transformability with \texttt{rw}, \texttt{rs}, and \texttt{rf}, and determining the local gains as $G_{rw} = -1$, $G_{rs} = 3$, and $G_{rf} = 1$. The \textit{Local-greedy orchestration} algorithm selects the operation with the highest local gain for optimization, in this case, \texttt{rs}. By iteratively traversing the entire logic graph, the \textit{Local-greedy orchestration} algorithm optimizes the AIG with a node reduction of $6$, as depicted in Figure \ref{fig:aig_local}.}


\subsection{{Algorithm 2: Priority-ordered Orchestration}} \label{sec: Orchrules}
In this algorithm, the selection of the optimization operation to be applied at each node depends on a pre-defined priority order with respect to the available optimizations. For the three operations \texttt{rw}, \texttt{rs}, and \texttt{rf}, there are six possible permutations of the priority order, namely: 
$\widehat{\texttt{O1}}$ $\mapsto$ \texttt{rw}$>$\texttt{rs}$>$\texttt{rf}, $\widehat{\texttt{O2}}$ $\mapsto$ \texttt{rw}$>$\texttt{rf}$>$\texttt{rs}, $\widehat{\texttt{O3}}$ $\mapsto$ \texttt{rs}$>$\texttt{rw}$>$\texttt{rf}, $\widehat{\texttt{O4}}$ $\mapsto$ \texttt{rs}$>$\texttt{rf}$>$\texttt{rw}, $\widehat{\texttt{O5}}$ $\mapsto$ \texttt{rf}$>$\texttt{rs}$>$\texttt{rw}, and $\widehat{\texttt{O6}}$ $\mapsto$ \texttt{rf}$>$\texttt{rw}$>$\texttt{rs}. {For instance, the priority order $\widehat{\texttt{O1}}$ implies that \texttt{rw} has the highest priority during optimization, meaning it is checked first for transformability; \texttt{rs} is evaluated next if \texttt{rw} is not applicable to the node; and \texttt{rf} is considered last when the higher priority operations are not applicable.}


%The proposed orchestration implementation is described in Algorithm \ref{alg:orch}. While traversing the AIG, the nodes are visited in topological order (line 1). Given the input AIG $G(V, E)$ and the priority orchestration policy $P_{>}$, where the first position has the highest priority, at the unseen node $v$, the algorithm checks the transformability of the operation at the node following the policy $P_{>}$. When the first priority operation is available, this operation will be selected and applied to update the graph, and the algorithm will move to the next iteration while ignoring transformability checks with other operations (lines 2 -- 4). If the transformability check for the first operation fails at the node, the transformability w.r.t the operation at the second position will be checked for the node. When the second operation is applicable, it will apply the second operation and update the graph accordingly and move to the next iteration (lines 5 -- 7). The algorithm will check the least priority operation when the first two operations are both inapplicable (lines 8 -- 10). When all the operations are checked, and none of them are applicable, the node will be skipped for the optimization, and the algorithm moves to the next iteration without graph updates (lines 11 -- 13). Note that the the leave nodes in the optimized cuts of $v$ are marked as the seen nodes, which are excluded from the successive iterations (line 14). The algorithm completes the optimization for each node in the AIG graph iteratively until no unseen node exists in the updated graph.  

{Algorithm \ref{alg:orch} outlines the implementation of the priority-ordered orchestration for logic graphs. This algorithm takes an AIG $G(V, E)$ and a priority orchestration policy $P_{>}$ as inputs. The policy $P_{>}$ is defined as a precedence-ordered set of operations, wherein the operation positioned first has the highest priority. 
%In each iteration at node $v$, the algorithm assesses the feasibility of performing an operation following the policy $P_{>}$. Upon discovering a viable operation following the priority order, the operation is applied to the current node and update the graph, and the algorithm will exit the current iteration and move to the next iteration without evaluations for other available operations with lower priority. 
{As delineated in Algorithm \ref{alg:orch}, for each node, the algorithm initially examines the transformability of the highest-priority operation, $P_{>}[0]$ (line 2). If $P_{>}[0]$ is applicable, it is applied, and the graph is updated accordingly (line 3). Following this, the algorithm proceeds to the next node without evaluating other lower-priority operations (line 4).
If $P_{>}[0]$ is not applicable, the algorithm assesses the next highest-priority operation, $P_{>}[1]$ (lines 5 -- 7). This process is repeated, methodically evaluating operations in descending order of priority (lines 8 -- 10). In cases where none of the operations in the policy $P_{>}$ are applicable, the node is bypassed in the current iteration, resulting in no modifications to the graph (lines 11 -- 12).}
}

{The selection of the most effective priority order depends heavily on the specific design domain. The initial transformation chosen can significantly impact the optimization process. Operations with higher priority tend to play a more critical role. Furthermore, incorporating domain knowledge into the optimization process can improve performance. Machine learning techniques can be helpful in this regard and exploring their potential leads to more further work.}

% The selection of the most effective priority order requires domain knowledge specific to the design. As noted in \cite{yu2020flowtune}, the first transformation choice significantly impacts the optimization performance. Specifically, the operation assigned the highest priority tends to have a more critical role in the priority-ordered orchestration process. \yingjie{Furthermore, the more specific domain knowledge can be discovered by machine learning with the node-level optimization space~\cite{li2024boolgebra}, where machine learning is implied to produce the node-level optimization decisions for better optimization performance.}

%\yingjie{Furthermore, the orchestration of \texttt{rw}, \texttt{rs}, and \texttt{rf} represents a combination of fine-grained, exact optimization (\texttt{rw}) with heuristic, larger-scope operations (\texttt{rs}, \texttt{rf}). Insights from Section \ref{sec:experiment} suggest that fine-grained operations (\texttt{rw}) are typically favored at higher priorities, while coarser operations like \texttt{rf} are preferred at lower priorities due to their structural transformations on large logic cuts. Additionally, the domain knowledge can be discovered by machine learning algorithms~\cite{}.}


%\yingjie{The \textit{Priority-ordered orchestration} algorithm exhibits a lower runtime cost compared to the \textit{Local-greedy orchestration} algorithm, primarily due to fewer transformability checks necessitated by its pre-defined priority order. Remarkably, this approach also demonstrates a runtime advantage over stand-alone algorithms. This efficiency gain, along with a detailed comparison, is further explored in Section \ref{sec:runtime_result}. }

\input{algorithm}

\noindent
\textbf{Example:} An illustrative example is shown in Figure \ref{fig:aig_pri}, using the original AIG from Figure \ref{fig:aig_ori}. The priority sorting is set as $P_{>}(\texttt{rw}, \texttt{rf}, \texttt{rs})$, corresponding to $\widehat{O2}$. Following the topological order, the PIs and nodes $n$, $m$, $d$, and $p$ are bypassed as none of the optimizations are applicable. For node $g$, the algorithm first checks \texttt{rw} as per the priority order but finds it inapplicable, proceeding then to \texttt{rf}. Since \texttt{rf} is applicable, it is applied to update the AIG (indicated by the blue box), with no need to check the transformability of \texttt{rs}. {The iterative traversal of the entire graph leads to the AIG, optimized via the \textit{Priority-ordered orchestration} algorithm, achieving $4$ node reductions compared to the original graph.}


{These two orchestration algorithms apply stand-alone optimizations within a single AIG traversal, each leveraging distinct strategies. The \textit{Local-greedy orchestration} algorithm selects the most effective operation for logic minimization based on the current local node structure. In contrast, the \textit{Priority-ordered orchestration} algorithm utilizes a variety of pre-defined priority orders, potentially enhancing overall performance. A key distinction lies in their operational approach: the \textit{Local-greedy orchestration} algorithm examines the transformability with respect to all operations at each node, whereas the \textit{Priority-ordered} algorithm progresses to the next node once an applicable operation is found in the given order, effectively minimizing redundant transformability checks. Consequently, in terms of runtime efficiency, the \textit{Local-greedy orchestration} may be less efficient compared to the \textit{Priority-ordered orchestration}. Detailed empirical studies and discussions of these findings are presented in Section \ref{sec:experiment}.}


%\cy{I am thinking about adding a short self-discussion here to quickly discuss the differences between algorithms 1 and 2, which connects to our experimental setups in next section. For example, local greedy with have no problem of exploring any algorithm space (does not have any) but orchestration has. If has options like priority orch, then the flow problem will exsit. anything else?}



%As a result, compared with the stand-alone optimizations produced by ABC in Figure \ref{fig:aig_rw} -- Figure \ref{fig:aig_rs}, the \texttt{orchestration}-optimized graph shown in Figure \ref{fig:aig_orch} shows better logic minimization optimization performance in fewer optimization iterations as shown in Table \ref{tbl:reduce}. With skipped nodes in the stand-alone operations optimized with other orchestrated operations, more nodes within the operation cuts are marked "seen" nodes in each iteration, thus highly reducing the iteration numbers and improving the minimization performance.




==> TCAD24-Orch/4_experiment.tex <==

\input{tbls/table_1o}

\section{Experiments}
\label{sec:experiment}

%We evaluate the performance of the proposed \texttt{orchestration} synthesis in logic minimization and area reduction after post-synthesis technology-mapping, in single traversal optimization, iterative optimization, and synthesis flow settings. 
Our experimental results include comparisons with stand-alone optimizations in ABC, covering: \textbf{(1)} performance and runtime evaluation with single traversal optimization;
%\yingjie{and performance evaluation with single traversal of all available optimizations, where we apply single traversal of graph with each optimization (\texttt{rw}, \texttt{rs}, \texttt{rf}) for sequential optimization compared with the sequential optimization with three times of sequential orchestration optimization}; 
 \textbf{(2)} performance evaluation of optimization methods in iterative synthesis; \textbf{(3)} end-to-end performance evaluation in existing ABC flows \texttt{resyn} by OpenROAD \cite{ajayi2019openroad}, where the orchestration method is integrated into ABC in Yosys \cite{wolf2016yosys} for OpenROAD. OpenROAD reports the performance of area minimization (technology mapping) and post-routing area minimization with respect to different optimization methods. Experimental results are conducted on 104 designs from the ISCAS’85/89/99, VTR\cite{murray2020vtr}, and EPFL\cite{soeken2018epfl} benchmark suites. All experiments are conducted on an Intel Xeon Gold 6230 20x CPU. %Upon analyzing the results shown as follows, the outperformance of orchestration to the original ABC can be assured to a great extent.

%\input{figs/results_1o_plot}

%\subsection{Stand-alone Optimization Evaluations}\label{sec:single_result}

%First, we compare \texttt{orchestration} proposed in Section \ref{sec:approach} with stand-alone optimizations in ABC in single traversal on all 104 designs. The complete results are shown in Figure \ref{fig:1O}, and in each sub-figure, we compare stand-alone optimizations, i.e., \texttt{rw}, \texttt{rs}, \texttt{rf} with our \texttt{orchestration} of different orchestration policies, i.e., $\widehat{\texttt{O1}}$ -- $\widehat{\texttt{O6}}$ defined in Section \ref{sec: Orchrules} on all designs. Note that we use normalized node numbers achieved by stand-alone optimizations as $X-$axis and normalized node numbers achieved by \texttt{orchestration} as $Y-$axis to present all results in one figure due to different design spaces. Expressly, we set the original node number of each design (baseline) to be the upper bound and the minimum node number achieved from all stand-alone optimizations and \texttt{orchestration} as the lower bound. In this paper, the normalized range is set as $\left [ 0,1 \right ]$, such that points falling below (/ above) the diagonal indicate that the selected policy-based \texttt{orchestration} optimization outperforms (/ underperforms) the selected stand-alone optimization. %Due to the normalization strategy, a very small amount of designs with no optimization space to all above mentioned optimizations cannot be shown in the figure. 
%In addition, we introduce \textbf{R} as the ratio of the number of designs on which \texttt{orchestration} outperforms stand-alone optimizations to the number of total tested designs. %In addition, each sub-figure is divided by the diagonal ($x=y$): points falling below the diagonal indicates that the selected policy-based \texttt{orchestration} optimization outperforms the selected stand-alone optimization; points falling above the diagonal indicates that the selected stand-alone operation outperforms the selected policy-based \texttt{orchestration} optimization; for each point falls on the diagonal, both have comparable performance. 
%Thus, we can see that Figure \ref{fig:1O_O1} and Figure \ref{fig:1O_O3} show that $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$, respectively, outperforms stand-alone optimizations on all tested designs, while $\widehat{\texttt{O3}}$ reaches the best performance by presenting more clustered points below the diagonal. Furthermore, we present detailed results of 16 designs in Table \ref{table:1O}. Overall, \texttt{orchestration} with $\widehat{\texttt{O3}}$ shows an average of $4.0\%$ more reduction in graph size compared to the best result achieved by stand-alone optimizations, which sustains the advantage of \texttt{orchestration}. 
% \texttt{O3} obtains the best average node reduction of $17.9\%$ which is an improvement of $4.5\%$ comparing to \texttt{rw} which is the best option from original ABC with a node reduction of $13.4\%$. 
% For example, after applying \texttt{O3} on design voter from EPFL, the node reduction of $31.7\%$ is an improvement of $11.6\%$ comparing to the best result from original ABC which sustains the advantage of orchestration.

%\input{figs/results_3o_plot}
%\input{tbls/table_resyn}
\subsection{{Single Optimization Evaluations}}
\label{sec:single_result}
Initially, we validate the benefits of the orchestration concept in logic optimization for single AIG traversal. Specifically, we compiled optimization results for all 104 designs from various benchmark suites. These results are related to (1) the \textit{stand-alone optimization} methods, namely \texttt{rw}, \texttt{rs}, and \texttt{rf}, and (2) the \textit{orchestration optimization} methods, which include \textit{priority-ordered orchestration} ($\widehat{\texttt{O1}}$ – $\widehat{\texttt{O6}}$) and \textit{local-greedy orchestration} (\texttt{LocalGreedy}). A subset of these results, focusing on large designs, is presented in Table \ref{table:1O}.

The data indicates that the most effective optimization method for all designs consistently originates from one of the \textit{orchestration} methods, exhibiting notable improvements over \textit{stand-alone} optimizations. {Specifically, the best performing \textit{orchestration} algorithm ($\widehat{\texttt{O3}}$) demonstrates an average performance benefit of at least 4.0\% compared to stand-alone methods (specifically \texttt{rw}). Additionally, the table includes the average runtime cost for each optimization, where the orchestrated algorithms with better optimization performance take runtime overhead at the same time. Specifically, it takes more runtime overhead than \texttt{rs} and \texttt{rf} while less than \texttt{rw}. %The orchestration optimization requires more runtime than the stand-alone optimization, with an average runtime overhead of xx\%. 
}
%For example, for the design \texttt{voter}, the best performance produced by orchestration methods ($\widehat{\texttt{O3}}$) is 31.7\% node reduction, while the best node reduction produced by stand-alone methods (\texttt{rs}) is 20.1\%, with 11.6\% less node reduction, which confirms the advantages of implementing the orchestration concept in logic synthesis. 

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.99\textwidth]{TCAD24-Orch/figs/rw.pdf}
        \caption{runtime comparison with \texttt{rw}}
        \label{fig:rt_rw}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.99\textwidth]{TCAD24-Orch/figs/RS.pdf}
        \caption{runtime comparison with \texttt{rs}}
        \label{fig:rt_rs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
\includegraphics[width=0.99\textwidth]{TCAD24-Orch/figs/rf.pdf}
        \caption{runtime comparison with \texttt{rf}}
        \label{fig:rt_rf}
    \end{subfigure}
     
 \caption{Runtime comparison between selected single-traversal \textit{orchestration} policies ($\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{Local-greedy} (labeled as \texttt{LGP})) and \textit{stand-alone} optimizations from ABC: (a) runtime comparison with \texttt{rw}; (b) runtime comparison with \texttt{rs}; (c) runtime comparison with \texttt{rf}.
}
    \label{fig:runtime comparison}
\end{figure*}

\subsection{Single Runtime Evaluations}
\label{sec:runtime_result}

{We also analyze the runtime of the orchestration algorithm \textit{Local-greedy} optimization (\texttt{LGP}) and \textit{Priority-ordered} optimization with $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$. This analysis, including a comparison with stand-alone optimizations (i.e., \texttt{rw}, \texttt{rs}, and \texttt{rf}), is illustrated for all 104 designs in Figure \ref{fig:runtime comparison}. To effectively showcase the runtime variances, the figure employs a logarithmic scale. The x-axis represents the runtime of the stand-alone ABC optimizations, while the y-axis denotes the runtime of the \textit{orchestration} algorithms. The dotted line ($x=y$) acts as a benchmark, where points above this line indicate a higher runtime cost for the \textit{orchestration} algorithm compared to its stand-alone ABC counterpart. Conversely, points below the line suggest a lower runtime cost.} {From the runtime data, we draw two main conclusions: \textbf{(1)} Generally, orchestration algorithms {(with comparable performance, i.e., $\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$ and \texttt{LGP})} have a comparable runtime, with \texttt{LGP} tending to incur a higher runtime overhead than other orchestration methods. \textbf{(2)} Orchestration algorithms exhibit runtime overhead when compared to stand-alone optimizations, their runtime is akin to \texttt{rw} but notably higher than \texttt{rs} and \texttt{rf}.}


{A further analysis of the runtime for each optimization iteration, focusing on different optimization methods, has been conducted. As outlined in Section \ref{sec:background_DAG_syn}, logic optimizations predominantly involve two phases: \textit{transformability check} and \textit{graph update}. \textbf{Firstly}, the transformability check constitutes the bulk of runtime in logic optimizations. \textbf{Secondly}, despite an equal number of total iterations, \texttt{rs} and \texttt{rf} optimizations are quicker than \texttt{rw}, implying that the per iteration runtime cost is lower for \texttt{rs} and \texttt{rf}. %Thus, the runtime for \texttt{rw} iterations will dominate the runtime in orchestration optimizations, resulting in comparable runtime with stand-alone \texttt{rw}. 
\textbf{Thirdly}, a substantial number of iterations are ‘wasted’ with merely performing transformability checks without contributing to graph optimization.
For instance, in Figure \ref{fig:ana}, design \textit{bfly}, the number of valid iterations is $1764$/$1374$/$920$ for \texttt{rw}/\texttt{rs}/\texttt{rf}, which is 6\%/5\%/3\% of total iterations, with 94\%/95\%/97\% iterations are wasted. However, with orchestration algorithms, the number of valid iterations is $2306$, which is 8\% of total iterations with 92\% wasted iterations. Despite the orchestration optimization has a higher percentage of valid iterations, it still incurs runtime overhead due to these wasted iterations. Specifically, in orchestration, nodes in wasted iterations undergo transformability checks for all three optimizations, significantly increasing the runtime. Particularly, \textit{Local-greedy} orchestration suffers the most as it requires transformability checks for all optimizations in every iteration. \textbf{Consequently}, the runtime inefficiency in orchestration algorithms is mainly due to the substantial number of wasted iterations involving comprehensive transformability checks. The per iteration runtime is heavily influenced by \texttt{rw} iterations, leading to an overall runtime overhead for orchestration optimizations compared to stand-alone methods, albeit being comparable to \texttt{rw}.}

%\textbf{Third}, lots of iterations with transformablity check are "wasted", i.e., most of the iterations are checked with transformablity but fail in graph optimization. As shown in Figure \ref{fig:ana}, for design \textit{bfly}, the number of valid iterations is $1764$/$1374$/$920$ for \texttt{rw}/\texttt{rs}/\texttt{rf}, which is 6\%/5\%/3\% of total iterations. However, with orchestration algorithms, the number of valid iterations is $2306$, which is 8\% of total iterations. However, even with the improved iteration efficiency with more valid iterations, the runtime performance is worse for orchestration algorithms due to the large number of wasted iterations. Specifically, the nodes in wasted iterations in orchestration optimizations will check the transformablity with all three optimizations, which takes the most runtime and results in runtime overhead than stand-alone optimizations. Moreover, \textit{Local-greedy} orchestration performs with worse runtime as all iterations are checked the transformability w.r.t all optimizations. \textbf{As a result}, the runtime for orchestration algorithms is dominated by the wasted iterations that checks the transformability with all three optimizations, and the runtime per iteration is dominated by \texttt{rw} iterations, resulting in the runtime overhead in orchestration optimization compared with stand-alone optimizations, while the runtime is comparable with \texttt{rw}.



%{\color{red}\textbf{As a result}, the key in the orchestration concept is improving the efficiency in finding the "valid iterations" and saving the wasted runtime.}

\iffalse
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.99\textwidth]{TCAD24-Orch/figs/runtime_rw.pdf}
        \caption{runtime comparison with \texttt{rw}}
        \label{fig:rt_rw_pure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.99\textwidth]{TCAD24-Orch/figs/runtime_rs.pdf}
        \caption{runtime comparison with \texttt{rs}}
        \label{fig:rt_rs_pure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
\includegraphics[width=0.99\textwidth]{TCAD24-Orch/figs/runtime_rf.pdf}
        \caption{runtime comparison with \texttt{rf}}
        \label{fig:rt_rf_pure}
    \end{subfigure}
     
 \caption{Runtime comparison between selected single-traversal \texttt{orchestration} policies ($\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{Local-greedy} (labeled as \texttt{LGP})) and stand-alone optimizations from ABC: (a) runtime comparison with \texttt{rw}; (b) runtime comparison with \texttt{rs}; (c) runtime comparison with \texttt{rf}.
}
    \label{fig:runtime comparison_pure}
\end{figure*}
\fi
%\input{tbls/table_runtime}



%\yingjie{\textbf{Therefore, the integration of \texttt{rw}, \texttt{rs}, and \texttt{rf} in a single graph traversal through \textit{orchestration} yields superior AIG optimization performance. This approach incurs a reasonable runtime overhead compared to the conventional stand-alone algorithms. }
% {\color{red}As a result, the orchestration is more compatible as a evaluation backend of machine learning, where we pre-define the operation at node-level in the graph, i.e., pre-define the "valid iterations" and save runtime from wasted iterations.}
%}

% The runtime comparison of all 104 designs from various benchmark suites between $\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{LocalGreedy} with \texttt{rw}, \texttt{rs}, and \texttt{rf}, respectively, is presented in Figure \ref{fig:runtime comparison}. To enhance the clarity of runtime differences, the figure axes are presented in a logarithmic scale. The x-axis represents the stand-alone ABC optimization runtime, while the y-axis represents the \texttt{orchestration} runtime. The dotted line ($x=y$) in the figure is the dividing line for runtime performance, where a point above this line indicates a greater runtime overhead produced by the corresponding \texttt{orchestration} policy compared to the corresponding stand-alone ABC optimization, and a point below this line indicates a smaller runtime overhead produced by the corresponding \texttt{orchestration} policy compared to the corresponding stand-alone ABC optimization. For instance, as shown in Figure \ref{fig:rt_rs}, the majority of blue dots fall above the dotted line, indicating that the \texttt{LocalGreedy} policy induces a higher runtime overhead compared to \texttt{rs} despite providing a greater reduction in nodes.

%A runtime comparison for all 104 designs across diverse benchmark suites between $\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{Local-greedy} (denoted as \texttt{LGP} in Figure \ref{fig:runtime comparison}) as opposed to \texttt{rw}, \texttt{rs}, and \texttt{rf}, respectively, is depicted in Figure \ref{fig:runtime comparison}. To improve the discernibility of runtime discrepancies, the figure's axes employ a logarithmic scale. The x-axis signifies the stand-alone ABC optimization runtime, while the y-axis corresponds to the \texttt{orchestration} runtime. In Figure \ref{fig:runtime comparison}, the dotted line ($x=y$) serves as a demarcation for runtime performance: a point above the line suggests increased runtime overhead generated by the respective \texttt{orchestration} policy in comparison to the corresponding stand-alone ABC optimization, while a point below the line implies reduced runtime overhead. 

%For example, in Figure \ref{fig:rt_rs}, a majority of the blue dots are positioned above the dotted line, denoting that the \texttt{Local-greedy} policy incurs greater runtime overhead relative to \texttt{rs}, despite achieving enhanced node reduction; while the red triangles and green stars, which denotes the runtime for \texttt{Priority} policy with $\widehat{\texttt{O1}}$ and with $\widehat{\texttt{O3}}$, respectively, are mostly below the dotted line, indicating that the \texttt{Priority} policy functions with less runtime compared to \texttt{rs}. Thus, as shown in Figure \ref{fig:runtime comparison}, compared with stand-alone optimizations, i.e, \texttt{rw}, \texttt{rs}, and \texttt{rf}, we find that (1) the \texttt{Local-greedy} orchestration method incurs greater runtime overhead for most designs as it requires the transformability check for all three optimization operations at each node as shown in Algorithm \ref{alg:local}, line 2; (2) the \texttt{Priority} orchestration incurs less runtime overhead than \texttt{Local-greedy} orchestration method and stand-alone optimizations. Compared with \texttt{Local-greedy} orchestration, \texttt{Priority} orchestration conducts significantly less transformability check based on the pre-defined priority order, while compared with stand-alone optimizations, it involves less running iterations as more optimization opportunities lead to more nodes within the optimization cut excluded from the iterations at each applicable optimization operation.

%{To further analyze the runtime differences, we include }Table \ref{table:it_count} that presents the iteration counts of stand-alone ABC optimizations and the best \texttt{Priority} orchestration policy in terms of AIG optimization with selected 16 designs to further evaluate the runtime efficiency. In general, our approach can significantly reduce the iterations required during a single traversal AIG optimization as the AIG structure is much more aggressively optimized when more optimizations are involved, while achieving desirable node reduction performance. For example, when considering the design \texttt{voter}, stand-alone \texttt{rw} achieves a $12.7$\% node reduction, but requires $13,697$ iterations. On the other hand, our approach can achieve a $16.7$\% node reduction with only $3,712$ iterations, resulting in a $72.1$\% reduction in the number of iterations required for the complete AIG optimization.

%However, we find that the ratio of the actual runtime from \texttt{orchestration} policies and stand-alone ABC optimization is not exactly correlated with the ratio of the iteration counts. When considering the iteration number reductions as shown in Table \ref{table:it_count}, the runtime improvements of orchestration policy over stand-alone optimizations are all over 70\%. However, for the actual runtime evaluation in Figure \ref{fig:runtime comparison}, in Figure \ref{fig:rt_rw}, $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$ exhibit an average runtime speedup of over 60\% when compared to \texttt{rw}, while in Figure \ref{fig:rt_rs} and Figure \ref{fig:rt_rf}, the average runtime speedup decrease to only ~30\% when comparing to \texttt{rs} and \texttt{rf}, respectively. As for the \texttt{Local-greedy} policy, it incurs an average of around 48\% extra runtime overhead despite high node reduction performance. This is because, while our methods reduce the iteration counts during AIG optimization, the engineering effort required to implement each \texttt{orchestration} policy must still be considered, which degrades the major strength of iteration reduction.

%\input{figs/results_3o_plot}

\input{TCAD24-Orch/tbls/table_3o_2}

\input{tbls/table_resyn}

%In conclusion, the analysis presented in Section \ref{sec:single_result} and illustrated in Table \ref{table:1O} demonstrates that \texttt{orchestration} policies $\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{Local-greedy} outperform stand-alone optimization strategies from ABC, specifically \texttt{rw}, \texttt{rs}, and \texttt{rf}, in terms of node reduction efficiency. However, as indicated by the runtime comparison depicted in Figure \ref{fig:runtime comparison}, these \texttt{orchestration} policies may introduce varying degrees of runtime overhead. For instance, the \texttt{Local-greedy} policy appears to incur a higher runtime overhead compared to \texttt{rs}, even though it provides more substantial node reduction. This highlights the need for a careful evaluation of the trade-offs between node reduction performance and the potential runtime overheads associated with the implementation of these \texttt{orchestration} policies, in order to make informed decisions for optimal design and engineering outcomes.


\input{tbls/tabel_end-to-end}
\subsection{Iterative Optimization Evaluations}
\label{sec:iterative_result}


It is known that DAG-aware synthesis performs better in iterative transformations. However, considering the runtime for fair comparison, in this iterative optimization evaluation, %we omit the iterative optimization with \textit{Local-greedy} orchestration policy due to its significant runtime overhead even with single traversal optimization as shown in Section \ref{sec:runtime_result}. 
%Therefore, to make fair comparison, 
we compare \textit{priority-ordered orchestration} optimization (e.g., \{$\widehat{\texttt{O1}}$ $\rightarrow$ $\widehat{\texttt{O1}}$ $\rightarrow$ $\widehat{\texttt{O1}}$\}, denoted as Seq($\widehat{\texttt{O1}}$)) to the corresponding stand-alone optimization sequence of the priority order (e.g., correspond to $\widehat{\texttt{O1}}$, the sequence is \{\texttt{rw} $\rightarrow$ \texttt{rs} $\rightarrow$ \texttt{rf}\}, denoted as Seq(ABC)). We use the same notations and perform experiments on other \textit{Priority-ordered} orchestration algorithms. 
{The results of the iterative-traversal with orchestration algorithms and the corresponding sequence of stand-alone optimizations are shown in Table \ref{table:3O}. In all permutations of stand-alone optimization sequences, node reduction performance ranges from 16.9\% to 17.2\%. However, with orchestrated operation sequences, this performance varies between 9.7\% and 18.3\%. In line with single traversal results, sequential optimizations using $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$ surpass their corresponding stand-alone sequences by 1.1\% and 1.4\% respectively.}
%Based on results shown in Section \ref{sec:single_result} that demonstrates $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$ are the best among \texttt{Priority} {orchestration} policies, we keep only these two priority order policies for experiments beyond this point. 

%Figure \ref{fig:3O} includes the results from the experiments mentioned above. Note that we only crop range $\left [0, 0.20\right]$, since iterative optimization significantly reduces the AIG size, to show the most clustered part. {We set \textbf{R} as the ratio of the number of designs on which Seq($\widehat{\texttt{O1}}$) and Seq($\widehat{\texttt{O3}}$) outperform Seq(ABC) to the number of total tested designs. Overall, both Seq($\widehat{\texttt{O1}}$) and Seq($\widehat{\texttt{O3}}$) outperform corresponded Seq(ABC) on more than $93\%$ of the benchmarks.} 

{Furthermore, we evaluate the performance of the orchestration methods when combined with other orthogonal optimizations in a sequential synthesis flow. Specifically, we evaluate the \textit{orchestration} algorithm in \texttt{resyn} and \texttt{resyn3} in ABC. The original flow involves iterative transformations such as \textit{rewriting} (\texttt{rw}), \textit{resubstitution} (\texttt{rs}), \textit{refactoring} (\texttt{rf}), and \textit{balance} (\texttt{b}). The zero-cost replacement enabled \texttt{rw}, \texttt{rs}, and \texttt{rf} are denoted as \texttt{rwz}, \texttt{rsz}, and \texttt{rfz}, respectively. Similarly for the zero-cost replacement enabled orchestration algorithms are denoted as \texttt{Z1} to \texttt{Z6}.
The optimization flow in \texttt{resyn} is \{\texttt{b};\texttt{rw};\texttt{rwz};\texttt{b};\texttt{rwz};\texttt{b}\}; the flow of \texttt{resyn3} is \{\texttt{b};\texttt{rs};\texttt{rs -K 6};\texttt{b};\texttt{rsz};\texttt{rsz -K 6};\texttt{b};\texttt{rsz -K 5};\texttt{b}\}.
We follow the permutation of the original flows by replacing the stand-alone optimization with orchestration optimizations to compose {orchestration} flows. 
We name the resyn flow where \texttt{rw}/\texttt{rwz} is replaced with $\widehat{\texttt{O1}}$/$\widehat{\texttt{Z1}}$ (because \texttt{rw} has the highest priority in $\widehat{\texttt{O1}}$) as \texttt{O-resyn}, the resyn3 flow where \texttt{rs} is replaced with $\widehat{\texttt{O3}}$ (because \texttt{rs} has the highest priority in $\widehat{\texttt{O3}}$) as \texttt{O-resyn3}, and the resyn/resyn3 flow where \texttt{rw}(\texttt{rwz})/\texttt{rs} is replaced with \texttt{Local-greedy}(\texttt{Local-greedy-z}) as \texttt{LGP-resyn}/\texttt{LGP-resyn3}. 

Table \ref{table:resyn} shows the AIG optimization results of 16 designs. Upon comparing the average node reduction of each optimization option, we can observe a consistent improvement with orchestration synthesis flows. Specifically, ${\texttt{O}}$\texttt{-resyn} and ${\texttt{LGP}}$\texttt{-resyn} outperforms \texttt{resyn} by 3.5\% and 4.7\% more average node reductions, respectively; and ${\texttt{O}}$\texttt{-resyn3} and ${\texttt{LGP}}$\texttt{-resyn3} with 10.8\% and 11.5\% more average node reductions than \texttt{resyn3}.}

%We conduct the logic synthesis with three resyn flow on all 104 design and present the results for 7 designs in the first three columns in Table \ref{tbl:resyn_openroad}. Both orchestration flows, i.e., \texttt{O-resyn} and \texttt{LGP-resyn}, consistently outperform the original \texttt{resyn} for all designs. For most designs (6/7), the \texttt{O-resyn} can slightly outperform \texttt{LGP-resyn}. The observations further confirm the advantages of implementing orchestration in logic synthesis for iterative optimizations and combined optimizations with other optimization methods.

%\input{tbls/table_resyn_map}



%\vspace{-3mm}
\subsection{End-to-end Evaluations}
\label{sec:eval_openroad}
Finally, we integrate our proposed orchestration optimization methods into the end-to-end design framework OpenROAD (Open Resilient Design for Autonomous Systems) \cite{ajayi2019openroad} to evaluate the end-to-end performance by the orchestration improved logic synthesis.
{OpenROAD \cite{ajayi2019openroad} Project is an open-source project aiming at developing a comprehensive, end-to-end, automated IC (Integrated Circuit) design flow that supports a wide range of design styles and technology nodes. It integrates various open-source tools to streamline chip development. The flow begins with RTL synthesis, where Yosys \cite{wolf2016yosys} converts high-level RTL descriptions into gate-level netlists and performs logic synthesis and technology mapping via ABC \cite{mishchenko2007abc}. As shown in Figure \ref{fig:openroad_frame}, this is the specific integration where we deploy our proposed orchestration methods in ABC in the end-to-end design flow (the dash line box). Next, the OpenROAD flow performs floorplanning, placement, and global routing. Tools such as RePlAce, TritonRoute, and FastRoute are used for these tasks, respectively. Afterward, detailed routing and signoff checks are completed, using tools like OpenROAD's built-in router and Magic.}

%To make fair comparisons, we follow the permutation of the original flows by replacing \texttt{rw} with $\widehat{\texttt{O1}}$ or \texttt{LocalGreedy} to compose \texttt{orchestration} flows, namely \texttt{O-resyn}. For instance, $\widehat{\texttt{O1}}$\texttt{-resyn} comprises \{\texttt{balance} $\rightarrow$ $\widehat{\texttt{O1}}$ $\rightarrow$ $\widehat{\texttt{O1}}$ $\rightarrow$ \texttt{balance} $\rightarrow$ $\widehat{\texttt{O1}}$ $\rightarrow$ \texttt{balance}\}. Table \ref{table:resyn} shows the AIG optimization results of 16 designs. Upon comparing the average node reduction of each optimization option, we can observe a consistent improvement with \texttt{O-resyn}. Specifically, $\widehat{\texttt{O1}}$\texttt{-resyn} and $\widehat{\texttt{O3}}$\texttt{-resyn} outperforms \texttt{resyn} by 4.4\% and 4.0\% more average node reductions, respectively; and $\widehat{\texttt{O1}}$\texttt{-resyn3} and $\widehat{\texttt{O3}}$\texttt{-resyn3} with 10.7\% and 10.8\% more average node reductions than \texttt{resyn3}. 


\subsubsection{Technology Mapping}
\label{sec:eval_map}

We have implemented AIG technology mapping for standard cells using the 45nm Nangate library \cite{knudsen2008nangate} and applied \texttt{resyn}, \texttt{O-resyn}, and \texttt{LGP-resyn} across all 104 designs in a consistent environment. Selected results for 7 detailed cases are presented in Table \ref{tbl:resyn_openroad} (columns 5 – 7), with the technology mapping outcomes reported by Yosys in OpenROAD. Generally, flows incorporating orchestration optimizations tend to yield better area minimization, averaging 2.2\% more area reduction. This suggests the potential of integrating \textit{orchestration} into existing synthesis flows for enhanced technology mapping performance. However, an exception is observed in the case of \textit{s35932}, where although orchestration-enhanced \texttt{resyn} flows surpass the original \texttt{resyn} in AIG reduction, they result in larger areas post-technology mapping.

Furthermore, a comparison between the post-technology mapping results and those from logic synthesis reveals that the benefits gained from orchestration methods during logic synthesis can diminish, disappear, or even turn into drawbacks after technology mapping. This discrepancy likely arises from the misalignment between technology-independent logic synthesis and technology-dependent mapping cost models, attributable to the high-level abstractions involved at the logic level.%, which introduces us to go further in exploring the miscorrelations in the successive stages. 

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figs/openroad-crop.pdf}
    \caption{The OpenROAD framework integrated with proposed orchestration methods. The dash line blue box shows the details in logic synthesis where the original ABC is replaced with our proposed orchestration optimization implemented ABC.  }
    \label{fig:openroad_frame}
\end{figure}


\subsubsection{Post-Routing}

Furthermore, we carry out post-routing evaluations in OpenROAD, applying the three \texttt{resyn} flows to various designs. The results, detailed in the last three columns of Table \ref{tbl:resyn_openroad}, indicate that the orchestration-enhanced flows (\texttt{O-resyn} and \texttt{LGP-resyn}) generally maintain superiority over the original \texttt{resyn} across most designs. However, the margin of this superiority is reduced when compared to the gains observed in logic synthesis. For instance, in the case of the design \textit{b21}, the \texttt{LGP-resyn} flow demonstrates a 6.2\% improvement in AIG reduction, but this advantage is reduced to 2.7\% in terms of area minimization following post-routing. A notable exception is observed in the design \textit{s35932}, where, despite a 4.8\% improvement in AIG reduction with orchestration methods, the post-routing area minimization performance degrades. This trend, similar to what was observed in technology mapping, underscores the potential misalignments between the benefits achieved during technology-independent logic synthesis and the outcomes post technology-dependent mapping and routing stages. 
%In conclusion, although the performance after post-routing correlates poorly with the performance after logic synthesis, it correlates well with that after technology mapping, which motivates us for implementing technology-aware logic synthesis in the futher works. 

In conclusion, our study reveals a modest correlation between the improvements achieved in logic optimization and the enhancements in post-routing performance. However, there is a more pronounced connection between the results following technology mapping and those observed in the post-routing stage. This finding motivates the focus of our future research on developing technology-aware logic synthesis approaches, aiming to align more closely with the subsequent stages of technology mapping and routing, thereby enhancing the overall design efficiency.

==> TCAD24-Orch/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we propose a novel concept in logic synthesis development -- DAG-aware synthesis \textit{orchestration}, which encompasses multiple optimization operations within a single AIG traversal. 
The proposed concept is implemented in ABC, orchestrating the pre-exisiting stand-alone optimizations, namely \textit{rewriting}, \textit{resubstitution}, \textit{refactoring} for fine-grained node-level logic optimization within a single AIG traversal. Specifically, we provide two algorithms for this \textit{orchestration} process: (1) The \textit{Local-greedy orchestration} algorithm, which selects the optimization operation offering the highest local gain at each node for AIG optimization; (2) The \textit{Priority-ordered orchestration} algorithm, which employs a predefined priority order to select the optimization operation at each node.
Our implementations have been rigorously tested on 104 designs from benchmark suites such as ISCA'85/89/99, VTR, and EPFL. {In comparison to conventional stand-alone optimizations, our \textit{orchestration} optimization achieves superior performance with a reasonable runtime overhead during single graph traversal. Additionally, this optimization maintains its performance benefits in iterative optimizations and integrated design flows, such as \texttt{resyn}, when combined with other optimizations like \textit{balance}. Notably, when implemented within an end-to-end design flow, the orchestration algorithm surpasses stand-alone optimizations in technology mapping and post-routing for the majority of designs. However, it is important to note the observed discrepancies between technology-independent stages (e.g., logic synthesis) and technology-dependent stages (e.g., technology mapping and post-routing). These observations have spurred our interest in future research, specifically aiming to develop end-to-end aware DAG-aware synthesis \textit{orchestrations} that address these optimization miscorrelations.}




==> TCAD24-Orch/alg_local.tex <==
\begin{algorithm}
\caption{Local-greedy Orchestration}   
\footnotesize
\label{alg:local}
 
   \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}
    \KwIn{~$G(V,E) \leftarrow$ Boolean Networks/Circuits in AIG} 
    \KwOut{~Post-optimized AIG $G(V,E)$}
 \For{$v \in V$ in topological order}{
 %\tcp{New order}
       check transformability of $v$ w.r.t orchestrated operations: \texttt{rw}, \texttt{rs}, \texttt{rf}, and get the corresponding optimization gain: \texttt{G$_{rw}^{v}$}, \texttt{G$_{rs}^{v}$}, \texttt{G$_{rf}^{v}$}.
        \tcp*[f]{if operation is not applicable, $G$ is $-1$; otherwise, $G$ is a non-negative number.}

  \uIf{\texttt{G$_{rw}^{v}$} $\geq$ 0 and \texttt{G$_{rw}^{v}$} $\geq$ \texttt{G$_{rs}^{v}$} and \texttt{G$_{rw}^{v}$} $\geq$ \texttt{G$_{rf}^{v}$} }{
  Apply ${rw}$ to $v$ and update $G(V,E)$ \\ %$ \leftarrow$ \texttt{Dec\_GraphUpdateNetwork} \\
        continue
     \tcp*[f]{\texttt{rw} with the highest gain}
         }
  \uElseIf{\texttt{G$_{rs}^{v}$} $\geq$ 0 and \texttt{G$_{rs}^{v}$} $\geq$ \texttt{G$_{rw}^{v}$} and \texttt{G$_{rs}^{v}$} $\geq$ \texttt{G$_{rf}^{v}$} }{
  Apply ${rs}$ to $v$ and update $G(V,E)$ \\ %$ \leftarrow$ \texttt{Dec\_GraphUpdateNetwork} \\   
        continue
     \tcp*[f]{\texttt{rs} with the highest gain}
  }
  \uElseIf{\texttt{G$_{rf}^{v}$} $\geq$ 0 and \texttt{G$_{rf}^{v}$} $\geq$ \texttt{G$_{rw}^{v}$} and \texttt{G$_{rf}^{v}$} $\geq$ \texttt{G$_{rs}^{v}$} }{
  Apply ${rf}$ to $v$ and update $G(V,E)$ \\ %$ \leftarrow$ \texttt{Dec\_GraphUpdateNetwork} \\
        continue
     \tcp*[f]{\texttt{rf} with the highest gain}
  }
  \Else{
          %Update $G(V,E)$ \\ %$\leftarrow$ \texttt{Dec\_GraphUpdateNetwork} \\
    continue 
  }
  }

\end{algorithm}



==> TCAD24-Orch/algorithm.tex <==
 

\begin{algorithm}
\caption{Priority-ordered orchestration}   
%\begin{algorithmic} %\begin{algorithmic}[1]
%\vspace{-2mm}
\footnotesize
\label{alg:orch}
 
   \SetKwInOut{KwIn}{Input}
     \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}
    \KwIn{~$G(V,E) \leftarrow$ Boolean Networks/Circuits in AIG} 
    \KwIn{~Orchestration rule: $\mathcal{P}_>$(\texttt{rw, rf, rs}) }
    \tcp{$\mathcal{P}_>$ is a list as the permutation of the available Boolean transformations.}
    \KwOut{~Post-optimized AIG $G(V,E)$}
 \For{$v \in V$ in topological order}{
 %\tcp{New order}
  \uIf{v \text{is transformable w.r.t} $\mathcal{P}_>$[0]}{
        Apply ${\mathcal{P}_>[0]}$ to $v$ and update $G(V,E) $\\%$ \leftarrow$ \texttt{Dec\_GraphUpdateNetwork} \\
        continue
     \tcp*[f]{check first priority}
         }
  \uElseIf{v \text{is transformable w.r.t} $\mathcal{P}_>$[1]}{
        Apply ${\mathcal{P}_>[1]}$ to $v$ and update $G(V,E)$\\%$ \leftarrow$ \texttt{Dec\_GraphUpdateNetwork} \\
        continue
     \tcp*[f]{check second priority}
  }
  \uElseIf{v \text{is transformable w.r.t} $\mathcal{P}_>$[2]}{
        Apply ${\mathcal{P}_>[2]}$ to $v$ and update $G(V,E) $\\%$ \leftarrow$ \texttt{Dec\_GraphUpdateNetwork} \\
        continue
     \tcp*[f]{check third priority}
  }
  \Else{
    %Update $G(V,E) \leftarrow$ \texttt{Dec\_GraphUpdateNetwork} \\
    continue 
  }
  %Update $G(V,E) \leftarrow$ \texttt{Dec\_GraphUpdateNetwork}, and exclude $v$ from $V$
  }
%  \end{algorithmic}
\end{algorithm}

  




\iffalse
\begin{algorithm}
\caption{Pseudo-code for synthesis orchestration}\label{alg:orch}
\textbf{procedure} DAG-Aware Synthesis Orchestration()\\
$G(V, E)$ $\leftarrow$ Boolean Circuits/Network to AIG \\
\For{v $\in$ V } %\COMMENT{this is a comment}
{    
   \texttt{valid\_ops}=\{ \}; $\leftarrow$ applicable operations for the node \\
   check transformability for all \textit{rw}, \textit{rs}, \textit{rf} statically; \\
   collect transformable nodes in \texttt{valid\_ops}; \\
   pick the operation based on the priority sorting \texttt{orch}; \\
   %select_operation(v) = orch(valid\_ops);\\
    \If{transformable(v)}
    {
        apply transformation to $v$;
    }
    update G(V, E)
}
\end{algorithm}
\fi 

==> TCAD24-Orch/approach.tex <==
\section{Approach}\label{sec:approach}

\subsection{On the Impact of DAG-Aware Synthesis Algorithms}\label{sec:algorithm}

The most efficient algorithms that optimize the Boolean networks are directed acyclic graph (DAG) aware based Boolean synthesis algorithms \cite{mishchenko:2006-dag,wolf2016yosys}, which are widely used in both open-source tools \cite{mishchenko2010abc,wolf2016yosys,luu2014vtr, neto2019lsoracle} and industrial tools \cite{cunxiyu:dac16,stok1996booledozer,DBLP:conf/iccad/YuCSC17,amaru2014majority}. Specifically, this work focuses on optimizing the synthesis flows that comprise DAG-aware synthesis algorithms and heuristics, targeting AIG- and MIG-based flows. Thus, to understand how effective each synthesis transformation (algorithm) is in the synthesis flows, we analyze the basic graph operations in DAG-aware algorithms. We showcase the number of transformed nodes for an AIG-based flow, running 6 different transformations  {(bracket 4 in the pseudo-code of the Algorithm presented in Fig. \ref{fig:motivation})}. With that, we can estimate the effectiveness of the algorithm for a given DAG (a circuit). Hence, to understand how effective each synthesis transformation (algorithm) is in the synthesis flows, we monitor the number of transformed nodes of all transformations using 100 random flows. The selected ABC synthesis transformations are the same six transformations as in \cite{DBLP:conf/dac/YuXM18,hosny2019drills}, namely $\mathbb{S}$=\{balance, restructure, rewrite, refactor, rewrite -z, refactor -z\}. We collect these results for six VTR benchmarks, as shown in Table \ref{tbl:benchmark}, and plot the average, max, min number of relative transformable nodes. While we plot the average over six designs, we observed a similar trend in all the designs. 

The analysis results are shown in Figure \ref{fig:motivation}, where the y-axis represents the relative number of transformed nodes of each transformation, and the x-axis shows the steps of the synthesis flows. For example, given a random \textit{none}-repetition flow composed by the transformations available in $\mathbb{S}$, assume the first transformation is applied to $\sim$1,000 nodes in the {original} graph and the second transformation is applied to $\sim$200 nodes in the {updated} graph. In which case, the relative percentage of the first two transformations of this example is denoted as $1$ and $0.2$. Therefore, in Figure \ref{fig:motivation}, the relative number of transformed nodes of all randoms flows start with $1$. As there are 100 random permuted flows for six designs in this analysis, the error-bars are used to indicate the upper/lower bound of transformable nodes among all the random generated flows. MIG-based transformations have a similar trend, with a particularity: the number of relative transformable nodes for the first two transformations tend to be closer. {Our intuition is that the input for MIG-based synthesis is an AIG data structure, where the nodes have at least one input as constant (true or false)}. Thus, it limits the number of applicable MIG-based transformations on the first iteration. On the other hand, the second iteration has more majority nodes, so there are still a good amount of transformable nodes for MIG-based algorithms. Thus, the observations done for AIGs also hold for MIGs. 


\begin{figure}[t]
\begin{minipage}{.24\textwidth}
\scriptsize
%\captionof{algorithm}{Euclids algorithm}\label{myalg}
\begin{algorithmic}[1]
 \Procedure{dag-aware synthesis}\;\\
  $G(\mathcal{V},\mathcal{E})$ $\gets$ circuit\;\\
 \For{$v \in \mathcal{V}$}{
 \If{\color{red} transformable($v$)}{
  {\color{red} apply transformation to $v$}\; \\
  update $G(\mathcal{V},\mathcal{E})$\;
  }
 }
 %\EndFor
 %\EndIf
 \EndProcedure
\end{algorithmic}
\end{minipage}%
\begin{minipage}{.25\textwidth}
 \centering
\includegraphics[width=1\textwidth]{./figs/motivation.pdf}
\end{minipage}
\caption{Illustration of DAG-aware synthesis algorithm. And, the {relative number} of AIG nodes that are effectively executed in each transformation of the synthesis flows, using 100 random flows with six transformations used in \cite{DBLP:conf/dac/YuXM18,hosny2019drills}.}
\label{fig:motivation}
\end{figure}

There are two important observations can be concluded empirically from the experiments: 

\begin{itemize}

\item Observation (1) \textit{The earlier transformations selected in a given synthesis flow have the highest impacts to the Boolean optimization problem w.r.t DAG-aware logic transformations.}

\end{itemize}

In Figure \ref{fig:motivation}, we can see that for any random flow, the third to sixth transformations in the flow are applied to less than 10\% nodes compared to the first transformation. In this particular example, we observe many cases that the fifth and sixth transformations do not detect any transformable node, regardless of the permutations. 

\begin{itemize}

\item Observation (2) \textit{Earlier transformations in the synthesis flow dominates the performance of Boolean optimizations since the transformable nodes for the rest of the flow are determined by earlier transformations (local minima).}

\end{itemize}

That being said, starting a synthesis flow with an unsuccessful transformation will almost certainly result in an inefficient flow, regardless of how the other optimizations are permuted. This is also true for MIGs, because the first transformation sets the topology of the real MIG graph, influencing the efficacy of subsequent MIG-based transformations. As a result, having the first transformation bias the flow is equivalent to solving a non-convex optimization problem with an initialization that always converges at a suboptimal local optimum. We may conclude from the suggested experiment that the performance of synthesis flows for DAG-based transformations is dominated by the first transformation in the flow. With these two observations in mind, we propose a domain-knowledge MAB approach for automatic logic synthesis flow generation. 

% The main reason is that the DAG-aware synthesis algorithms are mostly implemented based on structural search. The performance of such algorithms heavily relies on the structure of a given DAG. As indicated in the first observation, the structure of the graph will be dominated by the first transformation. Thus, we can say that the first transformation in the flow dominates the performance of synthesis flows. With these two observations in mind, we propose a domain-knowledge Multi-Armed Bandits (MAB) approach for automatic logic synthesis flow generation. 

\noindent
\textbf{Example 1:} An illustrative example that demonstrates the importance of the extracted algorithmic domain knowledge presented in Figure \ref{fig:motivation} is shown in Table \ref{tbl:ex1}. Two DAG-aware synthesis transformations from ABC are selected to build two different flows $F_0$ and $F_1$ and are applied to design \texttt{bfly} from VTR \cite{luu2014vtr} benchmark. We focus on comparing the transformed AIG nodes (\#TNodes) of \texttt{rewrite} and the final number of AIG nodes. This is because \texttt{rewrite} performs a technology-independent rewriting algorithm of AIG, which offers the main reductions of \#AIG in this example. We can see that \textbf{(1)} \textit{The transformations at the early stage of the flows have more impacts than the transformations at the late stage.} For example, in both flows, first \texttt{rewrite} successfully applies to more than 7$\times$ \#AIG than the second \texttt{rewrite}. \textbf{(2)} \textit{The choice of early transformations has significant impacts on the performance of the flow}. Early transformations have more impacts on the Boolean network, so the DAG structure could change dramatically at the early stage compared to the late stage. For example, if we apply \texttt{balance} first, the first \texttt{rewrite} in $F_0$ applies to 951 nodes. On the other hand, without \texttt{balance}, the first  \texttt{rewrite} can be applied to 1764 nodes at ($F_1$). Similar results can be observed from the remaining two \texttt{rewrite}.

\begin{table}[t]
\caption{Example of the algorithmic domain knowledge presented in Figure \ref{fig:motivation} using ABC synthesis transformation \textit{rewrite} rw and \textit{balance} (b) with design {bfly} from VTR 8.0 \cite{luu2014vtr} benchmark. Note that rw is technology-independent rewriting of the AIG which offers the main AIG reductions in $F_0$ and $F_1$. \#TNodes = Number of AIG nodes transformed by the corresponding AIG transformation.}
\begin{tabular}{cccccccc}
\textit{$F_0$} & \textit{b} & \textit{rw} & \textit{b} & \textit{rw} & \textit{b} & \textit{rw} & Final \#AIG \\
\textit{\#TNodes} & 817 & \textbf{951} & 825 & \textbf{169} & 831 & \textbf{64} & 26339 \\ \hline\hline
\textit{$F_1$} & \textit{rw} & \textit{b} & \textit{rw} & \textit{b} & \textit{rw} & \textit{b} & Final \#AIG \\
\textit{\#TNodes} & \textbf{1764} & 824 & \textbf{290} & 834 & \textbf{90} & 832 & \textbf{26182}
\end{tabular}
\label{tbl:ex1}
\end{table}

\noindent
\textbf{Example 2:} Now, we show the importance of getting the right transformation for MIG-based synthesis, according to our discussion on MIG-based synthesis trends in Figure \ref{fig:motivation}. The experiment is depicted in Table \ref{tbl:ex2}. 
We select two area-oriented (nodes reduction) transformation to this end, so we aim to highlight the effectiveness of picking a right transformation at the 1st iteration to the overall circuit area (DAG size) reduction. 
Similarly to the previous example, we use two transformations (resub and refactor) to build two different flows $F_0$ and $F_1$. These flows are applied to the same design (\texttt{bfly}) as the previous example. Note that we do not intend to compare the effectiveness of AIG vs MIG based synthesis with this experiment, but rather show the importance of leveraging domain-knowledge for automatic flow generation. 
As in the previous example, we can see that \textbf{(1)} \textit{The transformations at the early stage of the flows have more impacts than the transformations at the late stage.} Also, as we discussed, we can see that for MIG-based, effective flows tend to have a similar number of transformable nodes for the first two transformations, as the first transformation actually defines the actual MIG structure.  
\textbf{(2)} \textit{The choice of early transformations has significant impacts on the performance of the flow}. In this case, the same observation as we did for AIGs hold for MIGs, and the early transformations have more impacts. 

\begin{table}[t]
\caption{Example of the algorithmic domain knowledge presented in Figure \ref{fig:motivation} using MIG-based synthesis transformation \textit{refactor} (rf) and \textit{resub} (rs) with design {bfly} from VTR 8.0 \cite{luu2014vtr} benchmark. We use these transformations as they are area-oriented within the LSOracle flow, and can highlight the importance of picking the right transformation w.r.t the effectiveness of transformable and reduced nodes. \#TNodes = Number of MIG nodes transformed by the corresponding MIG transformation.}
\begin{tabular}{cccccccc}
\textit{$F_0$} & \textit{rf} & \textit{rs} & \textit{rf} & \textit{rs} & \textit{rf} & \textit{rs} & Final \#MIG \\
\textit{\#TNodes} & 984 & 931 & 87 & 44 & 3 & 1 & \textbf{26659} \\ \hline\hline
\textit{$F_1$} & \textit{rs} & \textit{rf} & \textit{rs} & \textit{rf} & \textit{rs} & \textit{rf} & Final \#MIG \\
\textit{\#TNodes} & 1402 & 377 & 74 & 15 & 4 & 1 & 26779
\end{tabular}
\label{tbl:ex2}
\end{table}



\vspace{-3mm}
\subsection{Domain-specific MAB Formulation}\label{sec:mab}

An online program must choose from a set of strategies in a sequence of $n$ trials to maximize the overall payout of the chosen strategies in a multi-armed bandit problem. Such challenges require that a set quantity of resources must be distributed among accessible options in such a way that the expected gain of a given objective is maximized. These are the most important theoretical tools for modeling the exploration-exploitation trade-offs that are inherent in sequential decision-making under uncertainty. Specifically, MAB process is represented as a tuple of $<\mathcal{A},\mathcal{R}>$, where:

{\it
\begin{itemize}
\item $\mathcal{A}$ is a known set of available choices (arms).
\item At each time step $t$, an action $a_t$ is triggered by choosing with one of the choice $a_t \in \mathcal{A}$. 
\item $\mathcal{R}$ is a reward function and $\mathcal{R}^{a_t}$ is the reward at time step $t$ with action $a_t$.
\item The objective of bandit algorithm is to maximize $\textstyle \sum^{t}_{i} \mathcal{R}^{a_t}$
\end{itemize}
}

In a classic MAB sequential decision-making environment, the available decisions at time step $t$ are considered as arms. For example, considering the synthesis flow exploration problem, the selected synthesis transformations will be the set of arms $\mathcal{A}$. Let $\mathcal{A}$ include eight unique transformations $\mathcal{A}$=\{\texttt{resub,rewrite,...,refactor}\}. Let $\mathcal{R}$ be the number of AIG nodes that have been reduced by applying the transformations, such that the objective of the bandit algorithm is to maximize $\textstyle \sum^{t}_{i} \mathcal{R}^{a_t}$, i.e., minimize the number of AIG nodes. Let $F$ be a decision sequence, where $F$=\{$a_0, a_1,..., a_n$\}, $a_t \in \mathcal{A}$. This decision sequence $F$ is a synthesis flow. %
%
A brute-force approach to identifying the optimum flow that maximizes the benefit $F$ performs enough rounds with each transformation (each arm) to determine the true probability of reward. Unfortunately, a brute-force method like this is impractical. In this situation, the bandit algorithm's principal goal is to gather enough data to make the best overall decisions. According to prior plays, the best-known option is chosen during exploitation. The exploration phase will look into unknown choices inside the search space in order to gain more information and close the gap between estimated and true reward function probabilities. This process is analogous to reinforcement learning for synthesis flow exploration without internal states, such as a snapshot of current Boolean network statistics. Despite the fact that MAB sequential decision making is extensively used, it needs to be rethought to fit in with logic synthesis flow exploration. In particular, according to the two observations in Section \ref{sec:algorithm}: 

\begin{itemize}

\item Since the first synthesis transformation dominates the flow, the first action in exploration will dominate the true reward distribution $\mathcal{R}^{*}$ and the exploitation reward distribution $\mathcal{R}$. In other words, the initialization of the bandit algorithm dominates the gap between $\mathcal{R}^{*}$ and $\mathcal{R}$.  

\item While considering each transformation as an arm, each action corresponds to applying one synthesis transformation to the logic graph. Unlike the classic MAB problem that $\mathcal{R}^{*}$ is fixed over time, $\mathcal{R}^{*}$ in synthesis flow exploration changes at each time step, as the logic graph is updated by the transformation.

\end{itemize}



Therefore, to gather the domain knowledge of synthesis algorithms discussed in Section \ref{sec:algorithm}, we propose a novel MAB environment by re-defining the arms and actions, which fits the logic synthesis flow exploration problem. Thus, let $P(\mathcal{X})$ be a random permutation function over a set of decisions $\mathcal{X}$. Let $P(x|\mathcal{X})$ be a random permutation function over the set $\mathcal{X}$, $x \in \mathcal{X}$, such that $P(x_i|\mathcal{X})$ is a random permutation with $x_i$ always being the first element in the permutation, $P(x_i|\mathcal{X}) \in P(\mathcal{X})$. We define $P(x|\mathcal{X})$ to be the arms in the MAB environment, such that $\mathcal{A}$=\{$P(x_0|\mathcal{X})$,~$P(x_1|\mathcal{X})$,~...,~$P(x_n|\mathcal{X})$~\}, where $n$ is the number of available decisions in the exploration problem. Specifically, $n$ corresponds to the number of available synthesis transformations. \textbf{Unlike using traditional MAB algorithms, an action $a_t$ at time $t$ is a sampled permutation from $P(x_i|\mathcal{X})$.} In other words, $a_t$ is a \textit{multiset} over the set $\mathcal{X}$. Let $Q(a_t)$ be the action value that is obtained by applying $a_t$ to a given Boolean network at $t$ time step, the reward is $r_t$
%\begin{equation}
\[
r_t = Q(a_t) - Q(a_{t-1}) \implies Q(P(x_i|\mathcal{X})) - Q(P(x_j|\mathcal{X}))
\]
where the $i^{th}$ arm is played at $t$ time step and $j^{th}$ arm is played at $t-1$ time step, {and $Q(a) = \mathop{\mathbb{E}}(p|a)$ calculates the mean reward (e.g., number of AIGs minimized) from the actions at $t$ step over the estimated winning probabilities $p$}. Finally, we use upper confidence bound (UCB) bandit algorithm as the agent, such that $a_t$ is chosen with estimated upper bound $U_t(a)${, where setting the probability of the true mean being greater than the UCB to be less than or equal to $t^{-1}$, also known as UCB1 algorithm \cite{auer2002finite}. The adopted upper bound can be calculated using \textit{Lai and Robbins} theorem \cite{lai1985asymptotically} and the Hoeffding’s inequality. According to the Hoeffding’s inequality the probability of choosing an action exceeds upper confidence bound (UCB) is bounded by
\begin{equation}
    P[Q(a) > Q_{t}(a) + U_{t}(a)] \leq e^{-2N_{t}(a)U_{t}(a)^{2}}
\end{equation}

In other words, using Hoeffding’s inequality to assign an upper bound to an arm’s mean reward where there is high probability that the true mean will be below the UCB assigned by the algorithm. 

Therefore, while solving $U_t(a)$ in UCB,
\begin{equation}
    e^{-2N_{t}(a)U_{t}(a)^{2}} = p \Rightarrow U_{t}(a) = \sqrt{\frac{-log~p}{2N_{t}(a)}}
\end{equation}
In this case, we can see that reducing the probability of $p$ will increase the rewards from UCB. Setting the probability $p$ of the true mean being greater than the UCB to be less than or equal to $t^{-4}$, a small probability that quickly converges to zero as the number of rounds $t$ grows, which is also known as UCB1 algorithm. However, we find that setting $p=t^{-1}$ is sufficient based on our empirical studies, which results in 
\cite{auer2002finite}.

\begin{equation}
    \sqrt{\frac{-log~p}{2N_{t}(a)}} = \sqrt{\frac{log~t}{2N_{t}(a)}} = \sqrt{\frac{t}{2N_{t}(a)}}, ~~ \text{let} ~ p=t^{-1}
\end{equation}
Thus, we get the following:

\begin{equation}
    a_{t} = \underset{a \in \mathcal{A}}{\mathrm{argmax}}\, \left[ Q(a) + U_{t}(a) \right], ~~ U_{t}(a) = \sqrt{\frac{log~ t}{2N_{t}(a)}}
\end{equation}

% The adopted upper bound can be defined as follows w.r.t \textit{Lai and Robbins} theorem \cite{lai1985asymptotically}}:

%{
% \[
% a_t = \mathop{\mathrm{arg\,max}}_{a \in \mathcal{A}} \left[ Q(a) + U_t(a) \right], U_t(a)=\sqrt{\frac{log~t}{2N_t(a)}}
% \]
}


%\end{equation}

The performance of a multi-armed bandit algorithm is often evaluated in terms of its regret, defined as the gap between the expected payoff of the algorithm and that of an optimal strategy. In this work, the number of regrets equals to the number of synthesis flows that have been evaluated in the synthesis tool. Using the UCB algorithm, an asymptotic logarithmic total regret $L_t$ is achieved \cite{auer2002finite}:

\[
 \lim_{t \to \infty} L_t = 2log~t~\sum \Delta_{a}
\]
where $\Delta_{a}$ is the differences between arms in $\mathcal{A}$.

\begin{figure}[b]
\centering
\includegraphics[width=0.4\textwidth]{./figs/multi-stage-mab.pdf}
\caption{Illustration of the proposed multi-stage bandit approach with four stages.}
\label{fig:multistage}
\vspace{-2mm}
\end{figure}





\subsection{Improving Convergence with Multi-stage Bandit}



While the preceding section's technique relies on optimistic initialization, we suggest a multi-stage bandit to further improve convergence. We can see that the single-stage approach may be used to longer synthesis flows, with each transformation being performed numerous times, based on the formulation in the previous section. However, increasing the length of the sequences leads to a significant increase in the number of explorations required to close the gap between the optimistic reward distribution $\mathcal{R}^*$ and exploitation reward distribution $\mathcal{R}$. Moreover, the optimistic reward distribution $\mathcal{R}^*$ changes as the synthesis transformations are applied to the logic circuit, since the graph structure is modified iteratively. Finally, while synthesis transformations are less successful at late time steps, fine-grain exploration can have a significant impact on EDA flows later on, such as technology mapping and gate sizing.


\begin{figure*}[t]
\centering
\includegraphics[width=0.85\textwidth]{TCAD21-FlowTune/figs/TCAD_Flow_Chart-crop.pdf}
\caption{Overview of the proposed end-to-end MAB synthesis system -- Using ABC front-end, our system accepts technology mapped netlist, Boolean logic netlist, and LUT-netlist. The system is also integrated with VTR 8.0 and Yosys, which enable synthesis optimization for a large range of objectives for designing ASICs and FPGAs, and formal verification tools.}
\label{fig:system_overview}
\end{figure*}


In this context, we introduce the proposed MAB algorithm using a four-stage example shown in Figure \ref{fig:multistage}. Each stage in the multi-stage approach uses the same domain-specific bandit algorithm described in Section \ref{sec:algorithm}. Within each stage, the MAB algorithm is restricted to a fixed number of iterations $m$. Once the first stage is completed, the exploitation reward distribution $\mathcal{R}^1$ is updated (stage 1 in Figure \ref{fig:multistage}), in which a higher rate indicates a higher chance of gaining reward by playing that arm. After $m$ iterations in the first stage, the best-explored synthesis flow will be applied to the input logic circuit, and the synthesized circuit will be the input circuit for the next stage. Rather than starting a new MAB agent with a uniform distribution, we start the second stage using the reward distribution of the first stage's top two arms. For example, in Figure \ref{fig:multistage}, $\mathcal{R}^{1}_{a_0}$ and $\mathcal{R}^{1}_{a_1}$ will be merged and used as the initial reward distribution for the second stage, where $\mathcal{R}^{1}_{a_0}, \mathcal{R}^{1}_{a_1} \in \mathcal{R}^{1}$. This procedure will continue until the $s$ stages have been completed. As we can see, the total number of explorations is $s \cdot m$. In this work, we have explored five different options for ($s,m$), while maintaining the total number of iterations identical.


\noindent
\textbf{Example 2}: We present an illustrative example of the aforementioned domain-specific MAB and the multi-stage bandit algorithm for exploring synthesis flows using the following ABC transformations: \texttt{rw, b, rf,} and \texttt{resub}. Let $\mathcal{X}$ be \{\texttt{4$\times$rw, 4$\times$b, 4$\times$rf, 4$\times$resub}\}. Let the number of stages for exploration be four, such that $\mathcal{X}_{0,1,2,3}=$\{\texttt{rw, b, rf, resub}\}. At first MAB stage, arms $\mathcal{A}_0$
%$\mathcal{A}_0$=\{$P(rw|\mathcal{X}_0)$, ~$P(rf|\mathcal{X}_0)$, ~...,~$P(resub|\mathcal{X}_0)$~\}.
\vspace{-1mm}
\begin{align}
\tiny 
\mathcal{A}_0=\{P(rw|\mathcal{X}_0), 
P(b|\mathcal{X}_0),
P(rf|\mathcal{X}_0),
P(resub|\mathcal{X}_0)~\}
\end{align}
are explored with the proposed MAB algorithm presented in Section \ref{sec:algorithm}. The reward $r_t$ is calculated based on the target objective, e.g., number of reduced AIG nodes compared to the existing best actions. Next, Stage 1 terminates after a fixed number of iterations, and returns the arm(s) with the highest reward value. For the sake of simplicity, this example only includes the arm with the highest reward for stage 2. Let us assume $P(rw|\mathcal{X}_0)$ and $P(rf|\mathcal{X}_0)$ return the highest reward at stage 1. We then define $\mathcal{A}_0^*=\{P(rw|\mathcal{X}_0),P(rf|\mathcal{X}_0)\}$, the arms for second stage, $\mathcal{A}_1$, are updated as follows:
\begin{align}
\tiny 
\mathcal{A}_1=\{\mathcal{A}_0^* \frown  P(rw|\mathcal{X}_1), ~...,\mathcal{A}_0^* \frown  P(resub|\mathcal{X}_1)~\}
\end{align}
where the sample from each arm in $\mathcal{A}_1$ will be a concatenation of two actions from $\mathcal{A}_0^*$ and $P$. For stage 3, we simply replace $\mathcal{A}_0^*$ with $\mathcal{A}_1^*$, which will be the highest reward arms from $\mathcal{A}_1$. Finally, note that the subsets $\mathcal{X}_{0,1,2,3}$ are not necessary to be equally defined. For example, we can define $\mathcal{X}_0$= \{2$\times$\texttt{rw,b,rf,resub}\}, $\mathcal{X}_{1,2}=$\{\texttt{rw, b, rf, resub}\}, and $\mathcal{X}_3$=\{\texttt{b,rf,resub}\}.











\section{FlowTune Framework}

\subsection{Initialization}

As we discussed, the initialization step is crucial for MAB-based exploration performance. We leverage the domain knowledge of DAG-aware synthesis algorithms in our initialization stage. Specifically, for our multi-stage MAB exploration approach, we initialize the reward value for each arm in the first stage using the total number of transformable nodes by sampling each arm. While as demonstrated in Example 1, the total number of transformable nodes for a sequence of transformations highly depends on the first transformation, the initialization involves only one sampling of each arm. More importantly, this scheme significantly reduces the runtime of initialization for objectives such as technology mapping, since counting the number of transformable nodes does not require the actual mapping process. The initialization process is used at the beginning of each stage. To further improve the speed of initialization, we implement a parallel sampling function using OpenMP library \cite{chandra2001parallel}.

%\input{./figs/result_aig.tex}
%\input{./figs/result_fpga.tex}


\subsection{System Integration}

The proposed approach, namely \textit{FlowTune}, is implemented in ABC and LSOracle \cite{lso}. Using the I/O interfaces of ABC and LSOracle, \textit{FlowTune} can take as input logic networks in various formats such as Verilog, AIG, and BLIF. The system overview is shown in Figure \ref{fig:system_overview}. On the ABC side, besides integrating \textit{FlowTune} with logic transformations, we also integrated it with two technology mappers, i.e., \texttt{'map'} for standard-cell mapping, and \texttt{'if'} for FPGA mapping. %We present the effectiveness of \textit{FlowTune} in reducing the number of AIG nodes, as well as the number of LUTs after mapping. 
Similarly, for MIG evaluation, \textit{FlowTune} was integrated with LSOracle for both logic transformations and a native MIG LUT-mapper, the \texttt{'lut\_map'} command. 
For an accurate evaluation of \textit{FlowTune}, we perform post-technology mapping ASIC evaluation, using ABC + Genus for STA, and end-to-end FPGA evaluation in two different contexts: (i) using ABC + VTR as backend targeting a Stratix IV like architecture, and (ii) using LSOracle + OpenFPGA as back-end, also targeting a Stratix IV like architecture. %All the metrics are collected post-place and route, and we take as input for VTR optimized networks through ABC (for AIGs), and for OpenFPGA optimized networks with LSOracle (for MIGs). 
%Thus, for ASICs the timing and area results after standard-cell mapping are generated by reading the mapped Verilog produced by ABC in Cadence Genus, with the predictive ASAP 7nm liberty \cite{xu2017standard}. We also evaluate applying \textit{FlowTune} for CNF clauses minimization. The size of CNF formulations is important to reduce the runtime of Boolean SAT solving, which has been widely applied in verification \cite{moskewicz2001chaff,ciesielski2015verification}, security \cite{yu2017incremental,subramanyan2015evaluating} and reasoning \cite{mcmillan2003interpolation}. 
%To this end, we use \texttt{write\_cnf} function in ABC that dumps AIGs into CNF format. 
% Finally, for an end-to-end FPGA evaluation, we apply \textit{FlowTune} in two different contexts: (i) using the ABC interface built-in Yosys to generate mapped LUT-netlist, we evaluate \textit{FlowTune} in Xilinx Vivado targeting Kintex UltraScale device; (ii) using OpenFPGA and VTR as back-end, we evaluate \textit{FlowTune} targeting a Stratix IV like architecture. All the metrics are collected post-place and route, and we take as input for VTR optimized networks through ABC (for AIGs), and for OpenFPGA optimized networks with LSOracle (for MIGs). 


==> TCAD24-Orch/background.tex <==
%\section{Current state of research in the field}


\vspace{-3mm}
\section{Background}

This section presents useful notations for the reader, as well as reviews the search space while generating synthesis flows. We then present a motivational example on how delay and area may vary with synthesis flow, and how these gains are comparable w.r.t the state-of-the-art. 

\subsection{Notations and Search Space}\label{sec:space}

\noindent
\textbf{Definition 1 \textit{none}-repetition Synthesis Flow}: \textit{Given a set of unique synthesis transformations $\mathbb{S}$=\{$p_0$, $p_1$,..., $p_n$\}, a synthesis flow $\mathbb{F}$ is a permutation of $p_i$ $\in$ $\mathbb{S}$ performed iteratively.} 


%\noindent
\textbf{Example 1:} Let $\mathbb{S}$=\{$p_0$, $p_1$, $p_2$\}. $p_i$ are the transformations in the synthesis tools and can be processed independently. Then, there are totally six flows available: 

\vspace{0mm}
\begin{equation*}
\small
\begin{aligned}
F_0 : p_0 \rightarrow p_1 \rightarrow p_2 ~~
F_1 : p_0 \rightarrow p_2 \rightarrow p_1 \\
F_2 : p_1 \rightarrow p_0 \rightarrow p_2 ~~
F_3 : p_1 \rightarrow p_2 \rightarrow p_0 \\
F_4 : p_2 \rightarrow p_0 \rightarrow p_1 ~~
F_5 : p_2 \rightarrow p_1 \rightarrow p_0
\end{aligned}
\end{equation*}


\textbf{Remark 1}: \textit{Let $f(n,1)$ be the upper bound number of possible flows, where $\mathbb{S}$ includes $n$ elements, and each transformation appears only once, such that:}

\vspace{-2mm}
\begin{align}
\small
f(n,1) = n!
\end{align}

The upper bound of $\mathbb{N}$ happens \textit{iff} all elements in $\mathbb{S}$ can be processed independently. In practice, there could be some constraints to be satisfied for processing these transformations. In this case, $\mathbb{N}$ will be smaller than $n!$. For example, given a constraint that $p_1$ has to be processed before $p_2$, the available flows include only $F_0$, $F_2$, and $F_3$.

\textbf{Definition 2 $m$-repetition Synthesis Flow (m$\geq$2)}: \textit{Given a set of unique synthesis transformations $\mathbb{S}$=\{$p_0$, $p_1$,...,$p_n$\}, a synthesis flow with $m$-repetition $\mathbb{F}_{m}$ is a permutation of $p_i$ $\in$ $\mathbb{S}_{m}$, where $\mathbb{S}_{m}$ contains $m$ $\mathbb{S}$ sets.} 

\textbf{Example 2:} Let $\mathbb{S}$=\{$p_0$, $p_1$\}. Each $p_i$ can be processed independently. For developing $2$-repetition synthesis flows, $\mathbb{S}_{2}$=\{$p_0$, $p_1$, $p_0$, $p_1$\}. The available flows include:

\vspace{-2mm}
\begin{equation*}
\small
\begin{aligned}
F_0 : p_0 \rightarrow p_0 \rightarrow p_1 \rightarrow p_1~~
F_1 : p_1 \rightarrow p_1 \rightarrow p_0 \rightarrow p_0 \\
F_2 : p_0 \rightarrow p_1 \rightarrow p_0 \rightarrow p_1~~
F_3 : p_1 \rightarrow p_0 \rightarrow p_1 \rightarrow p_0 \\
F_4 : p_0 \rightarrow p_1 \rightarrow p_1 \rightarrow p_0~~
F_5 : p_1 \rightarrow p_0 \rightarrow p_0 \rightarrow p_1 \\
\end{aligned}
\end{equation*}




\textbf{Remark 2}: \textit{Let $\mathbb{L}$ be the length of a synthesis flow. Given a  $m$-repetition $\mathbb{F}_{m}$ with $n$ transformations in $\mathbb{S}$, $\mathbb{L}$ = $n$$\times$$m$.}

The search space for $m$-repetition flows is a \textit{multiset} permutation problem. Hence, a closed formula can be derived to describe the search space of $m$-repetition flows. The search space of $m$-repetition flows with $n$ unique transformations is shown in Equation \ref{eq:space1}.

\textbf{Remark 3}: \textit{Let function $f(n,m)$ be upper bound number of available $m$-repetition flows with $n$ elements in $S$. $f(n,m)$ uniquely satisfies the following formula :}%\cite{mendelson1981permutations}


\begin{align}
\small
\begin{aligned}
f(n,m) = \dfrac{(n\cdot m)!}{(m!)^n}
%where \mathbb{L} > m, m = 2,3,...
\end{aligned}
\label{eq:space1}
\end{align}

With the multiset permutation concept, Yu et al. \cite{DBLP:conf/dac/YuXM18} generalized the formula to describe the search space for any type of \textit{m-}repetition flows. {Let $n$ be the number of unique transformation, the $M$-repetition flows, $M$=\{$m_{0}, m_{1}, ...,m_{n-1}$\}, where $m_i$ is the number of repetitions of the $i^{th}$ transformation}. The total number of possible flows is shown in Equation 2. 

\textbf{Remark 4}: {\textit{Let function $f(n,\mathbb{L},\{m_{0}, m_{1}, ...,m_{n-1}\})$ be upper bound number of flows with $n$ elements in $S$}. The $i^{th}$ element in $S$ appears $m_i$ times. The function uniquely satisfies the following formula :}%\cite{mendelson1981permutations}

\vspace{-2mm}
\begin{align}
\scriptsize
f(n,\mathbb{L},\{m_{0}, m_{1}, ...,m_{n-1}\}) = \dfrac{(m_0+m_1+\cdot\cdot\cdot m_{n-1})!}{(m_0!)(m_1!)\cdot\cdot\cdot(m_{n-1}!)}
\end{align}

\textbf{Remark 5}: {\textit{Let {$\mathbb{L}$ be the length of the type of flows with upper bound $f(n,\mathbb{L},\{m_{0}, m_{1}, ...,m_{n-1}\})$, $\mathbb{L}$=$\sum_{i=0}^{n-1}m_i$.}}}

Whereas the work in \cite{DBLP:conf/dac/YuXM18} constraints the search-space to \textit{m-}repetitions flow, with the upper bound given by Equation 2, in this work we approach this problem in a more general way, where each repetition might have a different number of repetitions. In this case, the theoretical upper bound is given by Equation 3. 

%\subsection{Quality of Result in Digital ICs}

% \begin{figure}[t]
% \centering
% \begin{minipage}{0.24\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/1-crop.pdf}
% \subcaption{}\label{fig:fa_labeling_a}
% \end{minipage}%
% \begin{minipage}{0.2\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/2-crop.pdf}
% \subcaption{}\label{fig:fa_labeling_b}
% \end{minipage}%
% \caption{1-bit Full Adder ($F= 2C+S=a+b+c$) gate-level netlists produced by two different synthesis flows using 7nm FinFET technology library. a) Delay = 30.1 ps, Area = 9.40 um$^2$; b) Delay = 47.6 ps, Area = 8.38 um$^2$.}
% \label{fig:full_adder}
% \end{figure}


% \begin{figure*}[b]
% \centering
% \begin{minipage}{0.235\textwidth}
%   \centering
%   \small
% \includegraphics[width=1\textwidth]{figs/aes-all-distribution.eps}
% \subcaption{2-D QoR distro of AES}\label{fig:motivation1-aes}
% \end{minipage}%
% \begin{minipage}{0.235\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/aes-all-distribution-3D.eps}
% \subcaption{3-D QoR distro of AES}\label{fig:motivation2-aes}
% \end{minipage}%
% %datapath
% \begin{minipage}{0.235\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/datapath-all-distribution.eps}
% \subcaption{2-D QoR distro of ALU}\label{fig:motivation1-datapath}
% \end{minipage}%
% \begin{minipage}{0.235\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/datapath-all-distribution-3D.eps}
% \subcaption{3-D QoR distro of ALU}\label{fig:motivation2-datapath}
% \end{minipage}%
% \caption{Delay and area results of the 50,000 random ABC synthesis flows of 128-bit AES core and 64-bit ALU.}
% \vspace{-4mm}
% \label{fig:motivation}
% \end{figure*}


%QoR of Integrated Circuits (IC) is a term used in evaluating the quality of the IC based on different metrics. Mostly, it is represented as a vector of values that describes the performance of the designs and design process. For example, a QoR could include the critical path delay (chip frequency = 1$/$Delay), power dissipation, area, e.g., \{1 ns (1 GHz), 2.5 W, 1 mm$^2$\}. Given a design specification, the QoR of the technological processed designs can be very different using different synthesis flows. In particular, synthesis flows are designed and applied depending on the application, as different applications can have very different objectives and features. For instance, for high-performance image processing, the designs are mostly designed to be as fast as possible, i.e., delay to be as small as possible. On the other hand, for the Internet-of-Things (IoT), designs aim to minimize the power and area primarily. The massive search space of synthesis flows (Equations 1-3), the time-consuming technological design process for QoR evaluation, along the various design objectives are the main motivations of this work.

%An illustrative example of mapping a 1-bit Full Adder using 7nm FinFET technology library is shown in Figure \ref{fig:full_adder}. The specification of a 1-bit Full Adder is $a+b+c = 2C + S$, where $a,b,c,C,S$ are binary signals. Using two different synthesis flows, two gate-level netlists are produced. In Figure \ref{fig:full_adder}, each node represents one logic gate and the type label of the node is the type of the logic gate. Note that the performance of different logic gates are different and they are defined based on the technology libraries. For example, delay and area of XOR2 are 15.95 ps and 2.8 um$^2$; delay and area of NAND2 are 11.90 ps and 1.39 um$^2$. After applying synthesis flow, we observe that the QoRs of two netlists are different. The design in Figure \ref{fig:fa_labeling_a} is about 37\% faster than design in Figure \ref{fig:fa_labeling_b}, and requires 12\% more area. Note that the QoR can only be obtained after the entire technological design process. For large designs, this process is extremely time-consuming.




%3.2466705$\cdot10^{15}$

\subsection{Motivating Example}\label{sec:motivating-example}

\begin{figure}[!h]
\centering
\includegraphics[width=0.44\textwidth]{figs/aes_abc_heat_partial.pdf}
\caption{Evaluation of three default flows, \textit{resyn ('o'), resyn2 ('x')} and \textit{resyn3 (the star)} using 128-bit AES design. The heatmap includes the QoR of the 50,000 random flows.}
\label{fig:default_flow_compare}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=0.44\textwidth]{figs/aes_lso_heat_partial.pdf}
\caption{Evaluation of the LSOracle default flow (black star) using 128-bit AES design. The heatmap includes the QoR of the 50,000 random flows.}
\label{fig:lso_flow_compare}
\end{figure}

We provide two motivating examples using open-source logic synthesis framework ABC \cite{mishchenko2010abc} and LSOracle \cite{neto2019lsoracle}, in which the backend data structures are AIGs and MIGs, respectively. % shown in Figure \ref{fig:default_flow_compare}. 
The experimental setups for the motivational examples are as follows:

%    \vspace{0mm}
%\begin{itemize}
\noindent
\textbf{ABC \cite{mishchenko2010abc}} -- We use the following set of commands: $\mathbb{S}$=\{balance, restructure, rewrite, refactor, rewrite -z, refactor -z\} ($n$=6); the elements in  $\mathbb{S}$ are logic transformations in ABC\footnote{\small The names of these transformations are the same as the commands in ABC.} that can be processed independently. We take as input a 128-bit Advanced Encryption Standard (AES) core\cite{opencore-web} and generate 50,000 unique $4$-repetition flows are generated by random permutations of  $\mathbb{S}_{4}$ ($m$=4, $n$=6, $\mathbb{L}$=24). The delay and area of these flows are obtained after technology mapping using the ASAP 7nm predictive standard-cell library.  

\noindent
\textbf{LSOracle\cite{neto2019lsoracle}} -- We use the following transformations: $\mathbb{S}$=\{rewrite, resub, refactor\} ($n$=3). That is because these are the main transformations used in the highest MIG-based transformation in LSOracle. We take as input a 128-bit Advanced Encryption Standard (AES) core\cite{opencore-web} and generate 50,000 unique $4$-repetition flows are generated by random permutations of  $\mathbb{S}_{4}$ ($m$=3, $n$=9, $\mathbb{L}$=27). We chose to have a flow of length 27 as it is a multiplier of the default LSOracle flow, which has 9 transformations by default. To compare, we run the default LSOracle flow 3$\times$. The delay and area of these flows are obtained after technology mapping using the ASAP 7nm predictive standard-cell library.


The QoR distributions for the AES can be seen in Figures \ref{fig:default_flow_compare},\ref{fig:lso_flow_compare}, and several important observations can be drawn from it, which highlight the main motivations of this work:
    \vspace{0mm}


\begin{itemize}
    \item (1) Given the same set of synthesis transformations, the QoR is very different using different flows, for both AIG and MIG. For example, for the AIG case, the delay and area of AES design produced by the 50,000 flows have up to 40\% and 90\% difference, respectively. As for the MIG-based flow, the variance of delay and area are up to {39.27\% and 13.97\%}, respectively. 
    \vspace{0mm}
    \item (2) The search space of the synthesis flows is large. According to Remark 3, the total number of available $4$-repetition flows with $n=6$ independent synthesis transformations is more than $10^{16}$ (considering our AIG example). Discovering the high-quality synthesis flows with human-testing among the entire search space is unlikely to be achieved. Same holds for MIGs.
        \vspace{0mm}
    % \item The same set of flows perform differently on different designs. For example, in Figure \ref{fig:motivation}, QoR distributions of AES and ALU are \textit{statistically significant}. This means that the high-quality flows for AES design could perform poorly for ALU. Therefore, synthesis flows need to be customized for specific IP or design.
        \vspace{0mm}
\end{itemize}

% To further show the motivations, we compare the random flows to the default flows developed by experts provided in ABC using 128-bit AES design. The results are shown in Figure \ref{fig:default_flow_compare}.

As it is possible to observe, we position the three most widely used default flows provided in ABC, including \textit{resyn, resyn2} and \textit{resyn3}, with respect to the QoR achieved with the random flows. Whereas \textit{resyn} provides the best QoR among these three default flows, its result performs $>$10\% worse than the best flows of the 50,000 random flows, in both delay and area. Specifically, there are more than 25,000 random flows that perform better than all the default flows. This means that for every two random permuted flows, one of them is likely to over-perform the expert-developed flows for this design. 
Similarly, we show that a high-effort and well expert-tuned flow in LSOracle flow MIGs still have much room for improvement. In particular, the default flow presents a good delay overall, but with room for achieving a better area ($\approx$7\% worse area than random flows with similar delay). 
These motivational examples show that automatic flow generation is an important direction for both AIG- and MIG-based synthesis flow generation. This, along with the large search space, provides the main motivation for this work. It is also important to note that a given flow performs differently on different designs. For example, high-quality flows for our AES design could perform poorly on other designs \cite{DBLP:conf/dac/YuXM18}. 








==> TCAD24-Orch/figs/analysis_figure.tex <==

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_s38584.pdf}
        \caption{s38584}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_s35932.pdf}
        \caption{s35932}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_b17.pdf}
        \caption{b17\_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_b18.pdf}
        \caption{b18\_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_b21.pdf}
        \caption{b21}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_bfly.pdf}
        \caption{bfly}\label{fig:bfly_bd}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_fir.pdf}
        \caption{fir}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_mem_ctrl.pdf}
        \caption{mem\_ctrl}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_sqrt.pdf}
        \caption{sqrt}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_voter.pdf}
        \caption{voter}
        \label{fig:ana_voter}
    \end{subfigure}
     \caption{{The optimization opportunities with different optimization operations. The $X-$axis denotes the optimization operations. The $Y-$axis denotes the number of valid iterations with the corresponding operation.}}
    % \vspace{-2mm}
     \label{fig:ana}
\end{figure*}


==> TCAD24-Orch/figs/results_1o_plot.tex <==

\begin{figure}[!htb]
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O1.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O1}}$}
  \label{fig:1O_O1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include second image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O2.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O2}}$}
  \label{fig:1O_O2}
\end{subfigure}
\hfill

\begin{subfigure}{0.49\linewidth}
  \centering
  % include third image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O3.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O3}}$}
  \label{fig:1O_O3}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include fourth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O4.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O4}}$}
  \label{fig:1O_O4}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include fifth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O5.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O5}}$}
  \label{fig:1O_O5}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include sixth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O6.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O6}}$}
  \label{fig:1O_O6}
\end{subfigure}
\caption{Normalized node number comparison of the same design after applying stand-alone optimizations and \texttt{orchestration} with a single AIG traversal. \textbf{R} is the ratio of the number of designs on which \texttt{orchestration} outperforms stand-alone optimization to the number of total tested designs.}
\vspace{-4mm}
\label{fig:1O}
\end{figure}


==> TCAD24-Orch/figs/results_3o_plot.tex <==
\begin{figure}[!htb]
\centering
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_1.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{\texttt{O1}}$)}
  \label{fig:3O_O1}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include third image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_3.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{\texttt{O3}}$)}
  \label{fig:3O_O3}
\end{subfigure}

\caption{Normalized node number comparison between iterative \texttt{orchestration} and iterative ABC SOTA optimizations. \textbf{R} is the ratio of the number of designs on which Seq($\widehat{\texttt{On}}$) outperforms Seq(ABC) to the number of total tested designs.}
%\vspace{-3mm}
\label{fig:3O}
\end{figure}




==> TCAD24-Orch/preamble/authorlist.tex <==
\newbool{journalBasedAuthors}
\ifCLASSOPTIONpeerreview \setbool{journalBasedAuthors}{true}
\else \ifCLASSOPTIONjournal \setbool{journalBasedAuthors}{true}
\else \setbool{journalBasedAuthors}{false}
\fi
\fi

\ifbool{journalBasedAuthors}
{

    \author{Yingjie~Li,
            Mingju~Liu,
            Haoxing~Ren,
            Alan~Mishchenko, 
            Cunxi~Yu
    %\thanks{Manuscript received April XX, 2016; revised Month DD, 2016.}%
    % \thanks{W. Lau Neto is with Silicon Realization Group of Synopsys Inc., Sunnyvale, CA, US. (e-mail: launeto@synopsys.com).}
    \thanks{Y. Li, M. Liu and C. Yu are with the Department of Electrical and Computer Engineering, University of Maryland,  College Park, US (e-mails: yingjieli@umd.edu, mliu9867@umd.edu cunxiyu@umd.edu). A. Mishchenko is with the Department of Electrical Engineering and Computer Sciences, University of California, Berkeley, US (e-mail: alanmi@berkeley.edu). H. Ren is with Nvidia Research, Austin, Texas, US (e-mail: haoxingr@nvidia.com).}
    \thanks{This work is funded by National Science Foundation (NSF) NSF-2008144 and NSF CAREER award NSF-2047176.}
    \ifCLASSOPTIONjournal
        \thanks{Digital Object Identifier 10.1109/TCAD.XXXXXXX}
    \fi
    }
}





==> TCAD24-Orch/runtime_ana.tex <==
\subsection{Single Runtime Evaluation}
\label{sec:runtime_result}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.99\textwidth]{TCAD21-FlowTune/figs/runtime_rw.pdf}
        \caption{runtime comparison with \texttt{rw}}
        \label{fig:rt_rw_pure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.99\textwidth]{TCAD21-FlowTune/figs/runtime_rs.pdf}
        \caption{runtime comparison with \texttt{rs}}
        \label{fig:rt_rs_pure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
\includegraphics[width=0.99\textwidth]{TCAD21-FlowTune/figs/runtime_rf.pdf}
        \caption{runtime comparison with \texttt{rf}}
        \label{fig:rt_rf_pure}
    \end{subfigure}
     
 \caption{Runtime comparison between selected single-traversal \texttt{orchestration} policies ($\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{Local-greedy} (labeled as \texttt{LGP})) and stand-alone optimizations from ABC: (a) runtime comparison with \texttt{rw}; (b) runtime comparison with \texttt{rs}; (c) runtime comparison with \texttt{rf}.
}
    \label{fig:runtime comparison_pure}
\end{figure*}
\input{tbls/table_runtime}

\yingjie{In this section, we further discuss the runtime cost for orchestration algorithms and its comparison with stand-alone optimization algorithms for all 104 designs in Figure \ref{fig:runtime comparison}.
We present the runtime comparisons for the single graph traversal with \textit{Local-greedy} orchestration optimization (\texttt{LGP}) and \textit{Priority-ordered} orchestration optimization with $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$ ($\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$), with stand-alone optimizations (i.e., \texttt{rw}, \texttt{rs}, and \texttt{rf}).}
%A runtime comparison for all 104 designs across diverse benchmark suites between $\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{LGP} as opposed to \texttt{rw}, \texttt{rs}, and \texttt{rf}, respectively, is depicted in Figure \ref{fig:runtime comparison}. 
In Figure \ref{fig:runtime comparison}, to improve the discernibility of runtime discrepancies, the figure's axes employ a logarithmic scale. The x-axis signifies the stand-alone ABC optimization runtime, while the y-axis corresponds to the \textit{orchestration} runtime. The dotted line ($x=y$) serves as a demarcation for runtime performance: a point above the line suggests increased runtime cost generated by the respective \textit{orchestration} algorithm in comparison to the corresponding stand-alone ABC optimization, while a point below the line implies reduced runtime cost. 

For example, in Figure \ref{fig:rt_rs}, a majority of the blue dots are positioned above the dotted line, denoting that the \texttt{LGP} incurs runtime overhead relative to \texttt{rs}; while the red triangles and green stars, which denotes the runtime for $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$, are mostly below the dotted line, indicating that the \textit{Priority-ordered} orchestration algorithm functions with less runtime compared to \texttt{rs}. Thus, compared with stand-alone optimizations, i.e, \texttt{rw}, \texttt{rs}, and \texttt{rf}, we find that \textbf{(1)} the \textit{Local-greedy} orchestration method incurs runtime overhead for most designs as it requires the transformability check for all three optimization operations at each node as shown in Algorithm \ref{alg:local}, line 2; \textbf{(2)} the \textit{Priority-ordered} orchestration incurs less runtime cost than \textit{Local-greedy} orchestration method and stand-alone optimizations. Compared with \textit{Local-greedy} orchestration, \textit{Priority-ordered} orchestration conducts significantly less transformability check based on the pre-defined priority order. %while compared with stand-alone optimizations, it involves less running iterations as more optimization opportunities lead to more nodes within the optimization cut excluded from the iterations at each applicable optimization operation.

{To further analyze the runtime differences, we include }Table \ref{table:it_count} that presents the iteration counts of stand-alone ABC optimizations and the averagely best \textit{Priority-ordered} orchestration algorithm with $\widehat{\texttt{O3}}$. 
\yingjie{There are mainly two observations from Table \ref{table:it_count}: \textbf{(1)} The total number of iterations in the orchestration algorithm is significantly less than that in \texttt{rw}, which results in its less runtime cost compared with \texttt{rw}. As we discussed in Section \ref{sec:background_DAG_syn}, the logic cut used in each iteration in \texttt{rw} is relatively small (4-feasible cut), thus to traverse the whole graph (usually with the graph size of $10^{2} - 10^{6}$), it requires significantly more iterations compared with other optimization algorithms involving large logic cut per iteration such as \texttt{rs} and \texttt{rf}. While the orchestration algorithm involves \texttt{rs} and \texttt{rf} into the graph traversal, it saves a significant number of required iterations and thus the required runtime. \textbf{(2)} Even though the orchestration algorithm requires more iterations than \texttt{rs} and \texttt{rf}, it incurs less runtime. 
Compared with \texttt{rs} and \texttt{rf}, the orchestration algorithm requires more iterations, which results from the involvements of \texttt{rw} iterations with small cut size in the graph traversal in the orchestrated optimization. However, the small logic cut per iteration in \texttt{rw} incurs less runtime cost, and combining \texttt{rw} iterations in the optimization can result in less average runtime cost over all iterations compared to \texttt{rs} and \texttt{rf}.} 


==> TCAD24-Orch/tbls/tabel_end-to-end.tex <==
\begin{table*}[]
\caption{The results reported by OpenROAD with orchestration methods implementation, including the results from logic synthesis, i.e., AIG minimization, technology mapping with nangate 45nm, and post-routing.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
 &    &   &   & &  &  &  &  &      \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Logic Synthesis \\ (resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Logic Synthesis\\ (LGP-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Logic Synthesis\\  (O-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Tech Map\\  (resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Tech Map\\ (LGP-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Tech Map\\  (O-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Post-routing \\ (resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Post-routing\\ (LGP-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Post-routing\\ (O-resyn)\end{tabular}} \\ \hline
   & Node   & Node   & Node  & Area      & Area & Area    & Area/$um^{2}$       & Area/$um^{2}$       & Area/$um^{2}$        \\ \hline
s38584             & 10391                                                                                & 9988 (-3.9\%)                                                                             & 10085 (-2.9\%)                                                                                & 13161.95                                                                      & 13000.48 (-1.2\%)                                                                   & 13011.922 (-1.1\%)                                                                     & 14313                                                                             & 14013 (-2.1\%)                                                                          & 14137 (-1.2\%)                                                                            \\ \hline
s35932             & 8518   & 8113 (-4.8\%)    & 8177 (-4.0\%)                                                         & 15368.15                                              & 15372.40 (+0.03\%)              &15368.15 (0)   & 16045      & 16055 (+0.06\%)        & 16045 (0)                                                         \\ \hline
b17\_1             & 23021                                                                                & 21475 (-6.7\%)                                                                             & 22046 (-4.2\%)                                                                                & 26798.44                                                                      & 25640.27 (-4.3\%)                                                                                    & 26019.588 (-2.9\%)                                                                     & 29138                                                                             &   28193 (-3.2\%)                                                                                      & 28561 (-2.0\%)                                                                            \\ \hline
b18\_1             & 63151                                                                                & 58983 (-6.6\%)                                                                             & 60231 (-4.6\%)                                                                                & 70259.38                                                                      & 68211.18 (-2.9\%)                                                                   & 67852.876 (-3.4\%)                                                                     & 76811                                                                             & 74499 (-3.0\%)                                                                          & 74516 (-3.0\%)                                                                            \\ \hline
b20                & 10152                                                                                & 9464 (-6.8\%)                                                                              & 9678 (-4.6\%)                                                                                 & 11295.96                                                                      & 10915.57 (-3.3\%)                                                                   & 11029.158 (-2.4\%)                                                                     & 12247                                                                             & 11861 (-3.1\%)                                                                          & 12027 (-1.8\%)                                                                            \\ \hline
b21                & 10211                                                                                & 9580 (-6.2\%)                                                                              & 9790 (-4.1\%)                                                                                 & 11585.63                                                                      & 11190.09 (-3.4\%)                                                                   & 11222.274 (-3.1\%)                                                                     & 12596                                                                             & 12246 (-2.7\%)                                                                          & 12276 (-2.5\%)                                                                            \\ \hline
b22                & 15067                                                                                & 14137 (-6.2\%)                                                                             & 14480 (-3.9\%)                                                                                & 16115.61                                                                      & 15879.67 (-1.4\%)                                                                   & 15928.612 (-1.2\%)                                                                     & 17856                                                                             & 17404 (-2.5\%)                                                                          & 17518 (-1.9\%)                                                                            \\ \hline
\end{tabular}
}
% \caption{The results reported by OpenROAD with orchestration methods implementation, including the results from logic synthesis, i.e., AIG minimization, technology mapping with nangate 45nm, and post-routing.}
\label{tbl:resyn_openroad}
\end{table*}





==> TCAD24-Orch/tbls/table_1o.tex <==
\begin{table*}[t]
\centering
\caption{Detailed results of selected large size designs. Comparison of single-traversal \textit{orchestration} with stand-alone optimizations from ABC.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|ccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{11}{c|}{AIG} \\ \cline{3-13} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{Baseline} & \multicolumn{1}{c|}{\texttt{rw}} & \multicolumn{1}{c|}{\texttt{rs}} & \multicolumn{1}{c|}{\texttt{rf}} & \multicolumn{1}{c|}{$\widehat{\texttt{O1}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O2}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O3}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O4}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O5}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O6}}$} & ${\texttt{LocalGreedy}}$\\ \cline{3-13} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \#Node ($\Delta$\%) \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & \multicolumn{1}{c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{10697 (13.7\%)} & \multicolumn{1}{c|}{11505 (7.2\%)} & \multicolumn{1}{c|}{10932 (11.8\%)} & \multicolumn{1}{c|}{10366 (16.4\%)} & \multicolumn{1}{c|}{10379 (16.3\%)} & \multicolumn{1}{c|}{\textbf{10336 (16.7\%)}} & \multicolumn{1}{c|}{10655 (14.1\%)} & \multicolumn{1}{c|}{10932 (11.8\%)} & \multicolumn{1}{c|}{10932 (11.8\%)} & 10449 (15.7\%) \\ \cline{2-13} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{9110 (23.8\%)} & \multicolumn{1}{c|}{11916 (0.3\%)} & \multicolumn{1}{c|}{9836 (17.7\%)} & \multicolumn{1}{c|}{\textbf{8561 (28.4\%)}} & \multicolumn{1}{c|}{\textbf{8561 (28.4\%)}} & \multicolumn{1}{c|}{\textbf{8561 (28.4\%)}} & \multicolumn{1}{c|}{9836 (17.7\%)} & \multicolumn{1}{c|}{9836 (17.7\%)} & \multicolumn{1}{c|}{9836 (17.7\%)} & \textbf{8561 (28.4\%)} \\ \cline{2-13} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{24178 (12.6\%)} & \multicolumn{1}{c|}{26305 (4.9\%)} & \multicolumn{1}{c|}{24533 (11.3\%)} & \multicolumn{1}{c|}{22951 (17.0\%)} & \multicolumn{1}{c|}{23125 (16.4\%)} & \multicolumn{1}{c|}{\textbf{22935 (17.0\%)}} & \multicolumn{1}{c|}{23393 (15.4\%)} & \multicolumn{1}{c|}{24532 (11.3\%)} & \multicolumn{1}{c|}{24532 (11.3\%)} & {23008 (16.7\%)} \\ \cline{2-13} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{66807 (15.5\%)} & \multicolumn{1}{c|}{73076 (7.6\%)} & \multicolumn{1}{c|}{69606 (12.0\%)} & \multicolumn{1}{c|}{63431 (19.8\%)} & \multicolumn{1}{c|}{64135 (18.9\%)} & \multicolumn{1}{c|}{\textbf{63167 (20.1\%)}} & \multicolumn{1}{c|}{65956 (16.6\%)} & \multicolumn{1}{c|}{69586 (12.0\%)} & \multicolumn{1}{c|}{69587 (12.0\%)} & 63726 (19.4\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{10659 (12.8\%)} & \multicolumn{1}{c|}{11197 (8.4\%)} & \multicolumn{1}{c|}{10593 (13.3\%)} & \multicolumn{1}{c|}{10017 (18.02\%)} & \multicolumn{1}{c|}{10110 (17.3\%)} & \multicolumn{1}{c|}{\textbf{10011 (18.1\%)}} & \multicolumn{1}{c|}{10228 (16.3\%)} & \multicolumn{1}{c|}{10590 (13.3\%)} & \multicolumn{1}{c|}{10590 (13.3\%)} & 10129 (17.1\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{10863 (15.1\%)} & \multicolumn{1}{c|}{11449 (10.4\%)} & \multicolumn{1}{c|}{10961 (14.3\%)} & \multicolumn{1}{c|}{10146 (20.6\%)} & \multicolumn{1}{c|}{10237 (19.9\%)} & \multicolumn{1}{c|}{\textbf{10133 (20.7\%)}} & \multicolumn{1}{c|}{10458 (18.2\%)} & \multicolumn{1}{c|}{10958 (14.3\%)} & \multicolumn{1}{c|}{10958 (14.3\%)} & 10261 (19.7\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{15983 (13.6\%)} & \multicolumn{1}{c|}{16891 (8.6\%)} & \multicolumn{1}{c|}{15983 (13.6\%)} & \multicolumn{1}{c|}{14977 (19.0\%)} & \multicolumn{1}{c|}{15115 (18.2\%)} & \multicolumn{1}{c|}{\textbf{14953 (19.1\%)}} & \multicolumn{1}{c|}{15275 (17.4\%)} & \multicolumn{1}{c|}{15965 (13.6\%)} & \multicolumn{1}{c|}{15965 (13.6\%)} & 15127 (18.2\%) \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & \multicolumn{1}{c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{26827 (7.2\%)} & \multicolumn{1}{c|}{27060 (6.4\%)} & \multicolumn{1}{c|}{27487 (4.9\%)} & \multicolumn{1}{c|}{\textbf{25996 (10.1\%)}} & \multicolumn{1}{c|}{26183 (9.4\%)} & \multicolumn{1}{c|}{26027 (10.0\%)} & \multicolumn{1}{c|}{26353 (8.8\%)} & \multicolumn{1}{c|}{27487 (4.9\%)} & \multicolumn{1}{c|}{27487 (4.9\%)} & 26181 (9.4\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{26132 (7.5\%)} & \multicolumn{1}{c|}{26352 (6.73\%)} & \multicolumn{1}{c|}{26972 (4.5\%)} & \multicolumn{1}{c|}{\textbf{25339 (10.3\%)}} & \multicolumn{1}{c|}{25552 (9.5\%)} & \multicolumn{1}{c|}{25345 (10.3\%)} & \multicolumn{1}{c|}{25768 (8.8\%)} & \multicolumn{1}{c|}{26970 (4.5\%)} & \multicolumn{1}{c|}{26970 (4.5\%)} & {25496 (9.7\%)} \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{25641 (7.5\%)} & \multicolumn{1}{c|}{25768 (7.0\%)} & \multicolumn{1}{c|}{26437 (4.6\%)} & \multicolumn{1}{c|}{\textbf{24778 (10.6\%)}} & \multicolumn{1}{c|}{25061 (9.5\%)} & \multicolumn{1}{c|}{24831 (10.4\%)} & \multicolumn{1}{c|}{25189 (9.1\%)} & \multicolumn{1}{c|}{26437 (4.6\%)} & \multicolumn{1}{c|}{26437 (4.6\%)} & 24987 (9.8\%) \\ \cline{2-13}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{27787 (7.4\%)} & \multicolumn{1}{c|}{28031 (6.6\%)} & \multicolumn{1}{c|}{28617 (4.6\%)} & \multicolumn{1}{c|}{\textbf{27013 (10.0\%)}} & \multicolumn{1}{c|}{27266 (9.1\%)} & \multicolumn{1}{c|}{27048 (9.9\%)} & \multicolumn{1}{c|}{27444 (8.5\%)} & \multicolumn{1}{c|}{28617 (4.6\%)} & \multicolumn{1}{c|}{28617 (4.6\%)} & {27198 (9.3\%)} \\ \hline


\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & \multicolumn{1}{c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{41153 (28.1\%)} & \multicolumn{1}{c|}{52621 (8.1\%)} & \multicolumn{1}{c|}{56745 (0.9\%)} & \multicolumn{1}{c|}{\textbf{41123 (28.2\%)}} & \multicolumn{1}{c|}{41143 (28.1\%)} & \multicolumn{1}{c|}{41124 (28.2\%)} & \multicolumn{1}{c|}{52098 (9.0\%)} & \multicolumn{1}{c|}{56738 (0.9\%)} & \multicolumn{1}{c|}{56738 (0.9\%)} & 41147 (28.1\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{214274 (0.0\%)} & \multicolumn{1}{c|}{209164 (2.4\%)} & \multicolumn{1}{c|}{212341 (1.0\%)} & \multicolumn{1}{c|}{207335 (3.3\%)} & \multicolumn{1}{c|}{212327 (0.9\%)} & \multicolumn{1}{c|}{\textbf{207315 (3.3\%)}} & \multicolumn{1}{c|}{\textbf{207315 (3.3\%)}} & \multicolumn{1}{c|}{212338 (1.0\%)} & \multicolumn{1}{c|}{212338 (1.0\%)} & 207319 (3.3\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{46732 (0.2\%)} & \multicolumn{1}{c|}{46554 (0.6\%)} & \multicolumn{1}{c|}{46574 (0.6\%)} & \multicolumn{1}{c|}{46301 (1.1\%)} & \multicolumn{1}{c|}{46484 (0.8\%)} & \multicolumn{1}{c|}{\textbf{46085 (1.6\%)}} & \multicolumn{1}{c|}{46204 (1.4\%)} & \multicolumn{1}{c|}{46569 (0.6\%)} & \multicolumn{1}{c|}{46569 (0.6\%)} & {46201 (1.3\%)} \\ \cline{2-13}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{19441 (21.0\%)} & \multicolumn{1}{c|}{21690 (11.9\%)} & \multicolumn{1}{c|}{23685 (3.8\%)} & \multicolumn{1}{c|}{\textbf{19221 (21.9\%)}} & \multicolumn{1}{c|}{19441 (21.0\%)} & \multicolumn{1}{c|}{\textbf{19221 (21.9\%)}} & \multicolumn{1}{c|}{21582 (12.3\%)} & \multicolumn{1}{c|}{23685 (3.8\%)} & \multicolumn{1}{c|}{23685 (3.8\%)} & 19221 (21.9\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{11408 (17.0\%)} & \multicolumn{1}{c|}{10997 (20.1\%)} & \multicolumn{1}{c|}{12681 (7.8\%)} & \multicolumn{1}{c|}{9461 (31.2\%)} & \multicolumn{1}{c|}{10982 (20.2\%)} & \multicolumn{1}{c|}{\textbf{9399 (31.7\%)}} & \multicolumn{1}{c|}{9492 (31.0\%)} & \multicolumn{1}{c|}{12679 (7.8\%)} & \multicolumn{1}{c|}{12679 (7.8\%)} & 9606 (30.2\%) \\ \hline

\multicolumn{3}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{1}{c|}{12.7\%} & \multicolumn{1}{c|}{7.3\%} & \multicolumn{1}{c|}{7.9\%} & \multicolumn{1}{c|}{16.6\%} & \multicolumn{1}{c|}{15.3\%} & \multicolumn{1}{c|}{\textbf{16.7\%}} & \multicolumn{1}{c|}{13.0\%} & \multicolumn{1}{c|}{7.9\%} & \multicolumn{1}{c|}{7.9\%} & 16.1\% \\ \hline

\multicolumn{3}{|c|}{{\textbf{Avg. Runtime (s)}}} & \multicolumn{1}{c|}{{0.366}} & \multicolumn{1}{c|}{{0.177}} & \multicolumn{1}{c|}{{0.155}} & \multicolumn{1}{c|}{{0.459}} & \multicolumn{1}{c|}{{0.373}} & \multicolumn{1}{c|}{{0.454}} & \multicolumn{1}{c|}{{0.226}} & \multicolumn{1}{c|}{{0.123}} & \multicolumn{1}{c|}{{0.137}} & {0.478} \\ \hline
\end{tabular}
}
% \caption{Detailed results of selected large size designs. Comparison of single-traversal \texttt{orchestration} with stand-alone optimizations from ABC.}
% \vspace{-3mm}
\label{table:1O}
\end{table*}

==> TCAD24-Orch/tbls/table_3o.tex <==
\begin{table*}[t]
\color{blue}
\centering
\caption{\yingjie{Detailed results of selected large size designs. Comparison of Iterative-traversal \texttt{orchestration} with corresponding sequence optimizations from ABC.}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cccccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{14}{c|}{AIG} \\ \cline{3-16} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{Baseline} & \multicolumn{1}{c|}{\texttt{rw} $\rightarrow$ \texttt{rs} $\rightarrow$ \texttt{rf}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O1}}$)} & \multicolumn{1}{c|}{\texttt{rw} $\rightarrow$ \texttt{rf} $\rightarrow$ \texttt{rs}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O2}}$)} & \multicolumn{1}{c|}{\texttt{rs} $\rightarrow$ \texttt{rw} $\rightarrow$ \texttt{rf}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O3}}$)} & \multicolumn{1}{c|}{\texttt{rs} $\rightarrow$ \texttt{rf} $\rightarrow$ \texttt{rw}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O4}}$)} & \multicolumn{1}{c|}{\texttt{rf} $\rightarrow$ \texttt{rs} $\rightarrow$ \texttt{rw}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O5}}$)} & \multicolumn{1}{c|}{\texttt{rf} $\rightarrow$ \texttt{rw} $\rightarrow$ \texttt{rs}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O6}}$)} & {Seq(\texttt{LGP})} \\ \cline{3-16} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \#Node ($\Delta$\%) \\ \hline

\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & \multicolumn{1}{c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{10288 (17.0\%)} & \multicolumn{1}{c|}{10176 (17.9\%)} & \multicolumn{1}{c|}{10230 (17.5\%)} & \multicolumn{1}{c|}{10196 (17.8\%)} & \multicolumn{1}{c|}{10263 (17.2\%)} & \multicolumn{1}{c|}{\textbf{10115 (18.4\%)}} & \multicolumn{1}{c|}{10219 (17.6\%)} & \multicolumn{1}{c|}{10493 (15.4\%)} & \multicolumn{1}{c|}{10250 (17.3\%)} & \multicolumn{1}{c|}{10793 (13.0\%)} & \multicolumn{1}{c|}{10242 (17.4\%)} & \multicolumn{1}{c|}{10788 (13.0\%)} & 10187 (17.8\%) \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{\textbf{8177 (31.6\%)}} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{\textbf{8177 (31.6\%)}} & \textbf{8129 (32.0\%)} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{22724 (17.8\%)} & \multicolumn{1}{c|}{\textbf{22503 (18.6\%)}} & \multicolumn{1}{c|}{22664 (18.0\%)} & \multicolumn{1}{c|}{22620 (18.2\%)} & \multicolumn{1}{c|}{22831 (17.4\%)} & \multicolumn{1}{c|}{22533 (18.5\%)} & \multicolumn{1}{c|}{22841 (17.4\%)} & \multicolumn{1}{c|}{23084 (16.5\%)} & \multicolumn{1}{c|}{22888 (17.2\%)} & \multicolumn{1}{c|}{24203 (12.5\%)} & \multicolumn{1}{c|}{22832 (17.4\%)} & \multicolumn{1}{c|}{24203 (12.5\%)} & 22506 (18.6\%) \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{62622 (20.8\%)} & \multicolumn{1}{c|}{61556 (22.1\%)} & \multicolumn{1}{c|}{62425 (21.0\%)} & \multicolumn{1}{c|}{62676 (20.7\%)} & \multicolumn{1}{c|}{63060 (20.2\%)} & \multicolumn{1}{c|}{61568 (22.1\%)} & \multicolumn{1}{c|}{63042 (20.3\%)} & \multicolumn{1}{c|}{64492 (18.4\%)} & \multicolumn{1}{c|}{62552 (20.9\%)} & \multicolumn{1}{c|}{68539 (13.3\%)} & \multicolumn{1}{c|}{62288 (21.2\%)} & \multicolumn{1}{c|}{68540 (13.3\%)} & \textbf{61457 (22.3\%)} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{10009 (18.1\%)} & \multicolumn{1}{c|}{\textbf{9798 (19.8\%)}} & \multicolumn{1}{c|}{9972 (18.4\%)} & \multicolumn{1}{c|}{9921 (18.8\%)} & \multicolumn{1}{c|}{10029 (17.9\%)} & \multicolumn{1}{c|}{9799 (19.8\%)} & \multicolumn{1}{c|}{9910 (18.9\%)} & \multicolumn{1}{c|}{10026 (17.9\%)} & \multicolumn{1}{c|}{9933 (18.7\%)} & \multicolumn{1}{c|}{10370 (15.1\%)} & \multicolumn{1}{c|}{9907 (18.9\%)} & \multicolumn{1}{c|}{10372 (15.1\%)} & 9815 (19.7\%)\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{10150 (20.6\%)} & \multicolumn{1}{c|}{\textbf{9904 (22.5\%)}} & \multicolumn{1}{c|}{10137 (20.7\%)} & \multicolumn{1}{c|}{10034 (21.5\%)} & \multicolumn{1}{c|}{10175 (20.4\%)} & \multicolumn{1}{c|}{9914 (22.4\%)} & \multicolumn{1}{c|}{10084 (21.1\%)} & \multicolumn{1}{c|}{10163 (20.5\%)} & \multicolumn{1}{c|}{10211 (20.1\%)} & \multicolumn{1}{c|}{10654 (16.6\%)} & \multicolumn{1}{c|}{10033 (21.5\%)} & \multicolumn{1}{c|}{10656 (16.6\%)} & 9915 (22.4\%)\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{14960 (19.1\%)} & \multicolumn{1}{c|}{14633 (20.9\%)} & \multicolumn{1}{c|}{14891 (19.5\%)} & \multicolumn{1}{c|}{14830 (19.8\%)} & \multicolumn{1}{c|}{14952 (19.1\%)} & \multicolumn{1}{c|}{\textbf{14629 (20.9\%)}} & \multicolumn{1}{c|}{14856 (19.6\%)} & \multicolumn{1}{c|}{14962 (19.1\%)} & \multicolumn{1}{c|}{14743 (20.3\%)} & \multicolumn{1}{c|}{15654 (15.3\%)} & \multicolumn{1}{c|}{14710 (20.4\%)} & \multicolumn{1}{c|}{15656 (15.3\%)} & 14676 (20.6\%)\\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & \multicolumn{1}{c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{25914 (10.4\%)} & \multicolumn{1}{c|}{25750 (10.9\%)} & \multicolumn{1}{c|}{25839 (10.6\%)} & \multicolumn{1}{c|}{25945 (10.3\%)} & \multicolumn{1}{c|}{26015 (10.0\%)} & \multicolumn{1}{c|}{25818 (10.7\%)} & \multicolumn{1}{c|}{25931 (10.3\%)} & \multicolumn{1}{c|}{26163 (9.5\%)} & \multicolumn{1}{c|}{25871 (10.5\%)} & \multicolumn{1}{c|}{27373 (5.3\%)} & \multicolumn{1}{c|}{25827 (10.7\%)} & \multicolumn{1}{c|}{27375 (5.3\%)} & \textbf{25727 (11.0\%)} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{25269 (10.6\%)} & \multicolumn{1}{c|}{25093 (11.2\%)} & \multicolumn{1}{c|}{25208 (10.8\%)} & \multicolumn{1}{c|}{25281 (10.5\%)} & \multicolumn{1}{c|}{25377 (10.2\%)} & \multicolumn{1}{c|}{25119 (11.1\%)} & \multicolumn{1}{c|}{25312 (10.4\%)} & \multicolumn{1}{c|}{25566 (9.5\%)} & \multicolumn{1}{c|}{25250 (10.6\%)} & \multicolumn{1}{c|}{26861 (4.9\%)} & \multicolumn{1}{c|}{25175 (10.9\%)} & \multicolumn{1}{c|}{26861 (4.9\%)} & \textbf{25052 (11.3\%)} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{24751 (10.7\%)} & \multicolumn{1}{c|}{24568 (11.3\%)} & \multicolumn{1}{c|}{24688 (10.9\%)} & \multicolumn{1}{c|}{24818 (10.4\%)} & \multicolumn{1}{c|}{24802 (10.5\%)} & \multicolumn{1}{c|}{24607 (11.2\%)} & \multicolumn{1}{c|}{24757 (10.6\%)} & \multicolumn{1}{c|}{24984 (9.8\%)} & \multicolumn{1}{c|}{24733 (10.7\%)} & \multicolumn{1}{c|}{26191 (5.5\%)} & \multicolumn{1}{c|}{24718 (10.8\%)} & \multicolumn{1}{c|}{26209 (5.4\%)} & \textbf{24553 (11.4\%)}\\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{26890 (10.4\%)} & \multicolumn{1}{c|}{26708 (11.0\%)} & \multicolumn{1}{c|}{26833 (10.6\%)} & \multicolumn{1}{c|}{27001 (10.0\%)} & \multicolumn{1}{c|}{26962 (10.1\%)} & \multicolumn{1}{c|}{26738 (10.9\%)} & \multicolumn{1}{c|}{26942 (10.2\%)} & \multicolumn{1}{c|}{27188 (9.4\%)} & \multicolumn{1}{c|}{26854 (10.5\%)} & \multicolumn{1}{c|}{28494 (5.0\%)} & \multicolumn{1}{c|}{26810 (10.6\%)} & \multicolumn{1}{c|}{28480 (5.1\%)} & \textbf{26700 (11.0\%)} \\ \hline


\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & \multicolumn{1}{c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{40965 (28.4\%)} & \multicolumn{1}{c|}{40869 (28.6\%)} & \multicolumn{1}{c|}{40965 (28.4\%)} & \multicolumn{1}{c|}{40866 (28.6\%)} & \multicolumn{1}{c|}{41006 (28.4\%)} & \multicolumn{1}{c|}{40874 (28.6\%)} & \multicolumn{1}{c|}{41004 (28.4\%)} & \multicolumn{1}{c|}{51414 (10.2\%)} & \multicolumn{1}{c|}{41142 (28.1\%)} & \multicolumn{1}{c|}{56224 (1.8\%)} & \multicolumn{1}{c|}{41104 (28.2\%)} & \multicolumn{1}{c|}{56222 (1.8\%)} & \textbf{40849 (28.6\%)}\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{207340 (3.3\%)} & \multicolumn{1}{c|}{206559 (3.6\%)} & \multicolumn{1}{c|}{207343 (3.3\%)} & \multicolumn{1}{c|}{211283 (1.4\%)} & \multicolumn{1}{c|}{207320 (3.3\%)} & \multicolumn{1}{c|}{\textbf{206539 (3.6\%)}} & \multicolumn{1}{c|}{206648 (3.6\%)} & \multicolumn{1}{c|}{207240 (3.3\%)} & \multicolumn{1}{c|}{206671 (3.6\%)} & \multicolumn{1}{c|}{211991 (1.1\%)} & \multicolumn{1}{c|}{206671 (3.6\%)} & \multicolumn{1}{c|}{211991 (1.1\%)} & \textbf{206530 (3.6\%)}\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{46177 (1.4\%)} & \multicolumn{1}{c|}{45650 (2.5\%)} & \multicolumn{1}{c|}{46013 (1.8\%)} & \multicolumn{1}{c|}{46005 (1.8\%)} & \multicolumn{1}{c|}{46171 (1.4\%)} & \multicolumn{1}{c|}{\textbf{45360 (3.2\%)}} & \multicolumn{1}{c|}{46039 (1.7\%)} & \multicolumn{1}{c|}{45855 (2.1\%)} & \multicolumn{1}{c|}{46113 (1.5\%)} & \multicolumn{1}{c|}{46312 (1.1\%)} & \multicolumn{1}{c|}{46077 (1.6\%)} & \multicolumn{1}{c|}{46312 (1.1\%)} & 45418 (3.0\%)\\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{19327 (21.5\%)} & \multicolumn{1}{c|}{19219 (21.9\%)} & \multicolumn{1}{c|}{19327 (21.5\%)} & \multicolumn{1}{c|}{\textbf{19218 (21.9\%)}} & \multicolumn{1}{c|}{19333 (21.5\%)} & \multicolumn{1}{c|}{19219 (21.9\%)} & \multicolumn{1}{c|}{19333 (21.5\%)} & \multicolumn{1}{c|}{19223 (21.9\%)} & \multicolumn{1}{c|}{19332 (21.5\%)} & \multicolumn{1}{c|}{23661 (3.9\%)} & \multicolumn{1}{c|}{19328 (21.5\%)} & \multicolumn{1}{c|}{23661 (3.9\%)} & \textbf{19217 (21.9\%)}\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{8755 (36.4\%)} & \multicolumn{1}{c|}{\textbf{8428 (38.7\%)}} & \multicolumn{1}{c|}{9109 (33.8\%)} & \multicolumn{1}{c|}{10306 (25.1\%)} & \multicolumn{1}{c|}{9056 (34.2\%)} & \multicolumn{1}{c|}{8612 (37.4\%)} & \multicolumn{1}{c|}{9060 (34.1\%)} & \multicolumn{1}{c|}{8589 (37.6\%)} & \multicolumn{1}{c|}{9789 (28.8\%)} & \multicolumn{1}{c|}{12440 (9.6\%)} & \multicolumn{1}{c|}{9870 (28.3\%)} & \multicolumn{1}{c|}{12440 (9.6\%)} & 8861 (35.6\%) \\ \hline

\multicolumn{3}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{\textbf{18.3\%}} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{16.8\%} & \multicolumn{1}{c|}{16.9\%} & \multicolumn{1}{c|}{\textbf{18.3\%}} & \multicolumn{1}{c|}{17.3\%} & \multicolumn{1}{c|}{15.8\%} & \multicolumn{1}{c|}{17.0\%} & \multicolumn{1}{c|}{9.7\%} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{9.7\%} & 18.2\%\\ \hline
\end{tabular}
}
% \caption{Detailed results of selected large size designs. Comparison of single-traversal \texttt{orchestration} with stand-alone optimizations from ABC.}
% \vspace{-3mm}
\label{table:3O}
\end{table*}

==> TCAD24-Orch/tbls/table_resyn.tex <==
\begin{table*}[]
\centering
\caption{{Detailed results of selected large size designs. Comparison of \texttt{orchestration}-substituted \texttt{O-resyn}/\texttt{LGP-resyn} with original \texttt{resyn} and \texttt{resyn3}.}}
\resizebox{\textwidth}{!}{%
% \subfloat[First caption]{%
% \centering

\begin{tabular}{|cccccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{14}{c|}{AIG: \texttt{resyn}} \\ \cline{3-16} 
\multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{Baseline} & \multicolumn{2}{c|}{\texttt{resyn}} & \multicolumn{2}{c|}{\texttt{resyn3}} & \multicolumn{2}{c|}{$\widehat{\texttt{O}}$\texttt{-resyn}} & \multicolumn{2}{c|}{$\widehat{\texttt{O}}$\texttt{-resyn3}} & \multicolumn{2}{c|}{${\texttt{LGP}}$\texttt{-resyn}} & \multicolumn{2}{c|}{${\texttt{LGP}}$\texttt{-resyn3}} \\ \cline{3-16} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{{Depth}} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{{Depth}} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{{Depth}} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{{Depth}} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{{Depth}} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{{Depth}} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & {Depth} \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & \multicolumn{1}{c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{36} & \multicolumn{1}{c|}{10391  (16.2\%)} & \multicolumn{1}{c|}{{25}} & \multicolumn{1}{c|}{11378  (8.2\%)} & \multicolumn{1}{c|}{28} & \multicolumn{1}{c|}{10085  (18.7\%)} & \multicolumn{1}{c|}{26} & \multicolumn{1}{c|}{{10077  (18.7\%)}} & \multicolumn{1}{c|}{{26}} & \multicolumn{1}{c|}{9988  (19.5\%)} & \multicolumn{1}{c|}{\textbf{24}} & \multicolumn{1}{c|}{\textbf{9894  (20.2\%)}} & \textbf{24} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{8518  (28.7\%)} & \multicolumn{1}{c|}{12} & \multicolumn{1}{c|}{11916  (0.3\%)} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{8177  (31.6\%)} & \multicolumn{1}{c|}{13} & \multicolumn{1}{c|}{8177  (31.6\%)} & \multicolumn{1}{c|}{13} & \multicolumn{1}{c|}{\textbf{8113  (32.1\%)}} & \multicolumn{1}{c|}{\textbf{11}} & \multicolumn{1}{c|}{\textbf{8113  (32.1\%)}} & \textbf{11} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{52} & \multicolumn{1}{c|}{23021  (16.7\%)} & \multicolumn{1}{c|}{\textbf{46}} & \multicolumn{1}{c|}{26067  (5.7\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{22046  (20.3\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{{22011  (20.4\%)}} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{21475  (22.3\%)} & \multicolumn{1}{c|}{\textbf{46}} & \multicolumn{1}{c|}{\textbf{21459  (22.4\%)}} & \textbf{46} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{132} & \multicolumn{1}{c|}{63151 (20.1\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{70808  (10.4\%)} & \multicolumn{1}{c|}{128} & \multicolumn{1}{c|}{60231  (23.8\%)} & \multicolumn{1}{c|}{131} & \multicolumn{1}{c|}{59948  (24.2\%)} & \multicolumn{1}{c|}{130} & \multicolumn{1}{c|}{58983  (25.4\%)} & \multicolumn{1}{c|}{\textbf{127}} & \multicolumn{1}{c|}{\textbf{58710  (25.7\%)}} & \textbf{127} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{66} & \multicolumn{1}{c|}{10152 (16.9\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{11013  (9.9\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{9678  (20.8\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9622  (21.3\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9464  (22.5\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{\textbf{9304  (23.9\%)}} & 65 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{10211  (20.1\%)} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{11249  (12.0\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{9790  (23.4\%)} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{9721  (23.9\%)} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{9580  (25.1\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{\textbf{9414  (26.3\%)}} & \textbf{63} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{15067  (18.5\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{16643  (10.0\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14480  (21.7\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14390  (22.2\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14137  (23.5\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{\textbf{13910  (24.8\%)}} & 65 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & \multicolumn{1}{c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{97} & \multicolumn{1}{c|}{26177  (9.5\%)} & \multicolumn{1}{c|}{\textbf{68}} & \multicolumn{1}{c|}{26543  (8.2\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25242  (12.7\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25017  (13.5\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{24989  (13.6\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{\textbf{24605  (14.9\%)}} & 69 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{92} & \multicolumn{1}{c|}{25427  (9.9\%)} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{25806  (8.7\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24681  (12.6\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24434  (13.5\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24274  (14.1\%)} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{\textbf{23945 (15.2\%)}} & \textbf{66} \\ \cline{2-16}  

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{94} & \multicolumn{1}{c|}{24930  (10.0\%)} & \multicolumn{1}{c|}{\textbf{67}} & \multicolumn{1}{c|}{25242  (8.9\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{24081  (13.1\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{23870  (13.8\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{23842  (13.9\%)} & \multicolumn{1}{c|}{\textbf{67}} & \multicolumn{1}{c|}{\textbf{23472  (15.3\%)}} & 68 \\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{93} & \multicolumn{1}{c|}{26911  (10.3\%)} & \multicolumn{1}{c|}{\textbf{67}} & \multicolumn{1}{c|}{27355  (8.8\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{26160  (12.8\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{25839  (13.9\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{25806  (14.0\%)} & \multicolumn{1}{c|}{\textbf{67}} & \multicolumn{1}{c|}{\textbf{25370  (15.4\%)}} & \textbf{67} \\ \hline

\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & \multicolumn{1}{c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40889  (28.6\%)} & \multicolumn{1}{c|}{\textbf{4359}} & \multicolumn{1}{c|}{52336  (8.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40883  (28.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40908  (28.5\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40796  (28.7\%)} & \multicolumn{1}{c|}{4369} & \multicolumn{1}{c|}{\textbf{40749  (28.8\%)}} & 4370 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{214240  (0.0\%)} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{208371  (2.8\%)} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{206529  (3.6\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{205734  (4.0\%)} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{206005 (3.9\%)} & \multicolumn{1}{c|}{{24800}} & \multicolumn{1}{c|}{\textbf{205182  (4.3\%)}} & {\textbf{24799}} \\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{{114}} & \multicolumn{1}{c|}{46611  (0.5\%)} & \multicolumn{1}{c|}{111} & \multicolumn{1}{c|}{46484  (0.8\%)} & \multicolumn{1}{c|}{{114}} & \multicolumn{1}{c|}{45676  (2.5\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{45190  (3.5\%)} & \multicolumn{1}{c|}{{114}} & \multicolumn{1}{c|}{44063  (5.9\%)} & \multicolumn{1}{c|}{{111}} & \multicolumn{1}{c|}{\textbf{42165  (10.0\%)}} & \textbf{108} \\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{19437  (21.0\%)} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{21424  (13.0\%)} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{{19219  (21.9\%)}} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{{19218  (21.9\%)}} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{\textbf{19217  (21.9\%)}} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{\textbf{19217  (21.9\%)}} & 5058 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{10446  (24.1\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{10155  (26.2\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{8411  (38.9\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{8207  (40.3\%)} & \multicolumn{1}{c|}{\textbf{57}} & \multicolumn{1}{c|}{8224  (40.2\%)} & \multicolumn{1}{c|}{\textbf{57}} & \multicolumn{1}{c|}{\textbf{8071  (41.3\%)}} & 58 \\ \hline

\multicolumn{4}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{2}{c|}{15.7\%} & \multicolumn{2}{c|}{8.9\%} & \multicolumn{2}{c|}{19.2\% (+3.5\%)} & \multicolumn{2}{c|}{19.7\% (+10.8\%)} & \multicolumn{2}{c|}{20.4\% (+4.7\%)} & \multicolumn{2}{c|}{\textbf{21.4\% (+11.5\%)}} \\ \hline

\multicolumn{4}{|c|}{{\textbf{Avg. Runtime (s)}}} & \multicolumn{2}{c|}{{0.717}} & \multicolumn{2}{c|}{{0.521}} & \multicolumn{2}{c|}{{1.148}} & \multicolumn{2}{c|}{{1.840}} & \multicolumn{2}{c|}{{1.197}} & \multicolumn{2}{c|} {{1.908}} \\ \hline
\end{tabular}%
% }
}
% \caption{Detailed results of selected large size designs. Comparison of \texttt{orchestration}-substituted \texttt{O-resyn} with original \texttt{resyn}/\texttt{resyn3}.}
%\vspace{-4mm}
\label{table:resyn}
\end{table*}




% \hfill


% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% % \subfloat[First caption]{%
% % \centering

% \begin{tabular}{|cccccccccccccccc|}
% \hline
% \multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{14}{c|}{AIG: \texttt{resyn}} \\ \cline{3-16} 
% \multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{Baseline} & \multicolumn{2}{c|}{\texttt{resyn}} & \multicolumn{2}{c|}{\texttt{resyn3}} & \multicolumn{2}{c|}{$\widehat{\texttt{O1}}$\texttt{-resyn}} & \multicolumn{2}{c|}{$\widehat{\texttt{O1}}$\texttt{-resyn3}} & \multicolumn{2}{c|}{$\widehat{\texttt{O3}}$\texttt{-resyn}} & \multicolumn{2}{c|}{$\widehat{\texttt{O3}}$\texttt{-resyn3}} \\ \cline{3-16} 
% \multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{\#Depth} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Depth} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Depth} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Depth} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Depth} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Depth} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \#Depth \\ \hline
% \multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & \multicolumn{1}{c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{36} & \multicolumn{1}{c|}{10510  (15.2\%)} & \multicolumn{1}{c|}{\textbf{26}} & \multicolumn{1}{c|}{11378  (8.2\%)} & \multicolumn{1}{c|}{28} & \multicolumn{1}{c|}{10085  (18.7\%)} & \multicolumn{1}{c|}{\textbf{26}} & \multicolumn{1}{c|}{\textbf{10078  (18.7\%)}} & \multicolumn{1}{c|}{\textbf{26}} & \multicolumn{1}{c|}{\textbf{10085  (18.7\%)}} & \multicolumn{1}{c|}{\textbf{26}} & \multicolumn{1}{c|}{\textbf{10078  (18.7\%)}} & \textbf{26} \\ \cline{2-16} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{8598  (28.0\%)} & \multicolumn{1}{c|}{14} & \multicolumn{1}{c|}{11916  (0.3\%)} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{\textbf{8177  (31.6\%)}} & \multicolumn{1}{c|}{\textbf{13}} & \multicolumn{1}{c|}{\textbf{8177  (31.6\%)}} & \multicolumn{1}{c|}{\textbf{13}} & \multicolumn{1}{c|}{\textbf{8177  (31.6\%)}} & \multicolumn{1}{c|}{\textbf{13}} & \multicolumn{1}{c|}{\textbf{8177  (31.6\%)}} & \textbf{13} \\ \cline{2-16} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{52} & \multicolumn{1}{c|}{23096  (16.5\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{26067  (5.7\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{22047  (20.3\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{\textbf{21991  (20.5\%)}} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{22070  (20.2\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{22037  (20.3\%)} & 47 \\ \cline{2-16} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{132} & \multicolumn{1}{c|}{63826 (19.3\%)} & \multicolumn{1}{c|}{\textbf{117}} & \multicolumn{1}{c|}{70808  (10.4\%)} & \multicolumn{1}{c|}{128} & \multicolumn{1}{c|}{60232  (23.8\%)} & \multicolumn{1}{c|}{131} & \multicolumn{1}{c|}{60084  (24.0\%)} & \multicolumn{1}{c|}{131} & \multicolumn{1}{c|}{60211  (23.8\%)} & \multicolumn{1}{c|}{130} & \multicolumn{1}{c|}{\textbf{60022  (24.1\%)}} & 130 \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{66} & \multicolumn{1}{c|}{10243 (16.2\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{11013  (9.9\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{9676  (20.8\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{9627  (21.2\%)}} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9686  (20.7\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9641  (21.1\%)} & \textbf{64} \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{10407  (18.6\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{11249  (12.0\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{9788  (23.4\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{9725  (23.9\%)}} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9796  (23.4\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9743  (23.8\%)} & \textbf{64} \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{15259  (17.5\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{16643  (10.0\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14480  (21.7\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{\textbf{14399  (22.1\%)}} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14492  (21.6\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14411  (22.1\%)} & 65 \\ \hline

% \multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & \multicolumn{1}{c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{97} & \multicolumn{1}{c|}{26389  (8.7\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{26543  (8.2\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25248  (12.7\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{\textbf{24975  (13.6\%)}} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25252  (12.7\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25009  (13.5\%)} & 70 \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{92} & \multicolumn{1}{c|}{25710  (9.0\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{25806  (8.7\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24685  (12.6\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24401  (13.6\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24609  (12.9\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{\textbf{24329  (13.9\%)}} & 68 \\ \cline{2-16}  

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{94} & \multicolumn{1}{c|}{25176  (9.1\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{25242  (8.9\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{24084  (13.1\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{23885  (13.8\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{24086  (13.1\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{\textbf{23868  (13.8\%)}} & 69 \\ \cline{2-16}

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{93} & \multicolumn{1}{c|}{27258  (9.1\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{27355  (8.8\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{26159  (12.8\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{25901  (13.7\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{26128  (12.9\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{\textbf{25841  (13.9\%)}} & 68 \\ \hline

% \multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & \multicolumn{1}{c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{41053  (28.3\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{52336  (8.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40883  (28.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{\textbf{40881  (28.6\%)}} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40909  (28.5\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40908  (28.5\%)} & 4372 \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{214274  (0.0\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{208371  (2.8\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{206529  (3.6\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{206527  (3.6\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{206509  (3.7\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{\textbf{206507  (3.7\%)}} & 24801 \\ \cline{2-16}

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{46738  (0.2\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{46484  (0.8\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{45690  (2.4\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{45342  (3.2\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{45391  (3.1\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{\textbf{45174  (3.5\%)}} & 114 \\ \cline{2-16}

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{19439  (21.0\%)} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{21424  (13.0\%)} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{\textbf{19219  (21.9\%)}} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{\textbf{19219  (21.9\%)}} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{\textbf{19219  (21.9\%)}} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{\textbf{19219  (21.9\%)}} & 5058 \\ \cline{2-16} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{11033  (19.8\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{10155  (26.2\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{8411  (38.9\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{8324  (39.5\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{9231  (32.9\%)} & \multicolumn{1}{c|}{\textbf{57}} & \multicolumn{1}{c|}{\textbf{8225  (40.2\%)}} & \textbf{57} \\ \hline
% \multicolumn{4}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{2}{c|}{14.8\%} & \multicolumn{2}{c|}{8.9\%} & \multicolumn{2}{c|}{19.2\% (+4.4\%)} & \multicolumn{2}{c|}{19.6\% (+10.7\%)} & \multicolumn{2}{c|}{18.8\% (+4.0\%)} & \multicolumn{2}{c|}{\textbf{19.7\% (+10.8\%)}} \\ \hline
% \end{tabular}%
% % }
% }
% \caption{Detail results of selected large designs over all benchmark suites. Comparison of \texttt{orchestration}-substituted \texttt{O-resyn} with original \texttt{resyn}/\texttt{resyn3}.}
% \vspace{-4mm}
% \label{table:resyn}
% \end{table*}




==> TCAD24-Orch/tbls/table_resyn_map.tex <==
\begin{table}[!htb]
\centering
\caption{Detailed results of selected large size designs. Comparison of technology mapping of \texttt{resyn}/\texttt{resyn3} with Best \texttt{O-resyn}. Area and delay are reported in $um^2$ and $ps$.}
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|cccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{6}{c|}{Technology mapping: \texttt{resyn}} \\ \cline{3-8} 
\multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{\texttt{resyn}} & \multicolumn{2}{c|}{\texttt{resyn3}} & \multicolumn{2}{c|}{Best \texttt{O-resyn}} \\ \cline{3-8} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & Delay \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & \multicolumn{1}{c|}{5955.75} & \multicolumn{1}{c|}{12.0} & \multicolumn{1}{c|}{6129.26} & \multicolumn{1}{c|}{\bf 11.0} & \multicolumn{1}{c|}{\textbf{5747.79}} & 12.0 \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & s35932 & \multicolumn{1}{c|}{\textbf{5282.22}} & \multicolumn{1}{c|}{\bf 5.0} & \multicolumn{1}{c|}{6193.42} & \multicolumn{1}{c|}{6.0} & \multicolumn{1}{c|}{5414.85} & {\bf 5.0} \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & b17\_1 & \multicolumn{1}{c|}{12981.71} & \multicolumn{1}{c|}{18.0} & \multicolumn{1}{c|}{14354.19} & \multicolumn{1}{c|}{\bf 17.0} & \multicolumn{1}{c|}{\textbf{12952.42}} & {\bf 17.0} \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & b18\_1 & \multicolumn{1}{c|}{36892.34} & \multicolumn{1}{c|}{\bf 54.0} & \multicolumn{1}{c|}{39672.16} & \multicolumn{1}{c|}{58.0} & \multicolumn{1}{c|}{\textbf{36264.68}} & 56.0 \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & b20 & \multicolumn{1}{c|}{5013.41} & \multicolumn{1}{c|}{25.0} & \multicolumn{1}{c|}{5117.39} & \multicolumn{1}{c|}{\bf 24.0} & \multicolumn{1}{c|}{\textbf{4718.43}} & {\bf 24.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & b21 & \multicolumn{1}{c|}{5154.01} & \multicolumn{1}{c|}{25.0} & \multicolumn{1}{c|}{5289.59} & \multicolumn{1}{c|}{\bf 24.0} & \multicolumn{1}{c|}{\textbf{4877.81}} & {\bf 24.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & b22 & \multicolumn{1}{c|}{7464.92} & \multicolumn{1}{c|}{\bf 25.0} & \multicolumn{1}{c|}{7646.79} & \multicolumn{1}{c|}{\bf 25.0} & \multicolumn{1}{c|}{\textbf{7251.37}} & {\bf 25.0} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & \multicolumn{1}{c|}{15804.08} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{15589.98} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{\textbf{14869.39}} & 29.0 \\ \cline{2-8}

\multicolumn{1}{|c|}{} & dscg & \multicolumn{1}{c|}{15378.06} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{15475.00} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{\textbf{14846.70}} & {\bf 28.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & fir & \multicolumn{1}{c|}{15709.50} & \multicolumn{1}{c|}{\bf 27.0} & \multicolumn{1}{c|}{15544.94} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{\textbf{14794.36}} & 28.0 \\ \cline{2-8}

\multicolumn{1}{|c|}{} & syn2 & \multicolumn{1}{c|}{15943.05} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{15904.37} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{\textbf{15289.84}} & {\bf 27.0} \\ \hline

\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & div & \multicolumn{1}{c|}{23828.21} & \multicolumn{1}{c|}{1452.0} & \multicolumn{1}{c|}{\textbf{19881.61}} & \multicolumn{1}{c|}{1471.0} & \multicolumn{1}{c|}{24884.07} & {\bf 1435.0} \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & hyp & \multicolumn{1}{c|}{159726.43} & \multicolumn{1}{c|}{\bf 8315.0} & \multicolumn{1}{c|}{159690.55} & \multicolumn{1}{c|}{8316.0} & \multicolumn{1}{c|}{\textbf{159446.83}} & {\bf 8315.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & mem\_ctrl & \multicolumn{1}{c|}{13098.80} & \multicolumn{1}{c|}{\bf 37.0} & \multicolumn{1}{c|}{12937.87} & \multicolumn{1}{c|}{\bf 37.0} & \multicolumn{1}{c|}{\textbf{12616.00}} & {\bf 37.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & sqrt & \multicolumn{1}{c|}{10913.79} & \multicolumn{1}{c|}{\bf 2003.0} & \multicolumn{1}{c|}{\textbf{10069.77}} & \multicolumn{1}{c|}{2018.0} & \multicolumn{1}{c|}{10218.57} & {\bf 2003.0} \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & voter & \multicolumn{1}{c|}{8692.15} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{7747.81} & \multicolumn{1}{c|}{29.0} & \multicolumn{1}{c|}{\textbf{7061.83}} & {\bf 26.0} \\ \hline
\multicolumn{2}{|c|}{\textbf{Avg. Area Reduction\%}} & \multicolumn{2}{c|}{\color{red}-4.2\%} & \multicolumn{2}{c|}{\color{red}-4.5\%} & \multicolumn{2}{c|}{ - } \\ \hline
\end{tabular}%
% }
}
% \caption{Detailed results of selected large size designs. Comparison of technology mapping of \texttt{resyn}/\texttt{resyn3} with Best \texttt{O-resyn}. Area and delay are reported in $um^2$ and $ps$.}
\vspace{-4mm}
\label{table:resyn_map}
\end{table}

==> TCAD24-Orch/tbls/table_runtime.tex <==
\iffalse
\begin{table}[!htb]
\centering
\caption{Iteration count with a single graph traversal of optimization algorithms applied to selected large size designs.}
\footnotesize
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{4}{c|}{AIG} \\ \cline{3-6}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & Ours \\ \cline{3-6} 
\multicolumn{2}{|c|}{} & \#Iteration & \#Iteration & \#Iteration & \#Iteration \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 12396 & 12277 & 12278 & \textbf{1489} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & s35932 & 11948 & 11948 & 11948 & \textbf{2014} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b17\_1 & 27518 & 27504 & 27611 & \textbf{3635} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b18\_1 & 78440 & 78485 & 78891 & \textbf{10274} \\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b20} & 12093 & 12092 & 12094 & \textbf{1259} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b21 & 12498 & 12525 & 12658 &  \textbf{1402}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b22} & 18151 & 18140 & 18418 &  \textbf{2109}\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 28904 & 28895 & 28910 &  \textbf{2340}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {dscg} & 28237 & 28238 & 28250 &  \textbf{2304}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & fir & 27689 & 27686 & 27703 &  \textbf{2357}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {syn2} & 29991 & 29990 & 30003 &  \textbf{2318}\\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 57245 & 57239 & 57235 &  \textbf{16122}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {hyp} & 214335 & 214335 & 214335 &  \textbf{7113}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & mem\_ctrl & 46836 & 46836 & 46836 &  \textbf{2602}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & sqrt & 24618 & 24617 & 24617 &  \textbf{5290}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & voter & 13697 & 13753 & 13758 & \textbf{3712} \\ \hline
\end{tabular}
% }
}
% \caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:it_count}
\end{table}
\fi

\begin{table}[!htb]
\centering
\caption{\yingjie{Counts of required iterations in a single graph traversal of optimization algorithms with selected large size designs.}}
\footnotesize
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{4}{c|}{AIG} \\ \cline{3-6}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & Ours ($\widehat{\texttt{O3}}$) \\ \cline{3-6} 
\multicolumn{2}{|c|}{} & \#Iteration & \#Iteration & \#Iteration & \#Iteration \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 12396 & 551 & 927 & \textbf{1489} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & s35932 & 11948 & 32 & 1568 & \textbf{2014} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b17\_1 & 27518 & 842 & 1825 & \textbf{3635} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b18\_1 & 78440 & 3490 & 5648 & \textbf{10274} \\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b20} & 12093 & 473 & 714 & \textbf{1259} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b21 & 12498 & 556 & 841 &  \textbf{1402}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b22} & 18151 & 705 & 1171 &  \textbf{2109}\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 28904 & 1374 & 920 &  \textbf{2340}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {dscg} & 28237 & 1433 & 826 &  \textbf{2304}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & fir & 27689 & 1449 & 831 &  \textbf{2357}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {syn2} & 29991 & 1441 & 905 &  \textbf{2318}\\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 57245 & 4539 & 285 &  \textbf{16122}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {hyp} & 214335 & 5149 & 1992 &  \textbf{7113}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & mem\_ctrl & 46836 & 123 & 102 &  \textbf{2602}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & sqrt & 24618 & 2927 & 932 &  \textbf{5290}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & voter & 13697 & 2106 & 738 & \textbf{3712} \\ \hline
\end{tabular}
% }
}
% \caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:it_count}
\end{table}

\iffalse
\begin{table}[!htb]
\centering
\caption{\yingjie{Counts of required iterations in a single graph traversal of optimization algorithms with selected large size designs.}}
\footnotesize
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{4}{*}{Design}} & \multicolumn{8}{c|}{AIG} \\ \cline{3-10}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & \multicolumn{5}{c|}{Orchestration} \\ \cline{3-10} 

 \multicolumn{2}{|c|}{} &    &   &   & &  &  &   & \\

\multicolumn{2}{|c|}{} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter \\ \end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (rw)\end{tabular}}& \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (rs)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (rf)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (none)\end{tabular}} &
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (total)\end{tabular}}\\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 12396 & 551 & 927 &   &  &  &  &\textbf{1489}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & s35932 & 11948 & 32 & 1568 &  &  &  & &\textbf{2014} \\ \cline{2-10} 
\multicolumn{1}{|c|}{} & b17\_1 & 27518 & 842 & 1825 &  &  &  & &\textbf{3635}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & b18\_1 & 78440 & 3490 & 5648 &  &  &  & & \textbf{10274} \\ \cline{2-10}
\multicolumn{1}{|c|}{} & {b20} & 12093 & 473 & 714 &   &  &  &  &\textbf{1259}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & b21 & 12498 & 556 & 841 &    &  &  & & \textbf{1402}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & {b22} & 18151 & 705 & 1171 &   &  &  &  & \textbf{2109}\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 28904 & 1374 & 920 &   &  &  &  & \textbf{2340}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & {dscg} & 28237 & 1433 & 826 &   &  &  &  & \textbf{2304}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & fir & 27689 & 1449 & 831 &   &  &  &  & \textbf{2357}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & {syn2} & 29991 & 1441 & 905 &   &  &  &  & \textbf{2318}\\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 57245 & 4539 & 285 &   &  &  &  & \textbf{16122}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & {hyp} & 214335 & 5149 & 1992 &   &  &  &  & \textbf{7113}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & mem\_ctrl & 46836 & 123 & 102 &    &  &  & & \textbf{2602}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & sqrt & 24618 & 2927 & 932 &    &  &  & & \textbf{5290}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & voter & 13697 & 2106 & 738 &   &  &  & & \textbf{3712}\\ \hline
\end{tabular}
% }
}
% \caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:it_count}
\end{table}
\fi




\iffalse
\begin{table}[!htb]
\centering
\caption{\mingju{Runtime in a single graph traversal of optimization algorithms with selected large size designs.}}
\footnotesize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{10}{c|}{AIG} \\ \cline{3-12}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & \texttt{LGP} \\ \cline{3-12} 
\multicolumn{2}{|c|}{} & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 0.107 & 0.082 & 0.067 & 0.041 & 0.044 & 0.036 & 0.033 & 0.032 & 0.033 & 0.131 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & s35932 & 0.110 & 0.072 & 0.072 & 0.050 & 0.052 & 0.041 & 0.034 & 0.033 & 0.034 & 0.136 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & b17\_1 & 0.223 & 0.155 & 0.090 & 0.077 & 0.079 & 0.073 & 0.051 & 0.055 & 0.047 & 0.306 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & b18\_1 & 0.573 & 0.340 & 0.289 & 0.237 & 0.241 & 0.215 & 0.131 & 0.130 & 0.118 & 0.878 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & b20 & 0.141 & 0.075 & 0.063 & 0.038 & 0.042 & 0.042 & 0.030 & 0.026 & 0.026 & 0.160 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & b21 & 0.147 & 0.080 & 0.066 &  0.041 & 0.042 & 0.036 & 0.028 & 0.031 & 0.033 & 0.131\\ \cline{2-12}
\multicolumn{1}{|c|}{} & b22 & 0.143 & 0.103 & 0.093 &  0.054 & 0.057 & 0.051 & 0.040 & 0.044 & 0.039 & 0.197\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 0.215 & 0.114 & 0.101 & 0.090 & 0.099 & 0.082 & 0.054 & 0.047 & 0.049 & 0.303 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & {dscg} & 0.221 & 0.124 & 0.086 & 0.104 & 0.096 & 0.092 & 0.050 & 0.051 & 0.047 & 0.310 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & fir & 0.200 & 0.125 & 0.099 & 0.090 & 0.083 & 0.088 & 0.046 & 0.052 & 0.049 & 0.309 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & {syn2} & 0.201 & 0.137 & 0.120 & 0.094 & 0.086 & 0.094 & 0.058 & 0.059 & 0.048 & 0.340 \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 0.530 & 0.244 & 0.203 & 0.345 & 0.355 & 0.346 & 0.116 & 0.116 & 0.093 & 0.737 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & {hyp} & 2.207 & 0.778 & 0.738 & 0.643 & 0.561 & 0.277 & 0.239 & 0.195 & 0.179 & 2.626 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & mem\_ctrl & 0.366 & 0.188 & 0.208 & 0.050 & 0.057 & 0.049 & 0.050 & 0.047 & 0.043 & 0.501 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & sqrt & 0.279 & 0.143 & 0.114 & 0.125 & 0.136 & 0.117 & 0.079 & 0.072 & 0.074 & 0.343\\ \cline{2-12} 
\multicolumn{1}{|c|}{} & voter & 0.188 & 0.079 & 0.075 & 0.080 & 0.074 & 0.061 & 0.054 & 0.055 & 0.044 & 0.242 \\ \hline
\end{tabular}
% }
}
% \caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:real_runtime}
\end{table}
\fi

==> approach.tex <==
\section{Approach}\label{sec:approach}

\subsection{On the Impact of DAG-Aware Synthesis Algorithms}\label{sec:algorithm}

The most efficient algorithms that optimize the Boolean networks are directed acyclic graph (DAG) aware based Boolean synthesis algorithms \cite{mishchenko:2006-dag,wolf2016yosys}, which are widely used in both open-source tools \cite{mishchenko2010abc,wolf2016yosys,luu2014vtr, neto2019lsoracle} and industrial tools \cite{cunxiyu:dac16,stok1996booledozer,DBLP:conf/iccad/YuCSC17,amaru2014majority}. Specifically, this work focuses on optimizing the synthesis flows that comprise DAG-aware synthesis algorithms and heuristics, targeting AIG- and MIG-based flows. Thus, to understand how effective each synthesis transformation (algorithm) is in the synthesis flows, we analyze the basic graph operations in DAG-aware algorithms. We showcase the number of transformed nodes for an AIG-based flow, running 6 different transformations  {(bracket 4 in the pseudo-code of the Algorithm presented in Fig. \ref{fig:motivation})}. With that, we can estimate the effectiveness of the algorithm for a given DAG (a circuit). Hence, to understand how effective each synthesis transformation (algorithm) is in the synthesis flows, we monitor the number of transformed nodes of all transformations using 100 random flows. The selected ABC synthesis transformations are the same six transformations as in \cite{DBLP:conf/dac/YuXM18,hosny2019drills}, namely $\mathbb{S}$=\{balance, restructure, rewrite, refactor, rewrite -z, refactor -z\}. We collect these results for six VTR benchmarks, as shown in Table \ref{tbl:benchmark}, and plot the average, max, min number of relative transformable nodes. While we plot the average over six designs, we observed a similar trend in all the designs. 

The analysis results are shown in Figure \ref{fig:motivation}, where the y-axis represents the relative number of transformed nodes of each transformation, and the x-axis shows the steps of the synthesis flows. For example, given a random \textit{none}-repetition flow composed by the transformations available in $\mathbb{S}$, assume the first transformation is applied to $\sim$1,000 nodes in the {original} graph and the second transformation is applied to $\sim$200 nodes in the {updated} graph. In which case, the relative percentage of the first two transformations of this example is denoted as $1$ and $0.2$. Therefore, in Figure \ref{fig:motivation}, the relative number of transformed nodes of all randoms flows start with $1$. As there are 100 random permuted flows for six designs in this analysis, the error-bars are used to indicate the upper/lower bound of transformable nodes among all the random generated flows. MIG-based transformations have a similar trend, with a particularity: the number of relative transformable nodes for the first two transformations tend to be closer. {Our intuition is that the input for MIG-based synthesis is an AIG data structure, where the nodes have at least one input as constant (true or false)}. Thus, it limits the number of applicable MIG-based transformations on the first iteration. On the other hand, the second iteration has more majority nodes, so there are still a good amount of transformable nodes for MIG-based algorithms. Thus, the observations done for AIGs also hold for MIGs. 


\begin{figure}[t]
\begin{minipage}{.24\textwidth}
\scriptsize
%\captionof{algorithm}{Euclids algorithm}\label{myalg}
\begin{algorithmic}[1]
 \Procedure{dag-aware synthesis}\;\\
  $G(\mathcal{V},\mathcal{E})$ $\gets$ circuit\;\\
 \For{$v \in \mathcal{V}$}{
 \If{\color{red} transformable($v$)}{
  {\color{red} apply transformation to $v$}\; \\
  update $G(\mathcal{V},\mathcal{E})$\;
  }
 }
 %\EndFor
 %\EndIf
 \EndProcedure
\end{algorithmic}
\end{minipage}%
\begin{minipage}{.25\textwidth}
 \centering
\includegraphics[width=1\textwidth]{./figs/motivation.pdf}
\end{minipage}
\caption{Illustration of DAG-aware synthesis algorithm. And, the {relative number} of AIG nodes that are effectively executed in each transformation of the synthesis flows, using 100 random flows with six transformations used in \cite{DBLP:conf/dac/YuXM18,hosny2019drills}.}
\label{fig:motivation}
\end{figure}

There are two important observations can be concluded empirically from the experiments: 

\begin{itemize}

\item Observation (1) \textit{The earlier transformations selected in a given synthesis flow have the highest impacts to the Boolean optimization problem w.r.t DAG-aware logic transformations.}

\end{itemize}

In Figure \ref{fig:motivation}, we can see that for any random flow, the third to sixth transformations in the flow are applied to less than 10\% nodes compared to the first transformation. In this particular example, we observe many cases that the fifth and sixth transformations do not detect any transformable node, regardless of the permutations. 

\begin{itemize}

\item Observation (2) \textit{Earlier transformations in the synthesis flow dominates the performance of Boolean optimizations since the transformable nodes for the rest of the flow are determined by earlier transformations (local minima).}

\end{itemize}

That being said, starting a synthesis flow with an unsuccessful transformation will almost certainly result in an inefficient flow, regardless of how the other optimizations are permuted. This is also true for MIGs, because the first transformation sets the topology of the real MIG graph, influencing the efficacy of subsequent MIG-based transformations. As a result, having the first transformation bias the flow is equivalent to solving a non-convex optimization problem with an initialization that always converges at a suboptimal local optimum. We may conclude from the suggested experiment that the performance of synthesis flows for DAG-based transformations is dominated by the first transformation in the flow. With these two observations in mind, we propose a domain-knowledge MAB approach for automatic logic synthesis flow generation. 

% The main reason is that the DAG-aware synthesis algorithms are mostly implemented based on structural search. The performance of such algorithms heavily relies on the structure of a given DAG. As indicated in the first observation, the structure of the graph will be dominated by the first transformation. Thus, we can say that the first transformation in the flow dominates the performance of synthesis flows. With these two observations in mind, we propose a domain-knowledge Multi-Armed Bandits (MAB) approach for automatic logic synthesis flow generation. 

\noindent
\textbf{Example 1:} An illustrative example that demonstrates the importance of the extracted algorithmic domain knowledge presented in Figure \ref{fig:motivation} is shown in Table \ref{tbl:ex1}. Two DAG-aware synthesis transformations from ABC are selected to build two different flows $F_0$ and $F_1$ and are applied to design \texttt{bfly} from VTR \cite{luu2014vtr} benchmark. We focus on comparing the transformed AIG nodes (\#TNodes) of \texttt{rewrite} and the final number of AIG nodes. This is because \texttt{rewrite} performs a technology-independent rewriting algorithm of AIG, which offers the main reductions of \#AIG in this example. We can see that \textbf{(1)} \textit{The transformations at the early stage of the flows have more impacts than the transformations at the late stage.} For example, in both flows, first \texttt{rewrite} successfully applies to more than 7$\times$ \#AIG than the second \texttt{rewrite}. \textbf{(2)} \textit{The choice of early transformations has significant impacts on the performance of the flow}. Early transformations have more impacts on the Boolean network, so the DAG structure could change dramatically at the early stage compared to the late stage. For example, if we apply \texttt{balance} first, the first \texttt{rewrite} in $F_0$ applies to 951 nodes. On the other hand, without \texttt{balance}, the first  \texttt{rewrite} can be applied to 1764 nodes at ($F_1$). Similar results can be observed from the remaining two \texttt{rewrite}.

\begin{table}[t]
\caption{Example of the algorithmic domain knowledge presented in Figure \ref{fig:motivation} using ABC synthesis transformation \textit{rewrite} rw and \textit{balance} (b) with design {bfly} from VTR 8.0 \cite{luu2014vtr} benchmark. Note that rw is technology-independent rewriting of the AIG which offers the main AIG reductions in $F_0$ and $F_1$. \#TNodes = Number of AIG nodes transformed by the corresponding AIG transformation.}
\begin{tabular}{cccccccc}
\textit{$F_0$} & \textit{b} & \textit{rw} & \textit{b} & \textit{rw} & \textit{b} & \textit{rw} & Final \#AIG \\
\textit{\#TNodes} & 817 & \textbf{951} & 825 & \textbf{169} & 831 & \textbf{64} & 26339 \\ \hline\hline
\textit{$F_1$} & \textit{rw} & \textit{b} & \textit{rw} & \textit{b} & \textit{rw} & \textit{b} & Final \#AIG \\
\textit{\#TNodes} & \textbf{1764} & 824 & \textbf{290} & 834 & \textbf{90} & 832 & \textbf{26182}
\end{tabular}
\label{tbl:ex1}
\end{table}

\noindent
\textbf{Example 2:} Now, we show the importance of getting the right transformation for MIG-based synthesis, according to our discussion on MIG-based synthesis trends in Figure \ref{fig:motivation}. The experiment is depicted in Table \ref{tbl:ex2}. 
We select two area-oriented (nodes reduction) transformation to this end, so we aim to highlight the effectiveness of picking a right transformation at the 1st iteration to the overall circuit area (DAG size) reduction. 
Similarly to the previous example, we use two transformations (resub and refactor) to build two different flows $F_0$ and $F_1$. These flows are applied to the same design (\texttt{bfly}) as the previous example. Note that we do not intend to compare the effectiveness of AIG vs MIG based synthesis with this experiment, but rather show the importance of leveraging domain-knowledge for automatic flow generation. 
As in the previous example, we can see that \textbf{(1)} \textit{The transformations at the early stage of the flows have more impacts than the transformations at the late stage.} Also, as we discussed, we can see that for MIG-based, effective flows tend to have a similar number of transformable nodes for the first two transformations, as the first transformation actually defines the actual MIG structure.  
\textbf{(2)} \textit{The choice of early transformations has significant impacts on the performance of the flow}. In this case, the same observation as we did for AIGs hold for MIGs, and the early transformations have more impacts. 

\begin{table}[t]
\caption{Example of the algorithmic domain knowledge presented in Figure \ref{fig:motivation} using MIG-based synthesis transformation \textit{refactor} (rf) and \textit{resub} (rs) with design {bfly} from VTR 8.0 \cite{luu2014vtr} benchmark. We use these transformations as they are area-oriented within the LSOracle flow, and can highlight the importance of picking the right transformation w.r.t the effectiveness of transformable and reduced nodes. \#TNodes = Number of MIG nodes transformed by the corresponding MIG transformation.}
\begin{tabular}{cccccccc}
\textit{$F_0$} & \textit{rf} & \textit{rs} & \textit{rf} & \textit{rs} & \textit{rf} & \textit{rs} & Final \#MIG \\
\textit{\#TNodes} & 984 & 931 & 87 & 44 & 3 & 1 & \textbf{26659} \\ \hline\hline
\textit{$F_1$} & \textit{rs} & \textit{rf} & \textit{rs} & \textit{rf} & \textit{rs} & \textit{rf} & Final \#MIG \\
\textit{\#TNodes} & 1402 & 377 & 74 & 15 & 4 & 1 & 26779
\end{tabular}
\label{tbl:ex2}
\end{table}



\vspace{-3mm}
\subsection{Domain-specific MAB Formulation}\label{sec:mab}

An online program must choose from a set of strategies in a sequence of $n$ trials to maximize the overall payout of the chosen strategies in a multi-armed bandit problem. Such challenges require that a set quantity of resources must be distributed among accessible options in such a way that the expected gain of a given objective is maximized. These are the most important theoretical tools for modeling the exploration-exploitation trade-offs that are inherent in sequential decision-making under uncertainty. Specifically, MAB process is represented as a tuple of $<\mathcal{A},\mathcal{R}>$, where:

{\it
\begin{itemize}
\item $\mathcal{A}$ is a known set of available choices (arms).
\item At each time step $t$, an action $a_t$ is triggered by choosing with one of the choice $a_t \in \mathcal{A}$. 
\item $\mathcal{R}$ is a reward function and $\mathcal{R}^{a_t}$ is the reward at time step $t$ with action $a_t$.
\item The objective of bandit algorithm is to maximize $\textstyle \sum^{t}_{i} \mathcal{R}^{a_t}$
\end{itemize}
}

In a classic MAB sequential decision-making environment, the available decisions at time step $t$ are considered as arms. For example, considering the synthesis flow exploration problem, the selected synthesis transformations will be the set of arms $\mathcal{A}$. Let $\mathcal{A}$ include eight unique transformations $\mathcal{A}$=\{\texttt{resub,rewrite,...,refactor}\}. Let $\mathcal{R}$ be the number of AIG nodes that have been reduced by applying the transformations, such that the objective of the bandit algorithm is to maximize $\textstyle \sum^{t}_{i} \mathcal{R}^{a_t}$, i.e., minimize the number of AIG nodes. Let $F$ be a decision sequence, where $F$=\{$a_0, a_1,..., a_n$\}, $a_t \in \mathcal{A}$. This decision sequence $F$ is a synthesis flow. %
%
A brute-force approach to identifying the optimum flow that maximizes the benefit $F$ performs enough rounds with each transformation (each arm) to determine the true probability of reward. Unfortunately, a brute-force method like this is impractical. In this situation, the bandit algorithm's principal goal is to gather enough data to make the best overall decisions. According to prior plays, the best-known option is chosen during exploitation. The exploration phase will look into unknown choices inside the search space in order to gain more information and close the gap between estimated and true reward function probabilities. This process is analogous to reinforcement learning for synthesis flow exploration without internal states, such as a snapshot of current Boolean network statistics. Despite the fact that MAB sequential decision making is extensively used, it needs to be rethought to fit in with logic synthesis flow exploration. In particular, according to the two observations in Section \ref{sec:algorithm}: 

\begin{itemize}

\item Since the first synthesis transformation dominates the flow, the first action in exploration will dominate the true reward distribution $\mathcal{R}^{*}$ and the exploitation reward distribution $\mathcal{R}$. In other words, the initialization of the bandit algorithm dominates the gap between $\mathcal{R}^{*}$ and $\mathcal{R}$.  

\item While considering each transformation as an arm, each action corresponds to applying one synthesis transformation to the logic graph. Unlike the classic MAB problem that $\mathcal{R}^{*}$ is fixed over time, $\mathcal{R}^{*}$ in synthesis flow exploration changes at each time step, as the logic graph is updated by the transformation.

\end{itemize}



Therefore, to gather the domain knowledge of synthesis algorithms discussed in Section \ref{sec:algorithm}, we propose a novel MAB environment by re-defining the arms and actions, which fits the logic synthesis flow exploration problem. Thus, let $P(\mathcal{X})$ be a random permutation function over a set of decisions $\mathcal{X}$. Let $P(x|\mathcal{X})$ be a random permutation function over the set $\mathcal{X}$, $x \in \mathcal{X}$, such that $P(x_i|\mathcal{X})$ is a random permutation with $x_i$ always being the first element in the permutation, $P(x_i|\mathcal{X}) \in P(\mathcal{X})$. We define $P(x|\mathcal{X})$ to be the arms in the MAB environment, such that $\mathcal{A}$=\{$P(x_0|\mathcal{X})$,~$P(x_1|\mathcal{X})$,~...,~$P(x_n|\mathcal{X})$~\}, where $n$ is the number of available decisions in the exploration problem. Specifically, $n$ corresponds to the number of available synthesis transformations. \textbf{Unlike using traditional MAB algorithms, an action $a_t$ at time $t$ is a sampled permutation from $P(x_i|\mathcal{X})$.} In other words, $a_t$ is a \textit{multiset} over the set $\mathcal{X}$. Let $Q(a_t)$ be the action value that is obtained by applying $a_t$ to a given Boolean network at $t$ time step, the reward is $r_t$
%\begin{equation}
\[
r_t = Q(a_t) - Q(a_{t-1}) \implies Q(P(x_i|\mathcal{X})) - Q(P(x_j|\mathcal{X}))
\]
where the $i^{th}$ arm is played at $t$ time step and $j^{th}$ arm is played at $t-1$ time step, {and $Q(a) = \mathop{\mathbb{E}}(p|a)$ calculates the mean reward (e.g., number of AIGs minimized) from the actions at $t$ step over the estimated winning probabilities $p$}. Finally, we use upper confidence bound (UCB) bandit algorithm as the agent, such that $a_t$ is chosen with estimated upper bound $U_t(a)${, where setting the probability of the true mean being greater than the UCB to be less than or equal to $t^{-1}$, also known as UCB1 algorithm \cite{auer2002finite}. The adopted upper bound can be calculated using \textit{Lai and Robbins} theorem \cite{lai1985asymptotically} and the Hoeffding’s inequality. According to the Hoeffding’s inequality the probability of choosing an action exceeds upper confidence bound (UCB) is bounded by
\begin{equation}
    P[Q(a) > Q_{t}(a) + U_{t}(a)] \leq e^{-2N_{t}(a)U_{t}(a)^{2}}
\end{equation}

In other words, using Hoeffding’s inequality to assign an upper bound to an arm’s mean reward where there is high probability that the true mean will be below the UCB assigned by the algorithm. 

Therefore, while solving $U_t(a)$ in UCB,
\begin{equation}
    e^{-2N_{t}(a)U_{t}(a)^{2}} = p \Rightarrow U_{t}(a) = \sqrt{\frac{-log~p}{2N_{t}(a)}}
\end{equation}
In this case, we can see that reducing the probability of $p$ will increase the rewards from UCB. Setting the probability $p$ of the true mean being greater than the UCB to be less than or equal to $t^{-4}$, a small probability that quickly converges to zero as the number of rounds $t$ grows, which is also known as UCB1 algorithm. However, we find that setting $p=t^{-1}$ is sufficient based on our empirical studies, which results in 
\cite{auer2002finite}.

\begin{equation}
    \sqrt{\frac{-log~p}{2N_{t}(a)}} = \sqrt{\frac{log~t}{2N_{t}(a)}} = \sqrt{\frac{t}{2N_{t}(a)}}, ~~ \text{let} ~ p=t^{-1}
\end{equation}
Thus, we get the following:

\begin{equation}
    a_{t} = \underset{a \in \mathcal{A}}{\mathrm{argmax}}\, \left[ Q(a) + U_{t}(a) \right], ~~ U_{t}(a) = \sqrt{\frac{log~ t}{2N_{t}(a)}}
\end{equation}

% The adopted upper bound can be defined as follows w.r.t \textit{Lai and Robbins} theorem \cite{lai1985asymptotically}}:

%{
% \[
% a_t = \mathop{\mathrm{arg\,max}}_{a \in \mathcal{A}} \left[ Q(a) + U_t(a) \right], U_t(a)=\sqrt{\frac{log~t}{2N_t(a)}}
% \]
}


%\end{equation}

The performance of a multi-armed bandit algorithm is often evaluated in terms of its regret, defined as the gap between the expected payoff of the algorithm and that of an optimal strategy. In this work, the number of regrets equals to the number of synthesis flows that have been evaluated in the synthesis tool. Using the UCB algorithm, an asymptotic logarithmic total regret $L_t$ is achieved \cite{auer2002finite}:

\[
 \lim_{t \to \infty} L_t = 2log~t~\sum \Delta_{a}
\]
where $\Delta_{a}$ is the differences between arms in $\mathcal{A}$.

\begin{figure}[b]
\centering
\includegraphics[width=0.4\textwidth]{./figs/multi-stage-mab.pdf}
\caption{Illustration of the proposed multi-stage bandit approach with four stages.}
\label{fig:multistage}
\vspace{-2mm}
\end{figure}





\subsection{Improving Convergence with Multi-stage Bandit}



While the preceding section's technique relies on optimistic initialization, we suggest a multi-stage bandit to further improve convergence. We can see that the single-stage approach may be used to longer synthesis flows, with each transformation being performed numerous times, based on the formulation in the previous section. However, increasing the length of the sequences leads to a significant increase in the number of explorations required to close the gap between the optimistic reward distribution $\mathcal{R}^*$ and exploitation reward distribution $\mathcal{R}$. Moreover, the optimistic reward distribution $\mathcal{R}^*$ changes as the synthesis transformations are applied to the logic circuit, since the graph structure is modified iteratively. Finally, while synthesis transformations are less successful at late time steps, fine-grain exploration can have a significant impact on EDA flows later on, such as technology mapping and gate sizing.


\begin{figure*}[t]
\centering
\includegraphics[width=0.85\textwidth]{TCAD21-FlowTune/figs/TCAD_Flow_Chart-crop.pdf}
\caption{Overview of the proposed end-to-end MAB synthesis system -- Using ABC front-end, our system accepts technology mapped netlist, Boolean logic netlist, and LUT-netlist. The system is also integrated with VTR 8.0 and Yosys, which enable synthesis optimization for a large range of objectives for designing ASICs and FPGAs, and formal verification tools.}
\label{fig:system_overview}
\end{figure*}


In this context, we introduce the proposed MAB algorithm using a four-stage example shown in Figure \ref{fig:multistage}. Each stage in the multi-stage approach uses the same domain-specific bandit algorithm described in Section \ref{sec:algorithm}. Within each stage, the MAB algorithm is restricted to a fixed number of iterations $m$. Once the first stage is completed, the exploitation reward distribution $\mathcal{R}^1$ is updated (stage 1 in Figure \ref{fig:multistage}), in which a higher rate indicates a higher chance of gaining reward by playing that arm. After $m$ iterations in the first stage, the best-explored synthesis flow will be applied to the input logic circuit, and the synthesized circuit will be the input circuit for the next stage. Rather than starting a new MAB agent with a uniform distribution, we start the second stage using the reward distribution of the first stage's top two arms. For example, in Figure \ref{fig:multistage}, $\mathcal{R}^{1}_{a_0}$ and $\mathcal{R}^{1}_{a_1}$ will be merged and used as the initial reward distribution for the second stage, where $\mathcal{R}^{1}_{a_0}, \mathcal{R}^{1}_{a_1} \in \mathcal{R}^{1}$. This procedure will continue until the $s$ stages have been completed. As we can see, the total number of explorations is $s \cdot m$. In this work, we have explored five different options for ($s,m$), while maintaining the total number of iterations identical.


\noindent
\textbf{Example 2}: We present an illustrative example of the aforementioned domain-specific MAB and the multi-stage bandit algorithm for exploring synthesis flows using the following ABC transformations: \texttt{rw, b, rf,} and \texttt{resub}. Let $\mathcal{X}$ be \{\texttt{4$\times$rw, 4$\times$b, 4$\times$rf, 4$\times$resub}\}. Let the number of stages for exploration be four, such that $\mathcal{X}_{0,1,2,3}=$\{\texttt{rw, b, rf, resub}\}. At first MAB stage, arms $\mathcal{A}_0$
%$\mathcal{A}_0$=\{$P(rw|\mathcal{X}_0)$, ~$P(rf|\mathcal{X}_0)$, ~...,~$P(resub|\mathcal{X}_0)$~\}.
\vspace{-1mm}
\begin{align}
\tiny 
\mathcal{A}_0=\{P(rw|\mathcal{X}_0), 
P(b|\mathcal{X}_0),
P(rf|\mathcal{X}_0),
P(resub|\mathcal{X}_0)~\}
\end{align}
are explored with the proposed MAB algorithm presented in Section \ref{sec:algorithm}. The reward $r_t$ is calculated based on the target objective, e.g., number of reduced AIG nodes compared to the existing best actions. Next, Stage 1 terminates after a fixed number of iterations, and returns the arm(s) with the highest reward value. For the sake of simplicity, this example only includes the arm with the highest reward for stage 2. Let us assume $P(rw|\mathcal{X}_0)$ and $P(rf|\mathcal{X}_0)$ return the highest reward at stage 1. We then define $\mathcal{A}_0^*=\{P(rw|\mathcal{X}_0),P(rf|\mathcal{X}_0)\}$, the arms for second stage, $\mathcal{A}_1$, are updated as follows:
\begin{align}
\tiny 
\mathcal{A}_1=\{\mathcal{A}_0^* \frown  P(rw|\mathcal{X}_1), ~...,\mathcal{A}_0^* \frown  P(resub|\mathcal{X}_1)~\}
\end{align}
where the sample from each arm in $\mathcal{A}_1$ will be a concatenation of two actions from $\mathcal{A}_0^*$ and $P$. For stage 3, we simply replace $\mathcal{A}_0^*$ with $\mathcal{A}_1^*$, which will be the highest reward arms from $\mathcal{A}_1$. Finally, note that the subsets $\mathcal{X}_{0,1,2,3}$ are not necessary to be equally defined. For example, we can define $\mathcal{X}_0$= \{2$\times$\texttt{rw,b,rf,resub}\}, $\mathcal{X}_{1,2}=$\{\texttt{rw, b, rf, resub}\}, and $\mathcal{X}_3$=\{\texttt{b,rf,resub}\}.











\section{FlowTune Framework}

\subsection{Initialization}

As we discussed, the initialization step is crucial for MAB-based exploration performance. We leverage the domain knowledge of DAG-aware synthesis algorithms in our initialization stage. Specifically, for our multi-stage MAB exploration approach, we initialize the reward value for each arm in the first stage using the total number of transformable nodes by sampling each arm. While as demonstrated in Example 1, the total number of transformable nodes for a sequence of transformations highly depends on the first transformation, the initialization involves only one sampling of each arm. More importantly, this scheme significantly reduces the runtime of initialization for objectives such as technology mapping, since counting the number of transformable nodes does not require the actual mapping process. The initialization process is used at the beginning of each stage. To further improve the speed of initialization, we implement a parallel sampling function using OpenMP library \cite{chandra2001parallel}.

%\input{./figs/result_aig.tex}
%\input{./figs/result_fpga.tex}


\subsection{System Integration}

The proposed approach, namely \textit{FlowTune}, is implemented in ABC and LSOracle \cite{lso}. Using the I/O interfaces of ABC and LSOracle, \textit{FlowTune} can take as input logic networks in various formats such as Verilog, AIG, and BLIF. The system overview is shown in Figure \ref{fig:system_overview}. On the ABC side, besides integrating \textit{FlowTune} with logic transformations, we also integrated it with two technology mappers, i.e., \texttt{'map'} for standard-cell mapping, and \texttt{'if'} for FPGA mapping. %We present the effectiveness of \textit{FlowTune} in reducing the number of AIG nodes, as well as the number of LUTs after mapping. 
Similarly, for MIG evaluation, \textit{FlowTune} was integrated with LSOracle for both logic transformations and a native MIG LUT-mapper, the \texttt{'lut\_map'} command. 
For an accurate evaluation of \textit{FlowTune}, we perform post-technology mapping ASIC evaluation, using ABC + Genus for STA, and end-to-end FPGA evaluation in two different contexts: (i) using ABC + VTR as backend targeting a Stratix IV like architecture, and (ii) using LSOracle + OpenFPGA as back-end, also targeting a Stratix IV like architecture. %All the metrics are collected post-place and route, and we take as input for VTR optimized networks through ABC (for AIGs), and for OpenFPGA optimized networks with LSOracle (for MIGs). 
%Thus, for ASICs the timing and area results after standard-cell mapping are generated by reading the mapped Verilog produced by ABC in Cadence Genus, with the predictive ASAP 7nm liberty \cite{xu2017standard}. We also evaluate applying \textit{FlowTune} for CNF clauses minimization. The size of CNF formulations is important to reduce the runtime of Boolean SAT solving, which has been widely applied in verification \cite{moskewicz2001chaff,ciesielski2015verification}, security \cite{yu2017incremental,subramanyan2015evaluating} and reasoning \cite{mcmillan2003interpolation}. 
%To this end, we use \texttt{write\_cnf} function in ABC that dumps AIGs into CNF format. 
% Finally, for an end-to-end FPGA evaluation, we apply \textit{FlowTune} in two different contexts: (i) using the ABC interface built-in Yosys to generate mapped LUT-netlist, we evaluate \textit{FlowTune} in Xilinx Vivado targeting Kintex UltraScale device; (ii) using OpenFPGA and VTR as back-end, we evaluate \textit{FlowTune} targeting a Stratix IV like architecture. All the metrics are collected post-place and route, and we take as input for VTR optimized networks through ABC (for AIGs), and for OpenFPGA optimized networks with LSOracle (for MIGs). 


==> background.tex <==
%\section{Current state of research in the field}


\vspace{-3mm}
\section{Background}

This section presents useful notations for the reader, as well as reviews the search space while generating synthesis flows. We then present a motivational example on how delay and area may vary with synthesis flow, and how these gains are comparable w.r.t the state-of-the-art. 

\subsection{Notations and Search Space}\label{sec:space}

\noindent
\textbf{Definition 1 \textit{none}-repetition Synthesis Flow}: \textit{Given a set of unique synthesis transformations $\mathbb{S}$=\{$p_0$, $p_1$,..., $p_n$\}, a synthesis flow $\mathbb{F}$ is a permutation of $p_i$ $\in$ $\mathbb{S}$ performed iteratively.} 


%\noindent
\textbf{Example 1:} Let $\mathbb{S}$=\{$p_0$, $p_1$, $p_2$\}. $p_i$ are the transformations in the synthesis tools and can be processed independently. Then, there are totally six flows available: 

\vspace{0mm}
\begin{equation*}
\small
\begin{aligned}
F_0 : p_0 \rightarrow p_1 \rightarrow p_2 ~~
F_1 : p_0 \rightarrow p_2 \rightarrow p_1 \\
F_2 : p_1 \rightarrow p_0 \rightarrow p_2 ~~
F_3 : p_1 \rightarrow p_2 \rightarrow p_0 \\
F_4 : p_2 \rightarrow p_0 \rightarrow p_1 ~~
F_5 : p_2 \rightarrow p_1 \rightarrow p_0
\end{aligned}
\end{equation*}


\textbf{Remark 1}: \textit{Let $f(n,1)$ be the upper bound number of possible flows, where $\mathbb{S}$ includes $n$ elements, and each transformation appears only once, such that:}

\vspace{-2mm}
\begin{align}
\small
f(n,1) = n!
\end{align}

The upper bound of $\mathbb{N}$ happens \textit{iff} all elements in $\mathbb{S}$ can be processed independently. In practice, there could be some constraints to be satisfied for processing these transformations. In this case, $\mathbb{N}$ will be smaller than $n!$. For example, given a constraint that $p_1$ has to be processed before $p_2$, the available flows include only $F_0$, $F_2$, and $F_3$.

\textbf{Definition 2 $m$-repetition Synthesis Flow (m$\geq$2)}: \textit{Given a set of unique synthesis transformations $\mathbb{S}$=\{$p_0$, $p_1$,...,$p_n$\}, a synthesis flow with $m$-repetition $\mathbb{F}_{m}$ is a permutation of $p_i$ $\in$ $\mathbb{S}_{m}$, where $\mathbb{S}_{m}$ contains $m$ $\mathbb{S}$ sets.} 

\textbf{Example 2:} Let $\mathbb{S}$=\{$p_0$, $p_1$\}. Each $p_i$ can be processed independently. For developing $2$-repetition synthesis flows, $\mathbb{S}_{2}$=\{$p_0$, $p_1$, $p_0$, $p_1$\}. The available flows include:

\vspace{-2mm}
\begin{equation*}
\small
\begin{aligned}
F_0 : p_0 \rightarrow p_0 \rightarrow p_1 \rightarrow p_1~~
F_1 : p_1 \rightarrow p_1 \rightarrow p_0 \rightarrow p_0 \\
F_2 : p_0 \rightarrow p_1 \rightarrow p_0 \rightarrow p_1~~
F_3 : p_1 \rightarrow p_0 \rightarrow p_1 \rightarrow p_0 \\
F_4 : p_0 \rightarrow p_1 \rightarrow p_1 \rightarrow p_0~~
F_5 : p_1 \rightarrow p_0 \rightarrow p_0 \rightarrow p_1 \\
\end{aligned}
\end{equation*}




\textbf{Remark 2}: \textit{Let $\mathbb{L}$ be the length of a synthesis flow. Given a  $m$-repetition $\mathbb{F}_{m}$ with $n$ transformations in $\mathbb{S}$, $\mathbb{L}$ = $n$$\times$$m$.}

The search space for $m$-repetition flows is a \textit{multiset} permutation problem. Hence, a closed formula can be derived to describe the search space of $m$-repetition flows. The search space of $m$-repetition flows with $n$ unique transformations is shown in Equation \ref{eq:space1}.

\textbf{Remark 3}: \textit{Let function $f(n,m)$ be upper bound number of available $m$-repetition flows with $n$ elements in $S$. $f(n,m)$ uniquely satisfies the following formula :}%\cite{mendelson1981permutations}


\begin{align}
\small
\begin{aligned}
f(n,m) = \dfrac{(n\cdot m)!}{(m!)^n}
%where \mathbb{L} > m, m = 2,3,...
\end{aligned}
\label{eq:space1}
\end{align}

With the multiset permutation concept, Yu et al. \cite{DBLP:conf/dac/YuXM18} generalized the formula to describe the search space for any type of \textit{m-}repetition flows. {Let $n$ be the number of unique transformation, the $M$-repetition flows, $M$=\{$m_{0}, m_{1}, ...,m_{n-1}$\}, where $m_i$ is the number of repetitions of the $i^{th}$ transformation}. The total number of possible flows is shown in Equation 2. 

\textbf{Remark 4}: {\textit{Let function $f(n,\mathbb{L},\{m_{0}, m_{1}, ...,m_{n-1}\})$ be upper bound number of flows with $n$ elements in $S$}. The $i^{th}$ element in $S$ appears $m_i$ times. The function uniquely satisfies the following formula :}%\cite{mendelson1981permutations}

\vspace{-2mm}
\begin{align}
\scriptsize
f(n,\mathbb{L},\{m_{0}, m_{1}, ...,m_{n-1}\}) = \dfrac{(m_0+m_1+\cdot\cdot\cdot m_{n-1})!}{(m_0!)(m_1!)\cdot\cdot\cdot(m_{n-1}!)}
\end{align}

\textbf{Remark 5}: {\textit{Let {$\mathbb{L}$ be the length of the type of flows with upper bound $f(n,\mathbb{L},\{m_{0}, m_{1}, ...,m_{n-1}\})$, $\mathbb{L}$=$\sum_{i=0}^{n-1}m_i$.}}}

Whereas the work in \cite{DBLP:conf/dac/YuXM18} constraints the search-space to \textit{m-}repetitions flow, with the upper bound given by Equation 2, in this work we approach this problem in a more general way, where each repetition might have a different number of repetitions. In this case, the theoretical upper bound is given by Equation 3. 

%\subsection{Quality of Result in Digital ICs}

% \begin{figure}[t]
% \centering
% \begin{minipage}{0.24\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/1-crop.pdf}
% \subcaption{}\label{fig:fa_labeling_a}
% \end{minipage}%
% \begin{minipage}{0.2\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/2-crop.pdf}
% \subcaption{}\label{fig:fa_labeling_b}
% \end{minipage}%
% \caption{1-bit Full Adder ($F= 2C+S=a+b+c$) gate-level netlists produced by two different synthesis flows using 7nm FinFET technology library. a) Delay = 30.1 ps, Area = 9.40 um$^2$; b) Delay = 47.6 ps, Area = 8.38 um$^2$.}
% \label{fig:full_adder}
% \end{figure}


% \begin{figure*}[b]
% \centering
% \begin{minipage}{0.235\textwidth}
%   \centering
%   \small
% \includegraphics[width=1\textwidth]{figs/aes-all-distribution.eps}
% \subcaption{2-D QoR distro of AES}\label{fig:motivation1-aes}
% \end{minipage}%
% \begin{minipage}{0.235\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/aes-all-distribution-3D.eps}
% \subcaption{3-D QoR distro of AES}\label{fig:motivation2-aes}
% \end{minipage}%
% %datapath
% \begin{minipage}{0.235\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/datapath-all-distribution.eps}
% \subcaption{2-D QoR distro of ALU}\label{fig:motivation1-datapath}
% \end{minipage}%
% \begin{minipage}{0.235\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/datapath-all-distribution-3D.eps}
% \subcaption{3-D QoR distro of ALU}\label{fig:motivation2-datapath}
% \end{minipage}%
% \caption{Delay and area results of the 50,000 random ABC synthesis flows of 128-bit AES core and 64-bit ALU.}
% \vspace{-4mm}
% \label{fig:motivation}
% \end{figure*}


%QoR of Integrated Circuits (IC) is a term used in evaluating the quality of the IC based on different metrics. Mostly, it is represented as a vector of values that describes the performance of the designs and design process. For example, a QoR could include the critical path delay (chip frequency = 1$/$Delay), power dissipation, area, e.g., \{1 ns (1 GHz), 2.5 W, 1 mm$^2$\}. Given a design specification, the QoR of the technological processed designs can be very different using different synthesis flows. In particular, synthesis flows are designed and applied depending on the application, as different applications can have very different objectives and features. For instance, for high-performance image processing, the designs are mostly designed to be as fast as possible, i.e., delay to be as small as possible. On the other hand, for the Internet-of-Things (IoT), designs aim to minimize the power and area primarily. The massive search space of synthesis flows (Equations 1-3), the time-consuming technological design process for QoR evaluation, along the various design objectives are the main motivations of this work.

%An illustrative example of mapping a 1-bit Full Adder using 7nm FinFET technology library is shown in Figure \ref{fig:full_adder}. The specification of a 1-bit Full Adder is $a+b+c = 2C + S$, where $a,b,c,C,S$ are binary signals. Using two different synthesis flows, two gate-level netlists are produced. In Figure \ref{fig:full_adder}, each node represents one logic gate and the type label of the node is the type of the logic gate. Note that the performance of different logic gates are different and they are defined based on the technology libraries. For example, delay and area of XOR2 are 15.95 ps and 2.8 um$^2$; delay and area of NAND2 are 11.90 ps and 1.39 um$^2$. After applying synthesis flow, we observe that the QoRs of two netlists are different. The design in Figure \ref{fig:fa_labeling_a} is about 37\% faster than design in Figure \ref{fig:fa_labeling_b}, and requires 12\% more area. Note that the QoR can only be obtained after the entire technological design process. For large designs, this process is extremely time-consuming.




%3.2466705$\cdot10^{15}$

\subsection{Motivating Example}\label{sec:motivating-example}

\begin{figure}[!h]
\centering
\includegraphics[width=0.44\textwidth]{figs/aes_abc_heat_partial.pdf}
\caption{Evaluation of three default flows, \textit{resyn ('o'), resyn2 ('x')} and \textit{resyn3 (the star)} using 128-bit AES design. The heatmap includes the QoR of the 50,000 random flows.}
\label{fig:default_flow_compare}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=0.44\textwidth]{figs/aes_lso_heat_partial.pdf}
\caption{Evaluation of the LSOracle default flow (black star) using 128-bit AES design. The heatmap includes the QoR of the 50,000 random flows.}
\label{fig:lso_flow_compare}
\end{figure}

We provide two motivating examples using open-source logic synthesis framework ABC \cite{mishchenko2010abc} and LSOracle \cite{neto2019lsoracle}, in which the backend data structures are AIGs and MIGs, respectively. % shown in Figure \ref{fig:default_flow_compare}. 
The experimental setups for the motivational examples are as follows:

%    \vspace{0mm}
%\begin{itemize}
\noindent
\textbf{ABC \cite{mishchenko2010abc}} -- We use the following set of commands: $\mathbb{S}$=\{balance, restructure, rewrite, refactor, rewrite -z, refactor -z\} ($n$=6); the elements in  $\mathbb{S}$ are logic transformations in ABC\footnote{\small The names of these transformations are the same as the commands in ABC.} that can be processed independently. We take as input a 128-bit Advanced Encryption Standard (AES) core\cite{opencore-web} and generate 50,000 unique $4$-repetition flows are generated by random permutations of  $\mathbb{S}_{4}$ ($m$=4, $n$=6, $\mathbb{L}$=24). The delay and area of these flows are obtained after technology mapping using the ASAP 7nm predictive standard-cell library.  

\noindent
\textbf{LSOracle\cite{neto2019lsoracle}} -- We use the following transformations: $\mathbb{S}$=\{rewrite, resub, refactor\} ($n$=3). That is because these are the main transformations used in the highest MIG-based transformation in LSOracle. We take as input a 128-bit Advanced Encryption Standard (AES) core\cite{opencore-web} and generate 50,000 unique $4$-repetition flows are generated by random permutations of  $\mathbb{S}_{4}$ ($m$=3, $n$=9, $\mathbb{L}$=27). We chose to have a flow of length 27 as it is a multiplier of the default LSOracle flow, which has 9 transformations by default. To compare, we run the default LSOracle flow 3$\times$. The delay and area of these flows are obtained after technology mapping using the ASAP 7nm predictive standard-cell library.


The QoR distributions for the AES can be seen in Figures \ref{fig:default_flow_compare},\ref{fig:lso_flow_compare}, and several important observations can be drawn from it, which highlight the main motivations of this work:
    \vspace{0mm}


\begin{itemize}
    \item (1) Given the same set of synthesis transformations, the QoR is very different using different flows, for both AIG and MIG. For example, for the AIG case, the delay and area of AES design produced by the 50,000 flows have up to 40\% and 90\% difference, respectively. As for the MIG-based flow, the variance of delay and area are up to {39.27\% and 13.97\%}, respectively. 
    \vspace{0mm}
    \item (2) The search space of the synthesis flows is large. According to Remark 3, the total number of available $4$-repetition flows with $n=6$ independent synthesis transformations is more than $10^{16}$ (considering our AIG example). Discovering the high-quality synthesis flows with human-testing among the entire search space is unlikely to be achieved. Same holds for MIGs.
        \vspace{0mm}
    % \item The same set of flows perform differently on different designs. For example, in Figure \ref{fig:motivation}, QoR distributions of AES and ALU are \textit{statistically significant}. This means that the high-quality flows for AES design could perform poorly for ALU. Therefore, synthesis flows need to be customized for specific IP or design.
        \vspace{0mm}
\end{itemize}

% To further show the motivations, we compare the random flows to the default flows developed by experts provided in ABC using 128-bit AES design. The results are shown in Figure \ref{fig:default_flow_compare}.

As it is possible to observe, we position the three most widely used default flows provided in ABC, including \textit{resyn, resyn2} and \textit{resyn3}, with respect to the QoR achieved with the random flows. Whereas \textit{resyn} provides the best QoR among these three default flows, its result performs $>$10\% worse than the best flows of the 50,000 random flows, in both delay and area. Specifically, there are more than 25,000 random flows that perform better than all the default flows. This means that for every two random permuted flows, one of them is likely to over-perform the expert-developed flows for this design. 
Similarly, we show that a high-effort and well expert-tuned flow in LSOracle flow MIGs still have much room for improvement. In particular, the default flow presents a good delay overall, but with room for achieving a better area ($\approx$7\% worse area than random flows with similar delay). 
These motivational examples show that automatic flow generation is an important direction for both AIG- and MIG-based synthesis flow generation. This, along with the large search space, provides the main motivation for this work. It is also important to note that a given flow performs differently on different designs. For example, high-quality flows for our AES design could perform poorly on other designs \cite{DBLP:conf/dac/YuXM18}. 








==> figs/results_1o_plot.tex <==

\begin{figure}[!htb]
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O1.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O1}}$}
  \label{fig:1O_O1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include second image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O2.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O2}}$}
  \label{fig:1O_O2}
\end{subfigure}
\hfill

\begin{subfigure}{0.49\linewidth}
  \centering
  % include third image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O3.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O3}}$}
  \label{fig:1O_O3}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include fourth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O4.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O4}}$}
  \label{fig:1O_O4}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include fifth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O5.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O5}}$}
  \label{fig:1O_O5}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include sixth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O6.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O6}}$}
  \label{fig:1O_O6}
\end{subfigure}
\caption{Normalized node number comparison of the same design after applying stand-alone optimizations and \texttt{orchestration} with a single AIG traversal. \textbf{R} is the ratio of the number of designs on which \texttt{orchestration} outperforms stand-alone optimization to the number of total tested designs.}
\vspace{-4mm}
\label{fig:1O}
\end{figure}


==> figs/results_3o_plot.tex <==
\begin{figure}[!htb]
\centering
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_1.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{\texttt{O1}}$)}
  \label{fig:3O_O1}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include third image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_3.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{\texttt{O3}}$)}
  \label{fig:3O_O3}
\end{subfigure}

\caption{Normalized node number comparison between iterative \texttt{orchestration} and iterative ABC SOTA optimizations. \textbf{R} is the ratio of the number of designs on which Seq($\widehat{\texttt{On}}$) outperforms Seq(ABC) to the number of total tested designs.}
%\vspace{-3mm}
\label{fig:3O}
\end{figure}




==> figs/venn.tex <==
\begin{figure*}
    \centering
    %     \begin{subfigure}[b]{0.32\textwidth}
    % \centering
    %     \includegraphics[width=0.8\textwidth]{figs/tcad_venn_rw_rs_bfly.pdf}
    %     \caption{Venn diagram between \texttt{rw} and \texttt{rs}}
    %     \label{fig:venn_rw_rs}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.32\textwidth}
    % \centering
    %     \includegraphics[width=0.8\textwidth]{figs/tcad_venn_rw_rf_bfly.pdf}
    %     \caption{Venn diagram between \texttt{rw} and \texttt{rf}}
    %     \label{fig:venn_rw_rf}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{TCAD24-Orch/figs/tcad_venn_rs_rf_rw_bfly.pdf}
        \caption{\texttt{rw} and \texttt{rs} and \texttt{rf}}
        \label{fig:venn_rw_rs_rf}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=0.8\textwidth]{figs/tcad_venn_o1_rw_bfly.pdf}
        \caption{\texttt{rw} and the \texttt{rw} in $\widehat{\texttt{O1}}$}
        \label{fig:venn_o1_rw}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[width=0.8\textwidth]{figs/tcad_venn_o1_rs_bfly.pdf}
        \caption{\texttt{rs} and the \texttt{rs} in $\widehat{\texttt{O1}}$}
        \label{fig:venn_o1_rs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
\includegraphics[width=0.8\textwidth]{figs/tcad_venn_o1_rf_bfly.pdf}
        \caption{\texttt{rf} and the \texttt{rf} in $\widehat{\texttt{O1}}$}
        \label{fig:venn_o1_rf}
    \end{subfigure}
    
    \caption{{The Venn diagram for the design \textit{bfly}—a detailed analysis of Figure \ref{fig:bfly_bd}—illustrates the relationships as follows: (a) among standalone optimizations; and (b) to (d) between orchestration optimization $\widehat{\texttt{O1}}$ (as defined in Section \ref{sec: Orchrules}) and each of \texttt{rw}, \texttt{rs}, \texttt{rf}, respectively. In each diagram, we consider only the nodes that participate in valid iterations within the respective optimizations. Furthermore, for $\widehat{\texttt{O1}}$ in diagrams (b) to (d), the number of valid iterations is aligned with that of the corresponding optimization for comparison.}
    }
    \label{fig:venn}
\end{figure*}

==> runtime_ana.tex <==
\subsection{Single Runtime Evaluation}
\label{sec:runtime_result}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.99\textwidth]{TCAD21-FlowTune/figs/runtime_rw.pdf}
        \caption{runtime comparison with \texttt{rw}}
        \label{fig:rt_rw_pure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.99\textwidth]{TCAD21-FlowTune/figs/runtime_rs.pdf}
        \caption{runtime comparison with \texttt{rs}}
        \label{fig:rt_rs_pure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
\includegraphics[width=0.99\textwidth]{TCAD21-FlowTune/figs/runtime_rf.pdf}
        \caption{runtime comparison with \texttt{rf}}
        \label{fig:rt_rf_pure}
    \end{subfigure}
     
 \caption{Runtime comparison between selected single-traversal \texttt{orchestration} policies ($\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{Local-greedy} (labeled as \texttt{LGP})) and stand-alone optimizations from ABC: (a) runtime comparison with \texttt{rw}; (b) runtime comparison with \texttt{rs}; (c) runtime comparison with \texttt{rf}.
}
    \label{fig:runtime comparison_pure}
\end{figure*}
\input{tbls/table_runtime}

\yingjie{In this section, we further discuss the runtime cost for orchestration algorithms and its comparison with stand-alone optimization algorithms for all 104 designs in Figure \ref{fig:runtime comparison}.
We present the runtime comparisons for the single graph traversal with \textit{Local-greedy} orchestration optimization (\texttt{LGP}) and \textit{Priority-ordered} orchestration optimization with $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$ ($\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$), with stand-alone optimizations (i.e., \texttt{rw}, \texttt{rs}, and \texttt{rf}).}
%A runtime comparison for all 104 designs across diverse benchmark suites between $\widehat{\texttt{O1}}$, $\widehat{\texttt{O3}}$, and \texttt{LGP} as opposed to \texttt{rw}, \texttt{rs}, and \texttt{rf}, respectively, is depicted in Figure \ref{fig:runtime comparison}. 
In Figure \ref{fig:runtime comparison}, to improve the discernibility of runtime discrepancies, the figure's axes employ a logarithmic scale. The x-axis signifies the stand-alone ABC optimization runtime, while the y-axis corresponds to the \textit{orchestration} runtime. The dotted line ($x=y$) serves as a demarcation for runtime performance: a point above the line suggests increased runtime cost generated by the respective \textit{orchestration} algorithm in comparison to the corresponding stand-alone ABC optimization, while a point below the line implies reduced runtime cost. 

For example, in Figure \ref{fig:rt_rs}, a majority of the blue dots are positioned above the dotted line, denoting that the \texttt{LGP} incurs runtime overhead relative to \texttt{rs}; while the red triangles and green stars, which denotes the runtime for $\widehat{\texttt{O1}}$ and $\widehat{\texttt{O3}}$, are mostly below the dotted line, indicating that the \textit{Priority-ordered} orchestration algorithm functions with less runtime compared to \texttt{rs}. Thus, compared with stand-alone optimizations, i.e, \texttt{rw}, \texttt{rs}, and \texttt{rf}, we find that \textbf{(1)} the \textit{Local-greedy} orchestration method incurs runtime overhead for most designs as it requires the transformability check for all three optimization operations at each node as shown in Algorithm \ref{alg:local}, line 2; \textbf{(2)} the \textit{Priority-ordered} orchestration incurs less runtime cost than \textit{Local-greedy} orchestration method and stand-alone optimizations. Compared with \textit{Local-greedy} orchestration, \textit{Priority-ordered} orchestration conducts significantly less transformability check based on the pre-defined priority order. %while compared with stand-alone optimizations, it involves less running iterations as more optimization opportunities lead to more nodes within the optimization cut excluded from the iterations at each applicable optimization operation.

{To further analyze the runtime differences, we include }Table \ref{table:it_count} that presents the iteration counts of stand-alone ABC optimizations and the averagely best \textit{Priority-ordered} orchestration algorithm with $\widehat{\texttt{O3}}$. 
\yingjie{There are mainly two observations from Table \ref{table:it_count}: \textbf{(1)} The total number of iterations in the orchestration algorithm is significantly less than that in \texttt{rw}, which results in its less runtime cost compared with \texttt{rw}. As we discussed in Section \ref{sec:background_DAG_syn}, the logic cut used in each iteration in \texttt{rw} is relatively small (4-feasible cut), thus to traverse the whole graph (usually with the graph size of $10^{2} - 10^{6}$), it requires significantly more iterations compared with other optimization algorithms involving large logic cut per iteration such as \texttt{rs} and \texttt{rf}. While the orchestration algorithm involves \texttt{rs} and \texttt{rf} into the graph traversal, it saves a significant number of required iterations and thus the required runtime. \textbf{(2)} Even though the orchestration algorithm requires more iterations than \texttt{rs} and \texttt{rf}, it incurs less runtime. 
Compared with \texttt{rs} and \texttt{rf}, the orchestration algorithm requires more iterations, which results from the involvements of \texttt{rw} iterations with small cut size in the graph traversal in the orchestrated optimization. However, the small logic cut per iteration in \texttt{rw} incurs less runtime cost, and combining \texttt{rw} iterations in the optimization can result in less average runtime cost over all iterations compared to \texttt{rs} and \texttt{rf}.} 


==> tbls/table_3o.tex <==
\begin{table*}[t]
\color{blue}
\centering
\caption{\yingjie{Detailed results of selected large size designs. Comparison of Iterative-traversal \texttt{orchestration} with corresponding sequence optimizations from ABC.}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cccccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{14}{c|}{AIG} \\ \cline{3-16} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{Baseline} & \multicolumn{1}{c|}{\texttt{rw} $\rightarrow$ \texttt{rs} $\rightarrow$ \texttt{rf}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O1}}$)} & \multicolumn{1}{c|}{\texttt{rw} $\rightarrow$ \texttt{rf} $\rightarrow$ \texttt{rs}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O2}}$)} & \multicolumn{1}{c|}{\texttt{rs} $\rightarrow$ \texttt{rw} $\rightarrow$ \texttt{rf}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O3}}$)} & \multicolumn{1}{c|}{\texttt{rs} $\rightarrow$ \texttt{rf} $\rightarrow$ \texttt{rw}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O4}}$)} & \multicolumn{1}{c|}{\texttt{rf} $\rightarrow$ \texttt{rs} $\rightarrow$ \texttt{rw}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O5}}$)} & \multicolumn{1}{c|}{\texttt{rf} $\rightarrow$ \texttt{rw} $\rightarrow$ \texttt{rs}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O6}}$)} & {Seq(\texttt{LGP})} \\ \cline{3-16} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \#Node ($\Delta$\%) \\ \hline

\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & \multicolumn{1}{c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{10288 (17.0\%)} & \multicolumn{1}{c|}{10176 (17.9\%)} & \multicolumn{1}{c|}{10230 (17.5\%)} & \multicolumn{1}{c|}{10196 (17.8\%)} & \multicolumn{1}{c|}{10263 (17.2\%)} & \multicolumn{1}{c|}{\textbf{10115 (18.4\%)}} & \multicolumn{1}{c|}{10219 (17.6\%)} & \multicolumn{1}{c|}{10493 (15.4\%)} & \multicolumn{1}{c|}{10250 (17.3\%)} & \multicolumn{1}{c|}{10793 (13.0\%)} & \multicolumn{1}{c|}{10242 (17.4\%)} & \multicolumn{1}{c|}{10788 (13.0\%)} & 10187 (17.8\%) \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{\textbf{8177 (31.6\%)}} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{\textbf{8177 (31.6\%)}} & \textbf{8129 (32.0\%)} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{22724 (17.8\%)} & \multicolumn{1}{c|}{\textbf{22503 (18.6\%)}} & \multicolumn{1}{c|}{22664 (18.0\%)} & \multicolumn{1}{c|}{22620 (18.2\%)} & \multicolumn{1}{c|}{22831 (17.4\%)} & \multicolumn{1}{c|}{22533 (18.5\%)} & \multicolumn{1}{c|}{22841 (17.4\%)} & \multicolumn{1}{c|}{23084 (16.5\%)} & \multicolumn{1}{c|}{22888 (17.2\%)} & \multicolumn{1}{c|}{24203 (12.5\%)} & \multicolumn{1}{c|}{22832 (17.4\%)} & \multicolumn{1}{c|}{24203 (12.5\%)} & 22506 (18.6\%) \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{62622 (20.8\%)} & \multicolumn{1}{c|}{61556 (22.1\%)} & \multicolumn{1}{c|}{62425 (21.0\%)} & \multicolumn{1}{c|}{62676 (20.7\%)} & \multicolumn{1}{c|}{63060 (20.2\%)} & \multicolumn{1}{c|}{61568 (22.1\%)} & \multicolumn{1}{c|}{63042 (20.3\%)} & \multicolumn{1}{c|}{64492 (18.4\%)} & \multicolumn{1}{c|}{62552 (20.9\%)} & \multicolumn{1}{c|}{68539 (13.3\%)} & \multicolumn{1}{c|}{62288 (21.2\%)} & \multicolumn{1}{c|}{68540 (13.3\%)} & \textbf{61457 (22.3\%)} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{10009 (18.1\%)} & \multicolumn{1}{c|}{\textbf{9798 (19.8\%)}} & \multicolumn{1}{c|}{9972 (18.4\%)} & \multicolumn{1}{c|}{9921 (18.8\%)} & \multicolumn{1}{c|}{10029 (17.9\%)} & \multicolumn{1}{c|}{9799 (19.8\%)} & \multicolumn{1}{c|}{9910 (18.9\%)} & \multicolumn{1}{c|}{10026 (17.9\%)} & \multicolumn{1}{c|}{9933 (18.7\%)} & \multicolumn{1}{c|}{10370 (15.1\%)} & \multicolumn{1}{c|}{9907 (18.9\%)} & \multicolumn{1}{c|}{10372 (15.1\%)} & 9815 (19.7\%)\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{10150 (20.6\%)} & \multicolumn{1}{c|}{\textbf{9904 (22.5\%)}} & \multicolumn{1}{c|}{10137 (20.7\%)} & \multicolumn{1}{c|}{10034 (21.5\%)} & \multicolumn{1}{c|}{10175 (20.4\%)} & \multicolumn{1}{c|}{9914 (22.4\%)} & \multicolumn{1}{c|}{10084 (21.1\%)} & \multicolumn{1}{c|}{10163 (20.5\%)} & \multicolumn{1}{c|}{10211 (20.1\%)} & \multicolumn{1}{c|}{10654 (16.6\%)} & \multicolumn{1}{c|}{10033 (21.5\%)} & \multicolumn{1}{c|}{10656 (16.6\%)} & 9915 (22.4\%)\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{14960 (19.1\%)} & \multicolumn{1}{c|}{14633 (20.9\%)} & \multicolumn{1}{c|}{14891 (19.5\%)} & \multicolumn{1}{c|}{14830 (19.8\%)} & \multicolumn{1}{c|}{14952 (19.1\%)} & \multicolumn{1}{c|}{\textbf{14629 (20.9\%)}} & \multicolumn{1}{c|}{14856 (19.6\%)} & \multicolumn{1}{c|}{14962 (19.1\%)} & \multicolumn{1}{c|}{14743 (20.3\%)} & \multicolumn{1}{c|}{15654 (15.3\%)} & \multicolumn{1}{c|}{14710 (20.4\%)} & \multicolumn{1}{c|}{15656 (15.3\%)} & 14676 (20.6\%)\\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & \multicolumn{1}{c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{25914 (10.4\%)} & \multicolumn{1}{c|}{25750 (10.9\%)} & \multicolumn{1}{c|}{25839 (10.6\%)} & \multicolumn{1}{c|}{25945 (10.3\%)} & \multicolumn{1}{c|}{26015 (10.0\%)} & \multicolumn{1}{c|}{25818 (10.7\%)} & \multicolumn{1}{c|}{25931 (10.3\%)} & \multicolumn{1}{c|}{26163 (9.5\%)} & \multicolumn{1}{c|}{25871 (10.5\%)} & \multicolumn{1}{c|}{27373 (5.3\%)} & \multicolumn{1}{c|}{25827 (10.7\%)} & \multicolumn{1}{c|}{27375 (5.3\%)} & \textbf{25727 (11.0\%)} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{25269 (10.6\%)} & \multicolumn{1}{c|}{25093 (11.2\%)} & \multicolumn{1}{c|}{25208 (10.8\%)} & \multicolumn{1}{c|}{25281 (10.5\%)} & \multicolumn{1}{c|}{25377 (10.2\%)} & \multicolumn{1}{c|}{25119 (11.1\%)} & \multicolumn{1}{c|}{25312 (10.4\%)} & \multicolumn{1}{c|}{25566 (9.5\%)} & \multicolumn{1}{c|}{25250 (10.6\%)} & \multicolumn{1}{c|}{26861 (4.9\%)} & \multicolumn{1}{c|}{25175 (10.9\%)} & \multicolumn{1}{c|}{26861 (4.9\%)} & \textbf{25052 (11.3\%)} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{24751 (10.7\%)} & \multicolumn{1}{c|}{24568 (11.3\%)} & \multicolumn{1}{c|}{24688 (10.9\%)} & \multicolumn{1}{c|}{24818 (10.4\%)} & \multicolumn{1}{c|}{24802 (10.5\%)} & \multicolumn{1}{c|}{24607 (11.2\%)} & \multicolumn{1}{c|}{24757 (10.6\%)} & \multicolumn{1}{c|}{24984 (9.8\%)} & \multicolumn{1}{c|}{24733 (10.7\%)} & \multicolumn{1}{c|}{26191 (5.5\%)} & \multicolumn{1}{c|}{24718 (10.8\%)} & \multicolumn{1}{c|}{26209 (5.4\%)} & \textbf{24553 (11.4\%)}\\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{26890 (10.4\%)} & \multicolumn{1}{c|}{26708 (11.0\%)} & \multicolumn{1}{c|}{26833 (10.6\%)} & \multicolumn{1}{c|}{27001 (10.0\%)} & \multicolumn{1}{c|}{26962 (10.1\%)} & \multicolumn{1}{c|}{26738 (10.9\%)} & \multicolumn{1}{c|}{26942 (10.2\%)} & \multicolumn{1}{c|}{27188 (9.4\%)} & \multicolumn{1}{c|}{26854 (10.5\%)} & \multicolumn{1}{c|}{28494 (5.0\%)} & \multicolumn{1}{c|}{26810 (10.6\%)} & \multicolumn{1}{c|}{28480 (5.1\%)} & \textbf{26700 (11.0\%)} \\ \hline


\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & \multicolumn{1}{c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{40965 (28.4\%)} & \multicolumn{1}{c|}{40869 (28.6\%)} & \multicolumn{1}{c|}{40965 (28.4\%)} & \multicolumn{1}{c|}{40866 (28.6\%)} & \multicolumn{1}{c|}{41006 (28.4\%)} & \multicolumn{1}{c|}{40874 (28.6\%)} & \multicolumn{1}{c|}{41004 (28.4\%)} & \multicolumn{1}{c|}{51414 (10.2\%)} & \multicolumn{1}{c|}{41142 (28.1\%)} & \multicolumn{1}{c|}{56224 (1.8\%)} & \multicolumn{1}{c|}{41104 (28.2\%)} & \multicolumn{1}{c|}{56222 (1.8\%)} & \textbf{40849 (28.6\%)}\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{207340 (3.3\%)} & \multicolumn{1}{c|}{206559 (3.6\%)} & \multicolumn{1}{c|}{207343 (3.3\%)} & \multicolumn{1}{c|}{211283 (1.4\%)} & \multicolumn{1}{c|}{207320 (3.3\%)} & \multicolumn{1}{c|}{\textbf{206539 (3.6\%)}} & \multicolumn{1}{c|}{206648 (3.6\%)} & \multicolumn{1}{c|}{207240 (3.3\%)} & \multicolumn{1}{c|}{206671 (3.6\%)} & \multicolumn{1}{c|}{211991 (1.1\%)} & \multicolumn{1}{c|}{206671 (3.6\%)} & \multicolumn{1}{c|}{211991 (1.1\%)} & \textbf{206530 (3.6\%)}\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{46177 (1.4\%)} & \multicolumn{1}{c|}{45650 (2.5\%)} & \multicolumn{1}{c|}{46013 (1.8\%)} & \multicolumn{1}{c|}{46005 (1.8\%)} & \multicolumn{1}{c|}{46171 (1.4\%)} & \multicolumn{1}{c|}{\textbf{45360 (3.2\%)}} & \multicolumn{1}{c|}{46039 (1.7\%)} & \multicolumn{1}{c|}{45855 (2.1\%)} & \multicolumn{1}{c|}{46113 (1.5\%)} & \multicolumn{1}{c|}{46312 (1.1\%)} & \multicolumn{1}{c|}{46077 (1.6\%)} & \multicolumn{1}{c|}{46312 (1.1\%)} & 45418 (3.0\%)\\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{19327 (21.5\%)} & \multicolumn{1}{c|}{19219 (21.9\%)} & \multicolumn{1}{c|}{19327 (21.5\%)} & \multicolumn{1}{c|}{\textbf{19218 (21.9\%)}} & \multicolumn{1}{c|}{19333 (21.5\%)} & \multicolumn{1}{c|}{19219 (21.9\%)} & \multicolumn{1}{c|}{19333 (21.5\%)} & \multicolumn{1}{c|}{19223 (21.9\%)} & \multicolumn{1}{c|}{19332 (21.5\%)} & \multicolumn{1}{c|}{23661 (3.9\%)} & \multicolumn{1}{c|}{19328 (21.5\%)} & \multicolumn{1}{c|}{23661 (3.9\%)} & \textbf{19217 (21.9\%)}\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{8755 (36.4\%)} & \multicolumn{1}{c|}{\textbf{8428 (38.7\%)}} & \multicolumn{1}{c|}{9109 (33.8\%)} & \multicolumn{1}{c|}{10306 (25.1\%)} & \multicolumn{1}{c|}{9056 (34.2\%)} & \multicolumn{1}{c|}{8612 (37.4\%)} & \multicolumn{1}{c|}{9060 (34.1\%)} & \multicolumn{1}{c|}{8589 (37.6\%)} & \multicolumn{1}{c|}{9789 (28.8\%)} & \multicolumn{1}{c|}{12440 (9.6\%)} & \multicolumn{1}{c|}{9870 (28.3\%)} & \multicolumn{1}{c|}{12440 (9.6\%)} & 8861 (35.6\%) \\ \hline

\multicolumn{3}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{\textbf{18.3\%}} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{16.8\%} & \multicolumn{1}{c|}{16.9\%} & \multicolumn{1}{c|}{\textbf{18.3\%}} & \multicolumn{1}{c|}{17.3\%} & \multicolumn{1}{c|}{15.8\%} & \multicolumn{1}{c|}{17.0\%} & \multicolumn{1}{c|}{9.7\%} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{9.7\%} & 18.2\%\\ \hline
\end{tabular}
}
% \caption{Detailed results of selected large size designs. Comparison of single-traversal \texttt{orchestration} with stand-alone optimizations from ABC.}
% \vspace{-3mm}
\label{table:3O}
\end{table*}

==> tbls/table_3o_2.tex <==
\begin{table*}[t]
\centering
\caption{{Detailed results of selected large size designs. Comparison of Iterative-traversal \texttt{orchestration} with corresponding sequence optimizations from ABC.}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cccccccccccccc|}
\hline
{\multirow{3}{*}{Design}} & \multicolumn{14}{c|}{AIG} \\ \cline{2-15}  
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{Baseline} & \multicolumn{1}{c|}{\texttt{rw} $\rightarrow$ \texttt{rs} $\rightarrow$ \texttt{rf}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O1}}$)} & \multicolumn{1}{c|}{\texttt{rw} $\rightarrow$ \texttt{rf} $\rightarrow$ \texttt{rs}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O2}}$)} & \multicolumn{1}{c|}{\texttt{rs} $\rightarrow$ \texttt{rw} $\rightarrow$ \texttt{rf}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O3}}$)} & \multicolumn{1}{c|}{\texttt{rs} $\rightarrow$ \texttt{rf} $\rightarrow$ \texttt{rw}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O4}}$)} & \multicolumn{1}{c|}{\texttt{rf} $\rightarrow$ \texttt{rs} $\rightarrow$ \texttt{rw}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O5}}$)} & \multicolumn{1}{c|}{\texttt{rf} $\rightarrow$ \texttt{rw} $\rightarrow$ \texttt{rs}} & \multicolumn{1}{c|}{Seq($\widehat{\texttt{O6}}$)} & {Seq(\texttt{LGP})} \\ \cline{2-15} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \#Node ($\Delta$\%) \\ \hline

\multicolumn{1}{|c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{10288 (17.0\%)} & \multicolumn{1}{c|}{10176 (17.9\%)} & \multicolumn{1}{c|}{10230 (17.5\%)} & \multicolumn{1}{c|}{10196 (17.8\%)} & \multicolumn{1}{c|}{10263 (17.2\%)} & \multicolumn{1}{c|}{\textbf{10115 (18.4\%)}} & \multicolumn{1}{c|}{10219 (17.6\%)} & \multicolumn{1}{c|}{10493 (15.4\%)} & \multicolumn{1}{c|}{10250 (17.3\%)} & \multicolumn{1}{c|}{10793 (13.0\%)} & \multicolumn{1}{c|}{10242 (17.4\%)} & \multicolumn{1}{c|}{10788 (13.0\%)} & 10187 (17.8\%) \\ \cline{1-15} 

\multicolumn{1}{|c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8561 (28.3\%)} & \multicolumn{1}{c|}{\textbf{8177 (31.6\%)}} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{8177 (31.6\%)} & \multicolumn{1}{c|}{\textbf{8177 (31.6\%)}} & \textbf{8129 (32.0\%)} \\ \cline{1-15} 

\multicolumn{1}{|c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{22724 (17.8\%)} & \multicolumn{1}{c|}{\textbf{22503 (18.6\%)}} & \multicolumn{1}{c|}{22664 (18.0\%)} & \multicolumn{1}{c|}{22620 (18.2\%)} & \multicolumn{1}{c|}{22831 (17.4\%)} & \multicolumn{1}{c|}{22533 (18.5\%)} & \multicolumn{1}{c|}{22841 (17.4\%)} & \multicolumn{1}{c|}{23084 (16.5\%)} & \multicolumn{1}{c|}{22888 (17.2\%)} & \multicolumn{1}{c|}{24203 (12.5\%)} & \multicolumn{1}{c|}{22832 (17.4\%)} & \multicolumn{1}{c|}{24203 (12.5\%)} & 22506 (18.6\%) \\ \cline{1-15} 

\multicolumn{1}{|c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{62622 (20.8\%)} & \multicolumn{1}{c|}{61556 (22.1\%)} & \multicolumn{1}{c|}{62425 (21.0\%)} & \multicolumn{1}{c|}{62676 (20.7\%)} & \multicolumn{1}{c|}{63060 (20.2\%)} & \multicolumn{1}{c|}{61568 (22.1\%)} & \multicolumn{1}{c|}{63042 (20.3\%)} & \multicolumn{1}{c|}{64492 (18.4\%)} & \multicolumn{1}{c|}{62552 (20.9\%)} & \multicolumn{1}{c|}{68539 (13.3\%)} & \multicolumn{1}{c|}{62288 (21.2\%)} & \multicolumn{1}{c|}{68540 (13.3\%)} & \textbf{61457 (22.3\%)} \\ \cline{1-15} 

\multicolumn{1}{|c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{10009 (18.1\%)} & \multicolumn{1}{c|}{\textbf{9798 (19.8\%)}} & \multicolumn{1}{c|}{9972 (18.4\%)} & \multicolumn{1}{c|}{9921 (18.8\%)} & \multicolumn{1}{c|}{10029 (17.9\%)} & \multicolumn{1}{c|}{9799 (19.8\%)} & \multicolumn{1}{c|}{9910 (18.9\%)} & \multicolumn{1}{c|}{10026 (17.9\%)} & \multicolumn{1}{c|}{9933 (18.7\%)} & \multicolumn{1}{c|}{10370 (15.1\%)} & \multicolumn{1}{c|}{9907 (18.9\%)} & \multicolumn{1}{c|}{10372 (15.1\%)} & 9815 (19.7\%)\\ \cline{1-15} 

\multicolumn{1}{|c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{10150 (20.6\%)} & \multicolumn{1}{c|}{\textbf{9904 (22.5\%)}} & \multicolumn{1}{c|}{10137 (20.7\%)} & \multicolumn{1}{c|}{10034 (21.5\%)} & \multicolumn{1}{c|}{10175 (20.4\%)} & \multicolumn{1}{c|}{9914 (22.4\%)} & \multicolumn{1}{c|}{10084 (21.1\%)} & \multicolumn{1}{c|}{10163 (20.5\%)} & \multicolumn{1}{c|}{10211 (20.1\%)} & \multicolumn{1}{c|}{10654 (16.6\%)} & \multicolumn{1}{c|}{10033 (21.5\%)} & \multicolumn{1}{c|}{10656 (16.6\%)} & 9915 (22.4\%)\\ \cline{1-15} 

\multicolumn{1}{|c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{14960 (19.1\%)} & \multicolumn{1}{c|}{14633 (20.9\%)} & \multicolumn{1}{c|}{14891 (19.5\%)} & \multicolumn{1}{c|}{14830 (19.8\%)} & \multicolumn{1}{c|}{14952 (19.1\%)} & \multicolumn{1}{c|}{\textbf{14629 (20.9\%)}} & \multicolumn{1}{c|}{14856 (19.6\%)} & \multicolumn{1}{c|}{14962 (19.1\%)} & \multicolumn{1}{c|}{14743 (20.3\%)} & \multicolumn{1}{c|}{15654 (15.3\%)} & \multicolumn{1}{c|}{14710 (20.4\%)} & \multicolumn{1}{c|}{15656 (15.3\%)} & 14676 (20.6\%)\\ \hline

\multicolumn{1}{|c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{25914 (10.4\%)} & \multicolumn{1}{c|}{25750 (10.9\%)} & \multicolumn{1}{c|}{25839 (10.6\%)} & \multicolumn{1}{c|}{25945 (10.3\%)} & \multicolumn{1}{c|}{26015 (10.0\%)} & \multicolumn{1}{c|}{25818 (10.7\%)} & \multicolumn{1}{c|}{25931 (10.3\%)} & \multicolumn{1}{c|}{26163 (9.5\%)} & \multicolumn{1}{c|}{25871 (10.5\%)} & \multicolumn{1}{c|}{27373 (5.3\%)} & \multicolumn{1}{c|}{25827 (10.7\%)} & \multicolumn{1}{c|}{27375 (5.3\%)} & \textbf{25727 (11.0\%)} \\ \cline{1-15} 

\multicolumn{1}{|c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{25269 (10.6\%)} & \multicolumn{1}{c|}{25093 (11.2\%)} & \multicolumn{1}{c|}{25208 (10.8\%)} & \multicolumn{1}{c|}{25281 (10.5\%)} & \multicolumn{1}{c|}{25377 (10.2\%)} & \multicolumn{1}{c|}{25119 (11.1\%)} & \multicolumn{1}{c|}{25312 (10.4\%)} & \multicolumn{1}{c|}{25566 (9.5\%)} & \multicolumn{1}{c|}{25250 (10.6\%)} & \multicolumn{1}{c|}{26861 (4.9\%)} & \multicolumn{1}{c|}{25175 (10.9\%)} & \multicolumn{1}{c|}{26861 (4.9\%)} & \textbf{25052 (11.3\%)} \\ \cline{1-15} 

\multicolumn{1}{|c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{24751 (10.7\%)} & \multicolumn{1}{c|}{24568 (11.3\%)} & \multicolumn{1}{c|}{24688 (10.9\%)} & \multicolumn{1}{c|}{24818 (10.4\%)} & \multicolumn{1}{c|}{24802 (10.5\%)} & \multicolumn{1}{c|}{24607 (11.2\%)} & \multicolumn{1}{c|}{24757 (10.6\%)} & \multicolumn{1}{c|}{24984 (9.8\%)} & \multicolumn{1}{c|}{24733 (10.7\%)} & \multicolumn{1}{c|}{26191 (5.5\%)} & \multicolumn{1}{c|}{24718 (10.8\%)} & \multicolumn{1}{c|}{26209 (5.4\%)} & \textbf{24553 (11.4\%)}\\ \cline{1-15}

\multicolumn{1}{|c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{26890 (10.4\%)} & \multicolumn{1}{c|}{26708 (11.0\%)} & \multicolumn{1}{c|}{26833 (10.6\%)} & \multicolumn{1}{c|}{27001 (10.0\%)} & \multicolumn{1}{c|}{26962 (10.1\%)} & \multicolumn{1}{c|}{26738 (10.9\%)} & \multicolumn{1}{c|}{26942 (10.2\%)} & \multicolumn{1}{c|}{27188 (9.4\%)} & \multicolumn{1}{c|}{26854 (10.5\%)} & \multicolumn{1}{c|}{28494 (5.0\%)} & \multicolumn{1}{c|}{26810 (10.6\%)} & \multicolumn{1}{c|}{28480 (5.1\%)} & \textbf{26700 (11.0\%)} \\ \hline


\multicolumn{1}{|c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{40965 (28.4\%)} & \multicolumn{1}{c|}{40869 (28.6\%)} & \multicolumn{1}{c|}{40965 (28.4\%)} & \multicolumn{1}{c|}{40866 (28.6\%)} & \multicolumn{1}{c|}{41006 (28.4\%)} & \multicolumn{1}{c|}{40874 (28.6\%)} & \multicolumn{1}{c|}{41004 (28.4\%)} & \multicolumn{1}{c|}{51414 (10.2\%)} & \multicolumn{1}{c|}{41142 (28.1\%)} & \multicolumn{1}{c|}{56224 (1.8\%)} & \multicolumn{1}{c|}{41104 (28.2\%)} & \multicolumn{1}{c|}{56222 (1.8\%)} & \textbf{40849 (28.6\%)}\\ \cline{1-15} 

\multicolumn{1}{|c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{207340 (3.3\%)} & \multicolumn{1}{c|}{206559 (3.6\%)} & \multicolumn{1}{c|}{207343 (3.3\%)} & \multicolumn{1}{c|}{211283 (1.4\%)} & \multicolumn{1}{c|}{207320 (3.3\%)} & \multicolumn{1}{c|}{\textbf{206539 (3.6\%)}} & \multicolumn{1}{c|}{206648 (3.6\%)} & \multicolumn{1}{c|}{207240 (3.3\%)} & \multicolumn{1}{c|}{206671 (3.6\%)} & \multicolumn{1}{c|}{211991 (1.1\%)} & \multicolumn{1}{c|}{206671 (3.6\%)} & \multicolumn{1}{c|}{211991 (1.1\%)} & \textbf{206530 (3.6\%)}\\ \cline{1-15} 

\multicolumn{1}{|c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{46177 (1.4\%)} & \multicolumn{1}{c|}{45650 (2.5\%)} & \multicolumn{1}{c|}{46013 (1.8\%)} & \multicolumn{1}{c|}{46005 (1.8\%)} & \multicolumn{1}{c|}{46171 (1.4\%)} & \multicolumn{1}{c|}{\textbf{45360 (3.2\%)}} & \multicolumn{1}{c|}{46039 (1.7\%)} & \multicolumn{1}{c|}{45855 (2.1\%)} & \multicolumn{1}{c|}{46113 (1.5\%)} & \multicolumn{1}{c|}{46312 (1.1\%)} & \multicolumn{1}{c|}{46077 (1.6\%)} & \multicolumn{1}{c|}{46312 (1.1\%)} & 45418 (3.0\%)\\ \cline{1-15}

\multicolumn{1}{|c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{19327 (21.5\%)} & \multicolumn{1}{c|}{19219 (21.9\%)} & \multicolumn{1}{c|}{19327 (21.5\%)} & \multicolumn{1}{c|}{\textbf{19218 (21.9\%)}} & \multicolumn{1}{c|}{19333 (21.5\%)} & \multicolumn{1}{c|}{19219 (21.9\%)} & \multicolumn{1}{c|}{19333 (21.5\%)} & \multicolumn{1}{c|}{19223 (21.9\%)} & \multicolumn{1}{c|}{19332 (21.5\%)} & \multicolumn{1}{c|}{23661 (3.9\%)} & \multicolumn{1}{c|}{19328 (21.5\%)} & \multicolumn{1}{c|}{23661 (3.9\%)} & \textbf{19217 (21.9\%)}\\ \cline{1-15} 

\multicolumn{1}{|c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{8755 (36.4\%)} & \multicolumn{1}{c|}{\textbf{8428 (38.7\%)}} & \multicolumn{1}{c|}{9109 (33.8\%)} & \multicolumn{1}{c|}{10306 (25.1\%)} & \multicolumn{1}{c|}{9056 (34.2\%)} & \multicolumn{1}{c|}{8612 (37.4\%)} & \multicolumn{1}{c|}{9060 (34.1\%)} & \multicolumn{1}{c|}{8589 (37.6\%)} & \multicolumn{1}{c|}{9789 (28.8\%)} & \multicolumn{1}{c|}{12440 (9.6\%)} & \multicolumn{1}{c|}{9870 (28.3\%)} & \multicolumn{1}{c|}{12440 (9.6\%)} & 8861 (35.6\%) \\ \hline

\multicolumn{2}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{\textbf{18.3\%}} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{16.8\%} & \multicolumn{1}{c|}{16.9\%} & \multicolumn{1}{c|}{\textbf{18.3\%}} & \multicolumn{1}{c|}{17.3\%} & \multicolumn{1}{c|}{15.8\%} & \multicolumn{1}{c|}{17.0\%} & \multicolumn{1}{c|}{9.7\%} & \multicolumn{1}{c|}{17.2\%} & \multicolumn{1}{c|}{9.7\%} & 18.2\%\\ \hline

\multicolumn{2}{|c|}{{\textbf{Avg. Runtime (s)}}} & \multicolumn{1}{c|}{{0.443}} & \multicolumn{1}{c|}{{1.162}} & \multicolumn{1}{c|}{{0.438}} & \multicolumn{1}{c|}{{1.149}} & \multicolumn{1}{c|}{{0.434}} & \multicolumn{1}{c|}{{1.148}} & \multicolumn{1}{c|}{{0.430}} & \multicolumn{1}{c|}{{1.144}} & \multicolumn{1}{c|}{{0.429}} & \multicolumn{1}{c|} {{1.143}} & \multicolumn{1}{c|} {{0.431}} & \multicolumn{1}{c|} {{1.155}} & {1.162}\\ \hline
\end{tabular}
}
% \caption{Detailed results of selected large size designs. Comparison of single-traversal \texttt{orchestration} with stand-alone optimizations from ABC.}
% \vspace{-3mm}
\label{table:3O}
\end{table*}

==> tbls/table_resyn_map.tex <==
\begin{table}[!htb]
\centering
\caption{Detailed results of selected large size designs. Comparison of technology mapping of \texttt{resyn}/\texttt{resyn3} with Best \texttt{O-resyn}. Area and delay are reported in $um^2$ and $ps$.}
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|cccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{6}{c|}{Technology mapping: \texttt{resyn}} \\ \cline{3-8} 
\multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{\texttt{resyn}} & \multicolumn{2}{c|}{\texttt{resyn3}} & \multicolumn{2}{c|}{Best \texttt{O-resyn}} \\ \cline{3-8} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & Delay \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & \multicolumn{1}{c|}{5955.75} & \multicolumn{1}{c|}{12.0} & \multicolumn{1}{c|}{6129.26} & \multicolumn{1}{c|}{\bf 11.0} & \multicolumn{1}{c|}{\textbf{5747.79}} & 12.0 \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & s35932 & \multicolumn{1}{c|}{\textbf{5282.22}} & \multicolumn{1}{c|}{\bf 5.0} & \multicolumn{1}{c|}{6193.42} & \multicolumn{1}{c|}{6.0} & \multicolumn{1}{c|}{5414.85} & {\bf 5.0} \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & b17\_1 & \multicolumn{1}{c|}{12981.71} & \multicolumn{1}{c|}{18.0} & \multicolumn{1}{c|}{14354.19} & \multicolumn{1}{c|}{\bf 17.0} & \multicolumn{1}{c|}{\textbf{12952.42}} & {\bf 17.0} \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & b18\_1 & \multicolumn{1}{c|}{36892.34} & \multicolumn{1}{c|}{\bf 54.0} & \multicolumn{1}{c|}{39672.16} & \multicolumn{1}{c|}{58.0} & \multicolumn{1}{c|}{\textbf{36264.68}} & 56.0 \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & b20 & \multicolumn{1}{c|}{5013.41} & \multicolumn{1}{c|}{25.0} & \multicolumn{1}{c|}{5117.39} & \multicolumn{1}{c|}{\bf 24.0} & \multicolumn{1}{c|}{\textbf{4718.43}} & {\bf 24.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & b21 & \multicolumn{1}{c|}{5154.01} & \multicolumn{1}{c|}{25.0} & \multicolumn{1}{c|}{5289.59} & \multicolumn{1}{c|}{\bf 24.0} & \multicolumn{1}{c|}{\textbf{4877.81}} & {\bf 24.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & b22 & \multicolumn{1}{c|}{7464.92} & \multicolumn{1}{c|}{\bf 25.0} & \multicolumn{1}{c|}{7646.79} & \multicolumn{1}{c|}{\bf 25.0} & \multicolumn{1}{c|}{\textbf{7251.37}} & {\bf 25.0} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & \multicolumn{1}{c|}{15804.08} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{15589.98} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{\textbf{14869.39}} & 29.0 \\ \cline{2-8}

\multicolumn{1}{|c|}{} & dscg & \multicolumn{1}{c|}{15378.06} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{15475.00} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{\textbf{14846.70}} & {\bf 28.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & fir & \multicolumn{1}{c|}{15709.50} & \multicolumn{1}{c|}{\bf 27.0} & \multicolumn{1}{c|}{15544.94} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{\textbf{14794.36}} & 28.0 \\ \cline{2-8}

\multicolumn{1}{|c|}{} & syn2 & \multicolumn{1}{c|}{15943.05} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{15904.37} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{\textbf{15289.84}} & {\bf 27.0} \\ \hline

\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & div & \multicolumn{1}{c|}{23828.21} & \multicolumn{1}{c|}{1452.0} & \multicolumn{1}{c|}{\textbf{19881.61}} & \multicolumn{1}{c|}{1471.0} & \multicolumn{1}{c|}{24884.07} & {\bf 1435.0} \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & hyp & \multicolumn{1}{c|}{159726.43} & \multicolumn{1}{c|}{\bf 8315.0} & \multicolumn{1}{c|}{159690.55} & \multicolumn{1}{c|}{8316.0} & \multicolumn{1}{c|}{\textbf{159446.83}} & {\bf 8315.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & mem\_ctrl & \multicolumn{1}{c|}{13098.80} & \multicolumn{1}{c|}{\bf 37.0} & \multicolumn{1}{c|}{12937.87} & \multicolumn{1}{c|}{\bf 37.0} & \multicolumn{1}{c|}{\textbf{12616.00}} & {\bf 37.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & sqrt & \multicolumn{1}{c|}{10913.79} & \multicolumn{1}{c|}{\bf 2003.0} & \multicolumn{1}{c|}{\textbf{10069.77}} & \multicolumn{1}{c|}{2018.0} & \multicolumn{1}{c|}{10218.57} & {\bf 2003.0} \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & voter & \multicolumn{1}{c|}{8692.15} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{7747.81} & \multicolumn{1}{c|}{29.0} & \multicolumn{1}{c|}{\textbf{7061.83}} & {\bf 26.0} \\ \hline
\multicolumn{2}{|c|}{\textbf{Avg. Area Reduction\%}} & \multicolumn{2}{c|}{\color{red}-4.2\%} & \multicolumn{2}{c|}{\color{red}-4.5\%} & \multicolumn{2}{c|}{ - } \\ \hline
\end{tabular}%
% }
}
% \caption{Detailed results of selected large size designs. Comparison of technology mapping of \texttt{resyn}/\texttt{resyn3} with Best \texttt{O-resyn}. Area and delay are reported in $um^2$ and $ps$.}
\vspace{-4mm}
\label{table:resyn_map}
\end{table}

==> tbls/table_runtime.tex <==
\iffalse
\begin{table}[!htb]
\centering
\caption{Iteration count with a single graph traversal of optimization algorithms applied to selected large size designs.}
\footnotesize
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{4}{c|}{AIG} \\ \cline{3-6}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & Ours \\ \cline{3-6} 
\multicolumn{2}{|c|}{} & \#Iteration & \#Iteration & \#Iteration & \#Iteration \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 12396 & 12277 & 12278 & \textbf{1489} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & s35932 & 11948 & 11948 & 11948 & \textbf{2014} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b17\_1 & 27518 & 27504 & 27611 & \textbf{3635} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b18\_1 & 78440 & 78485 & 78891 & \textbf{10274} \\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b20} & 12093 & 12092 & 12094 & \textbf{1259} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b21 & 12498 & 12525 & 12658 &  \textbf{1402}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b22} & 18151 & 18140 & 18418 &  \textbf{2109}\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 28904 & 28895 & 28910 &  \textbf{2340}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {dscg} & 28237 & 28238 & 28250 &  \textbf{2304}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & fir & 27689 & 27686 & 27703 &  \textbf{2357}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {syn2} & 29991 & 29990 & 30003 &  \textbf{2318}\\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 57245 & 57239 & 57235 &  \textbf{16122}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {hyp} & 214335 & 214335 & 214335 &  \textbf{7113}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & mem\_ctrl & 46836 & 46836 & 46836 &  \textbf{2602}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & sqrt & 24618 & 24617 & 24617 &  \textbf{5290}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & voter & 13697 & 13753 & 13758 & \textbf{3712} \\ \hline
\end{tabular}
% }
}
% \caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:it_count}
\end{table}
\fi

\begin{table}[!htb]
\centering
\caption{\yingjie{Counts of required iterations in a single graph traversal of optimization algorithms with selected large size designs.}}
\footnotesize
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{4}{c|}{AIG} \\ \cline{3-6}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & Ours ($\widehat{\texttt{O3}}$) \\ \cline{3-6} 
\multicolumn{2}{|c|}{} & \#Iteration & \#Iteration & \#Iteration & \#Iteration \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 12396 & 551 & 927 & \textbf{1489} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & s35932 & 11948 & 32 & 1568 & \textbf{2014} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b17\_1 & 27518 & 842 & 1825 & \textbf{3635} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b18\_1 & 78440 & 3490 & 5648 & \textbf{10274} \\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b20} & 12093 & 473 & 714 & \textbf{1259} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b21 & 12498 & 556 & 841 &  \textbf{1402}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b22} & 18151 & 705 & 1171 &  \textbf{2109}\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 28904 & 1374 & 920 &  \textbf{2340}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {dscg} & 28237 & 1433 & 826 &  \textbf{2304}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & fir & 27689 & 1449 & 831 &  \textbf{2357}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {syn2} & 29991 & 1441 & 905 &  \textbf{2318}\\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 57245 & 4539 & 285 &  \textbf{16122}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {hyp} & 214335 & 5149 & 1992 &  \textbf{7113}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & mem\_ctrl & 46836 & 123 & 102 &  \textbf{2602}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & sqrt & 24618 & 2927 & 932 &  \textbf{5290}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & voter & 13697 & 2106 & 738 & \textbf{3712} \\ \hline
\end{tabular}
% }
}
% \caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:it_count}
\end{table}

\iffalse
\begin{table}[!htb]
\centering
\caption{\yingjie{Counts of required iterations in a single graph traversal of optimization algorithms with selected large size designs.}}
\footnotesize
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{4}{*}{Design}} & \multicolumn{8}{c|}{AIG} \\ \cline{3-10}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & \multicolumn{5}{c|}{Orchestration} \\ \cline{3-10} 

 \multicolumn{2}{|c|}{} &    &   &   & &  &  &   & \\

\multicolumn{2}{|c|}{} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter \\ \end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (rw)\end{tabular}}& \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (rs)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (rf)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (none)\end{tabular}} &
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\#Iter\\ (total)\end{tabular}}\\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 12396 & 551 & 927 &   &  &  &  &\textbf{1489}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & s35932 & 11948 & 32 & 1568 &  &  &  & &\textbf{2014} \\ \cline{2-10} 
\multicolumn{1}{|c|}{} & b17\_1 & 27518 & 842 & 1825 &  &  &  & &\textbf{3635}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & b18\_1 & 78440 & 3490 & 5648 &  &  &  & & \textbf{10274} \\ \cline{2-10}
\multicolumn{1}{|c|}{} & {b20} & 12093 & 473 & 714 &   &  &  &  &\textbf{1259}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & b21 & 12498 & 556 & 841 &    &  &  & & \textbf{1402}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & {b22} & 18151 & 705 & 1171 &   &  &  &  & \textbf{2109}\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 28904 & 1374 & 920 &   &  &  &  & \textbf{2340}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & {dscg} & 28237 & 1433 & 826 &   &  &  &  & \textbf{2304}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & fir & 27689 & 1449 & 831 &   &  &  &  & \textbf{2357}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & {syn2} & 29991 & 1441 & 905 &   &  &  &  & \textbf{2318}\\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 57245 & 4539 & 285 &   &  &  &  & \textbf{16122}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & {hyp} & 214335 & 5149 & 1992 &   &  &  &  & \textbf{7113}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & mem\_ctrl & 46836 & 123 & 102 &    &  &  & & \textbf{2602}\\ \cline{2-10}
\multicolumn{1}{|c|}{} & sqrt & 24618 & 2927 & 932 &    &  &  & & \textbf{5290}\\ \cline{2-10} 
\multicolumn{1}{|c|}{} & voter & 13697 & 2106 & 738 &   &  &  & & \textbf{3712}\\ \hline
\end{tabular}
% }
}
% \caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:it_count}
\end{table}
\fi




\iffalse
\begin{table}[!htb]
\centering
\caption{\mingju{Runtime in a single graph traversal of optimization algorithms with selected large size designs.}}
\footnotesize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{10}{c|}{AIG} \\ \cline{3-12}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & $\widehat{\texttt{O4}}$ & \texttt{LGP} \\ \cline{3-12} 
\multicolumn{2}{|c|}{} & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) & runtime(s) \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 0.107 & 0.082 & 0.067 & 0.041 & 0.044 & 0.036 & 0.033 & 0.032 & 0.033 & 0.131 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & s35932 & 0.110 & 0.072 & 0.072 & 0.050 & 0.052 & 0.041 & 0.034 & 0.033 & 0.034 & 0.136 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & b17\_1 & 0.223 & 0.155 & 0.090 & 0.077 & 0.079 & 0.073 & 0.051 & 0.055 & 0.047 & 0.306 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & b18\_1 & 0.573 & 0.340 & 0.289 & 0.237 & 0.241 & 0.215 & 0.131 & 0.130 & 0.118 & 0.878 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & b20 & 0.141 & 0.075 & 0.063 & 0.038 & 0.042 & 0.042 & 0.030 & 0.026 & 0.026 & 0.160 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & b21 & 0.147 & 0.080 & 0.066 &  0.041 & 0.042 & 0.036 & 0.028 & 0.031 & 0.033 & 0.131\\ \cline{2-12}
\multicolumn{1}{|c|}{} & b22 & 0.143 & 0.103 & 0.093 &  0.054 & 0.057 & 0.051 & 0.040 & 0.044 & 0.039 & 0.197\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 0.215 & 0.114 & 0.101 & 0.090 & 0.099 & 0.082 & 0.054 & 0.047 & 0.049 & 0.303 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & {dscg} & 0.221 & 0.124 & 0.086 & 0.104 & 0.096 & 0.092 & 0.050 & 0.051 & 0.047 & 0.310 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & fir & 0.200 & 0.125 & 0.099 & 0.090 & 0.083 & 0.088 & 0.046 & 0.052 & 0.049 & 0.309 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & {syn2} & 0.201 & 0.137 & 0.120 & 0.094 & 0.086 & 0.094 & 0.058 & 0.059 & 0.048 & 0.340 \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 0.530 & 0.244 & 0.203 & 0.345 & 0.355 & 0.346 & 0.116 & 0.116 & 0.093 & 0.737 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & {hyp} & 2.207 & 0.778 & 0.738 & 0.643 & 0.561 & 0.277 & 0.239 & 0.195 & 0.179 & 2.626 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & mem\_ctrl & 0.366 & 0.188 & 0.208 & 0.050 & 0.057 & 0.049 & 0.050 & 0.047 & 0.043 & 0.501 \\ \cline{2-12}
\multicolumn{1}{|c|}{} & sqrt & 0.279 & 0.143 & 0.114 & 0.125 & 0.136 & 0.117 & 0.079 & 0.072 & 0.074 & 0.343\\ \cline{2-12} 
\multicolumn{1}{|c|}{} & voter & 0.188 & 0.079 & 0.075 & 0.080 & 0.074 & 0.061 & 0.054 & 0.055 & 0.044 & 0.242 \\ \hline
\end{tabular}
% }
}
% \caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:real_runtime}
\end{table}
\fi
